H2 MAGIE: H2 as a Major Agent to Galaxy Interaction and Evolution

Spitzer space telescope spectroscopy reveal a new class of H2-luminous galaxies with enhanced H2 line emission, but where star formation is strongly suppressed. This is in sharp contrast with what is observed in standard star forming galaxies. These sources are all in active phases of galaxy evolution (galaxy interactions, AGN feedback, gas accretion in galaxy clusters, etc.). Why is H2 present in violent phases of galaxy evolution? How is the H2 emission powered? Why is the H2 gas inefficient at forming stars? What can we learn from these "H2 galaxies" about galaxy formation? This thesis addresses these questions, and discuss the theoretical and observational perspectives of this work (in particular Herschel and JWST).

==> abrege.tex <==
% TEX 7(ascii) bits
%
% ABREGE.tex
% LaTeX document
% Author: J.I. 
% Date  : Juillet 1996
%
% Raccourcis d'expressions très usitées
%
% Derniere modif le 10-07-96
%

% Raccourci pour \XS
\def\XS{\xspace}

%%%%%%%%%%%%%%%%%%% Pour definir nouvelle commande de changement de taille
\RequirePackage{ifthen}
\RequirePackage{calc}

\newcommand{\taille}[1][\scad]{%
\ifthenelse{#1 = -5}{}{}%
\ifthenelse{#1 = -4}{\tiny}{}%
\ifthenelse{#1 = -3}{\scriptsize}{}%
\ifthenelse{#1 = -2}{\footnotesize}{}%
\ifthenelse{#1 = -1}{\small}{}%
\ifthenelse{#1 = 0}{\normalsize}{}%
\ifthenelse{#1 = 1}{\large}{}%
\ifthenelse{#1 = 2}{\Large}{}%
\ifthenelse{#1 = 3}{\LARGE}{}%
\ifthenelse{#1 = 4}{\huge}{}%
\ifthenelse{#1 = 5}{\Huge}{}}

\newboolean{@serif}
\setboolean{@serif}{true}
\def\scad{-5} % scadefaultsize

\newcounter{taille}
\newcommand{\sca}[2][\scad]{\setcounter{taille}{#1}%
  \ifthenelse{\boolean{@serif}}
  {{\taille[\thetaille]\textsc{#2}}}
  {\setcounter{taille}{\value{taille}-1}{\uppercase{\taille[\thetaille]#2}}}}

% Mise en commentaire rapide !
\def\rem#1{}                    % rem{bla bla bla}

% References automatiquement entre parenthese
\def\reff#1{\XS(\ref{#1})}
\def\refs#1{section~\ref{#1}}
\def\refS#1{Section~\ref{#1}}

\newcommand{\clearemptydoublepage}{\newpage{\pagestyle{empty}\cleardoublepage}}  

% Numéro (pour biblio)
\def\numero{n°}
\def\Numero{N°}

% Majuscules
\def\UP#1{\uppercase{#1}}       % majuscules
\def\up#1{\uppercase{#1}}       % majuscules

% Liste des abreges
\def\adhoc{\textit{ad hoc}\XS}
\def\apost{\textit{a posteriori}\XS}
\def\Apost{\textit{A posteriori}\XS}
\def\APost{\textit{A Posteriori}\XS}
\def\post{\textit{posterior}\XS}
\def\Post{\textit{Posterior}\XS}
\def\afortio{\textit{a fortiori}\XS}
\def\Afortio{\textit{A fortiori}\XS}
\def\aprio{\textit{a priori}\XS}
\def\Aprio{\textit{A priori}\XS}
\def\Cad{C'est-à-dire\XS}
\def\cad{c'est-à-dire\XS}
\def\coeur{c{\oe}ur\XS}
\def\cf{\textit{cf.}\XS}
\def\cv{\textit{curriculum vitæ}\XS}
\def\Cv{\textit{Curriculum vitæ}\XS}
\def\CV{\textit{Curriculum Vitæ}\XS}
\def\eg{\textit{e.g.,}\XS}
\def\etal{\textit{et al.}\XS}
\def\etc{\textit{etc\dots}\XS}
\def\etcoll{{\textit et coll.}\XS}
\def\idem{\textit{idem}\XS}
\def\ie{\textit{i.e.,}\XS}
\def\IFF{\textit{if and only if}\XS}
\def\iid{i.i.d.\XS}
\def\infine{\textit{in fine}\XS}
\def\insit{\textit{in situ}\XS}
\def\inviv{\textit{in vivo}\XS}
\def\oeuvre{{\oe}uvre\XS}
\def\oeuvres{{\oe}uvres\XS}
\def\oeil{{\oe}il\XS}
\def\recto{\textit{recto}\XS}
\def\Toeplitz{T{\oe}plitz\XS}
\def\vav{vis-à-vis\XS}
\def\via{\textit{via}\XS}
\def\vic{\textit{vice-versa}\XS}
\def\verso{\textit{verso}\XS}
%\def\vitae{\textit{vitæ}\XS}
\def\vs{\textit{vs}\XS}
\def\versus{\textit{versus}\XS}
\def\ssi{\textit{si et seulement si}\XS}
\def\strsen{\textit{stricto sensu}\XS}
\def\wrt{w.r.t.\XS}

\def\ier{$^{\text{\small er}}$\XS}
\def\iere{$^{\text{\small re}}$\XS}
\def\ieme{$^{\text{\small e}}$\XS}

\def\primo{\ensuremath{1^{\oD}}\XS}
\def\secundo{\ensuremath{2^{\oD}}\XS}
\def\tertio{\ensuremath{3^{\oD}}\XS}
\def\quatro{\ensuremath{4^{\oD}}\XS}


\newcommand{\art}[1][\scad]{\sca[#1]{art}\XS}
\newcommand{\cnd}[1][\scad]{\sca[#1]{cnd}\XS}
\newcommand{\ndt}[1][\scad]{\sca[#1]{ndt}\XS}
\newcommand{\gnc}[1][\scad]{\sca[#1]{gnc}\XS}
\newcommand{\mfa}[1][\scad]{\sca[#1]{mfa}\XS}
\newcommand{\map}[1][\scad]{\sca[#1]{map}\XS}

\newcommand{\icm}[1][\scad]{\sca[#1]{icm}\XS}
\newcommand{\icd}[1][\scad]{\sca[#1]{icd}\XS}
\newcommand{\rsb}[1][\scad]{\sca[#1]{rsb}\XS}
\newcommand{\snr}[1][\scad]{\sca[#1]{snr}\XS}

\newcommand{\dess}[1][\scad]{\sca[#1]{dess}\XS}
\newcommand{\dea}[1][\scad]{\sca[#1]{dea}\XS}
\newcommand{\deug}[1][\scad]{\sca[#1]{deug}\XS}
\newcommand{\deust}[1][\scad]{\sca[#1]{deust}\XS}
\newcommand{\iut}[1][\scad]{\sca[#1]{iut}\XS}
\newcommand{\iup}[1][\scad]{\sca[#1]{iup}\XS}

\newcommand{\eea}[1][\scad]{\sca[#1]{eea}\XS}
\def\EEA{Électronique Électrotechnique Automatique\XS}
\newcommand{\ats}[1][\scad]{\sca[#1]{ats}\XS}
\def\ATS{Automatique et Traitement du Signal\XS}

\newcommand{\te}[1][\scad]{\sca[#1]{te}\XS}
\def\TE{travaux d'études\XS}
\newcommand{\td}[1][\scad]{\sca[#1]{td}\XS}
\def\TD{travaux dirigés\XS}
\newcommand{\tp}[1][\scad]{\sca[#1]{tp}\XS}
\def\TP{travaux pratiques\XS}
%\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\TDAO{travaux dirigés assistés sur ordinateur\XS}
\newcommand{\tdao}[1][\scad]{\sca[#1]{tdao}\XS}
\def\ts{traitement du signal\XS}
\def\TS{Traitement du Signal\XS}

\newcommand{\gbm}[1][\scad]{\sca[#1]{gbm}\XS}
\newcommand{\irmf}[1][\scad]{\sca[#1]{irm-f}\XS}
\newcommand{\irm}[1][\scad]{\sca[#1]{irm}\XS}
\newcommand{\rmn}[1][\scad]{\sca[#1]{rmn}\XS}
\newcommand{\eeg}[1][\scad]{\sca[#1]{eeg}\XS}
\newcommand{\meg}[1][\scad]{\sca[#1]{meg}\XS}

\newcommand{\stic}[1][\scad]{\sca[#1]{stic}\XS}
\newcommand{\pc}[1][\scad]{\sca[#1]{pc}\XS}

% Operating Systemes 
\newcommand{\linux}[1][\scad]{\sca[#1]{Linux}\XS}
\newcommand{\unix}[1][\scad]{\sca[#1]{Unix}\XS}
\newcommand{\msdos}[1][\scad]{\sca[#1]{msdos}\XS}
\newcommand{\sunos}[1][\scad]{\sca[#1]{Sunos}\XS}
\newcommand{\hupux}[1][\scad]{\sca[#1]{hp-ux}\XS}
\newcommand{\vms}[1][\scad]{\sca[#1]{vms}\XS}
\newcommand{\solaris}[1][\scad]{\sca[#1]{Solaris}\XS}
\newcommand{\winnt}[1][\scad]{\sca[#1]{Windows-nt}\XS}
\newcommand{\vmware}[1][\scad]{\sca[#1]{vmware}\XS}
\newcommand{\win}[1][\scad]{\sca[#1]{Windows}\XS}

% Calcul scientifique
\newcommand{\labview}[1][\scad]{\sca[#1]{Labview}\XS}
\newcommand{\matlab}[1][\scad]{\sca[#1]{Matlab}\XS}
\newcommand{\maple}[1][\scad]{\sca[#1]{Maple}\XS}
\newcommand{\mathe}[1][\scad]{\sca[#1]{Mathematica}\XS}
\newcommand{\idl}[1][\scad]{\sca[#1]{Idl}\XS}

% langages
\newcommand{\cmex}[1][\scad]{\sca[#1]{Cmex}\XS}
\newcommand{\pascal}[1][\scad]{\sca[#1]{Pascal}\XS}
\newcommand{\java}[1][\scad]{\sca[#1]{Java}\XS}
\newcommand{\lisp}[1][\scad]{\sca[#1]{Lisp}\XS}
\newcommand{\forts}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 77}\XS}
\newcommand{\fortq}[1][\scad]{\sca[#1]{Fortran}{\footnotesize 90}\XS}
\newcommand{\ada}[1][\scad]{\sca[#1]{Ada}\XS}
\newcommand{\eiffel}[1][\scad]{\sca[#1]{Eiffel}\XS}
\newcommand{\tcsh}[1][\scad]{\sca[#1]{tcsh}\XS}
\newcommand{\bash}[1][\scad]{\sca[#1]{bash}\XS}
\newcommand{\lgc}[1][\scad]{\sca[#1]{C}\XS}
\newcommand{\cpp}[1][\scad]{\sca[#1]{C}{\footnotesize ++}\XS}

\def\crec{chargé de recherche\XS}
\def\Crec{Chargé de recherche\XS}
\def\dr{directeur de recherche\XS}
\def\Dr{Directeur de recherche\XS}


% congres
\newcommand{\gretsi}[1][\scad]{\sca[#1]{gretsi}\XS}
\newcommand{\maxent}[1][\scad]{\sca[#1]{maxent}\XS}
\newcommand{\icip}[1][\scad]{\sca[#1]{icip}\XS}
\newcommand{\icassp}[1][\scad]{\sca[#1]{icassp}\XS}
\newcommand{\spie}[1][\scad]{\sca[#1]{spie}\XS}
\newcommand{\gdr}[1][\scad]{\sca[#1]{gdr--prc~isis}\XS}
\newcommand{\rfia}[1][\scad]{\sca[#1]{rfia}\XS}
\newcommand{\eusipco}[1][\scad]{\sca[#1]{eusipco}\XS}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Ajout de famouss.tex
% modif le 25/5/2000 Phiphi
% GPInuts - Famous people - VIP
%
\newcommand{\beaunom}[4][0]{{\taille[#1]#2 \uppercase{#3}}%
{\sca[#1]{#4}}\XS}

%\newcommand{\MA}[1][\scad]{{\taille[#1]Marc \uppercase{A}}% 
%{\sca[#1]{llain}\XS}}
\newcommand{\MA}[1][\scad]{\beaunom[#1]{Marc}{A}{llain}}
\newcommand{\FB}[1][\scad]{\beaunom[#1]{François}{B}{oulanger}}
\newcommand{\AB}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc}}
\newcommand{\ABF}[1][\scad]{\beaunom[#1]{Amandine}{B}{lanc~--~Fusco}}
\newcommand{\AAB}[1][\scad]{\beaunom[#1]{Alain}{A}{bergel}}
\newcommand{\AC}[1][\scad]{\beaunom[#1]{Alain}{C}{oulais}}
\newcommand{\AH}[1][\scad]{\beaunom[#1]{Alain}{H}{erment}}
\newcommand{\AHz}[1][\scad]{\beaunom[#1]{Aurélien}{H}{azart}}
\newcommand{\AMD}[1][\scad]{\beaunom[#1]{Ali}{M}{ohammad--Djafari}}
\newcommand{\AR}[1][\scad]{\beaunom[#1]{Andrea}{R}{idolfi}}
\newcommand{\BDuc}[1][\scad]{\beaunom[#1]{Bernard}{D}{uchêne}}
\newcommand{\CH}[1][\scad]{\beaunom[#1]{Christian}{H}{einrich}}
\newcommand{\CS}[1][\scad]{\beaunom[#1]{Charles}{S}{oussen}}
\newcommand{\DLB}[1][\scad]{\beaunom[#1]{Denis}{L}{e Bihan}}
\newcommand{\FC}[1][\scad]{\beaunom[#1]{Frédéric}{C}{hampagnat}}
\newcommand{\FL}[1][\scad]{\beaunom[#1]{Franck}{L}{etimonier}}
\newcommand{\FV}[1][\scad]{\beaunom[#1]{Francisco}{V}{arela}}
\newcommand{\FDU}[1][\scad]{\beaunom[#1]{Frédéric}{D}{ublanchet}}
\newcommand{\FO}[1][\scad]{\beaunom[#1]{Fran\c{c}ois}{O}{rieux}}
\newcommand{\GDE}[1][\scad]{\beaunom[#1]{Guy}{D}{emoment}}
\newcommand{\GS}[1][\scad]{\beaunom[#1]{Grégory}{S}{trubel}}
\newcommand{\GLB}[1][\scad]{\beaunom[#1]{Guy }{L}{e Besnerais}}
\newcommand{\GL}[1][\scad]{\beaunom[#1]{Guilaine }{L}{agache}}
\newcommand{\HC}[1][\scad]{\beaunom[#1]{Hervé}{C}{arfantan}}
\newcommand{\JFB}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{B}{ercher}}
\newcommand{\JFG}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{G}{iovannelli}}
\newcommand{\PG}[1][\scad]{\beaunom[#1]{Pierre}{G}{rangeat}}
\newcommand{\JFM}[1][\scad]{\beaunom[#1]{Jean--Fran\c{c}ois}{M}{angin}}
\newcommand{\JI}[1][\scad]{\beaunom[#1]{Jérôme}{I}{dier}}
\newcommand{\JBP}[1][\scad]{\beaunom[#1]{Jean-Baptiste}{P}{oline}}
\newcommand{\MF}[1][\scad]{\beaunom[#1]{Marc}{F}{ayolle}}
\newcommand{\Mimi}[1][\scad]{\beaunom[#1]{Myriam}{F}{iani}}
\newcommand{\MN}[1][\scad]{\beaunom[#1]{Mila}{N}{ikolova}}
\newcommand{\OF}[1][\scad]{\beaunom[#1]{Olivier}{F}{éron}}
\newcommand{\PC}[1][\scad]{\beaunom[#1]{Philippe}{C}{iuciu}}
\newcommand{\LG}[1][\scad]{\beaunom[#1]{Line}{G}{arnero}}
\newcommand{\SB}[1][\scad]{\beaunom[#1]{Stéphane}{B}{rette}}
\newcommand{\SG}[1][\scad]{\beaunom[#1]{Stéphane}{G}{autier}}
\newcommand{\SBA}[1][\scad]{\beaunom[#1]{Sylvain}{B}{ailet}}
\newcommand{\RB}[1][\scad]{\beaunom[#1]{Redha}{B}{oubertakh}}
\newcommand{\TM}[1][\scad]{\beaunom[#1]{Thierry}{M}{artin}}
\newcommand{\TR}[1][\scad]{\beaunom[#1]{Thomas}{R}{odet}}
\newcommand{\VS}[1][\scad]{\beaunom[#1]{Vincent}{S}{amson}}
\newcommand{\YG}[1][\scad]{\beaunom[#1]{Yves}{G}{oussard}}
\newcommand{\KS}[1][\scad]{\beaunom[#1]{Ken}{S}{auer}}
\newcommand{\HS}[1][\scad]{\beaunom[#1]{Hichem}{S}{noussi}}
\newcommand{\GR}[1][\scad]{\beaunom[#1]{Gilles}{R}{ochefort}}
\newcommand{\NBA}[1][\scad]{\beaunom[#1]{Nicolas}{B}{arbey}}
\newcommand{\FA}[1][\scad]{\beaunom[#1]{Frédéric}{A}{uchère}}
\newcommand{\JCV}[1][\scad]{\beaunom[#1]{Jean--Claude}{V}{ial}}
% Acronymes et raccourcis
%
\def\ATER{Attaché temporaire d'enseignement et de recherche}
\newcommand{\ater}[1][\scad]{\sca[#1]{ater}\xspace}
\def\ADDOC{Agir pour les Doctorants et les jeunes Docteurs\XS}
\newcommand{\addoc}[1][\scad]{\sca[#1]{addoc}\XS}

\def\CdO{Faculté d'Orsay\XS}

\def\CEA{Commissariat à l'Énegie Atomique\XS}
\newcommand{\cea}[1][\scad]{\sca[#1]{cea}\XS}
\newcommand{\dam}[1][\scad]{\sca[#1]{dam}\XS}
\def\DRM{Département de Recherche Médicale\XS}
\newcommand{\drm}[1][\scad]{\sca[#1]{drm}\XS}
\def\DSV{Direction des Sciences du Vivant\XS}
\newcommand{\dsv}[1][\scad]{\sca[#1]{dsv}\XS}
\newcommand{\leti}[1][\scad]{\sca[#1]{leti}\XS}
\newcommand{\minatec}[1][\scad]{\sca[#1]{minatec}\XS}
\def\SHFJ{Service Hospitalier Frédéric Joliot\XS}
\newcommand{\shfj}[1][\scad]{\sca[#1]{shfj}\XS}
\def\UNAF{Unité de Neuroimagerie Anatomo Foncxtionnelle\XS}
\newcommand{\unaf}[1][\scad]{\sca[#1]{unaf}\XS}


\newcommand{\chu}[1][\scad]{\sca[#1]{chu}\XS}
\def\CHU{Centre Hospitalier Universitaire\XS}
\def\salpe{Salpétrière\XS}
\def\hsalpe{Hôpital de la Salpétrière\XS}
\def\pisalpe{Pitié-Salpétrière\XS}
\def\gpisalpe{Groupe Pitié-Salpétrière\XS}
\def\LIF{Laboratoire d'Imagerie Fonctionnelle\XS}
\def\lif{\textsc{lif}\XS}

\def\CNRS{Centre National de la Recherche Scientifique\XS}
\newcommand{\cnrs}[1][\scad]{\sca[#1]{cnrs}\XS}

\def\CNES{Centre National d'Études Spatiales\XS}
\newcommand{\cnes}[1][\scad]{\sca[#1]{cnes}\XS}

\newcommand{\edf}[1][\scad]{\sca[#1]{edf}\XS}
\def\EDF{Électricité de France\XS}

\def\ENSTA{École Nationale Supérieure de Techniques Avancées\XS}
\newcommand{\ensta}[1][\scad]{\sca[#1]{ensta}\XS}

\def\ENST{École Nationale Supérieure des Télécommunications\XS}
\newcommand{\enst}[1][\scad]{\sca[#1]{enst}\XS}


\def\ESIEA{École Supérieure d'Informatique Électronique Automatique\XS}
\newcommand{\esiea}[1][\scad]{\sca[#1]{esiea}\XS}
\newcommand{\ensea}[1][\scad]{\sca[#1]{ensea}\XS}


\def\GPI{Groupe Problèmes Inverses\XS}
\newcommand{\gpi}[1][\scad]{\sca[#1]{gpi}\XS}

\def\INSERM{Institut National pour la Santé et la Recherche Médicale\XS}
\newcommand{\inserm}[1][\scad]{\sca[#1]{inserm}\XS}

\def\CNAM{Conservatoire National des Arts et Métiers\XS}
\newcommand{\cnam}[1][\scad]{\sca[#1]{cnam}\XS}

\def\OPM{Observatoire de Paris\XS}
\newcommand{\opm}[1][\scad]{\sca[#1]{opm}\XS}

\def\INRIA{Institut National de Recherche et Informatique et Automatique\XS}
\newcommand{\inria}[1][\scad]{\sca[#1]{inria}\XS}

\def\IAS{Institut d'Astrophysique Spatiale\XS}
\newcommand{\ias}[1][\scad]{\sca[#1]{ias}\XS}

\def\IAP{Institut d'Astrophysique de Paris\XS}
\newcommand{\iap}[1][\scad]{\sca[#1]{iap}\XS}

\newcommand{\ipsn}[1][\scad]{\sca[#1]{ipsn}\XS}
\def\IPSN{Institut de Protection et de Sureté Nucléaire\XS}

\def\LSS{Laboratoire des Signaux et Systèmes\XS}
\newcommand{\lss}[1][\scad]{\sca[#1]{l{\footnotesize 2}s}\XS}

\def\LIMSI{Laboratoire d'Informatique pour la Mécanique et les Sciences de l'Ingénieur\XS}
\newcommand{\limsi}[1][\scad]{\sca[#1]{limsi-cnrs}\XS}

\def\ONERA{Office National d'Études et de Recherches Aérospatiales\XS}
\newcommand{\onera}[1][\scad]{\sca[#1]{onéra}\XS}

\def\CLS{Collecte Localisation Satellites\XS}
\newcommand{\cls}[1][\scad]{\sca[#1]{cls}\XS}

%\def\ONERA{Office National d'Études et de Recherches Aérospatiales\XS}
\newcommand{\Loreal}[1][\scad]{\sca[#1]{L'oréal}\XS}


\def\MDC{Maître de conférences\XS}
\def\MDCs{Maîtres de conférences\XS}
\newcommand{\mdc}[1][\scad]{\sca[#1]{mdc}\XS}

\newcommand{\UND}[1][\scad]{Université de Notre Dame, \sca[#1]{usa}\XS}

%\def\UPS{Université Paris-Sud\XS}
\newcommand{\UPS}[1][\scad]{{Université Paris-Sud 11}\XS} % Modifié FO -- le 16-07-07 % Modifié TR -- le 26-02-08
\newcommand{\ups}[1][\scad]{\sca[#1]{ups}\XS}
\newcommand{\upxi}[1][\scad]{\sca[#1]{upxi}\XS}

% Unites Thomson
\newcommand{\thomair}[1][\scad]{\sca[#1]{Thomson-csf Airsys}\XS}
\newcommand{\oscar}[1][\scad]{\sca[#1]{Oscar}\XS}
\newcommand{\thomrcm}[1][\scad]{\sca[#1]{Thomson-rcm}\XS}

% Unite propre de recherche
\newcommand{\upr}[1][\scad]{\sca[#1]{upr}\XS}
% LENA, lena upr640,...
\newcommand{\uprlen}[1][\scad]{\sca[#1]{upr}{\footnotesize 640}\XS}
\def\LENA{Laboratoire d'Encéphalographie et de Neurophysiologie Appliquée\XS}
\newcommand{\lena}[1][\scad]{\sca[#1]{lena}\XS}
% Nous
\def\GsY{Gif--sur--Yvette\XS}
%\newcommand{\ESE}[1][\scad]{\sca[#1]{supélec}\XS}
\newcommand{\ESE}[1][\scad]{{Supélec}\XS}% Modifié Gio -- le 16-03-05


\def\adrshort{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex\XS}
%\def\adresse{\ESE, Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\hiercea}[1][\scad]{\dsv[#1]/\drm[#1]/\shfj[#1]\XS}

\newcommand{\adresselss}[1][\scad]{\ESE[#1], Plateau de Moulon, 91192 Gif--sur--Yvette Cedex, France\XS}
\newcommand{\adresscea}[1][\scad]{4 Place du Général Leclerc, 91406 Orsay Cedex, France\XS}
\newcommand{\tutelle}[1][\scad]{\cnrs[#1]~--~\ESE[#1]~--~\ups[#1]}
\def\ALSS{\LSS~(\tutelle)\\\adresselss}
\def\ALSSun{\LSS (\tutelle) \adresselss}
%

\newcommand{\tutelleIAS}[1][\scad]{\cnrs[#1]~--~\ups[#1]}
\newcommand{\adresseIAS}[1][\scad]{\UPS[#1], Bât. 121, 91405 Orsay, France\XS}
\def\AIAS{\IAS~(\tutelleIAS)\\ \adresseIAS}

% ---------------------------------------------------- 
% Modele d'en-tete par A. Mohammad-Djafari et J. Idier 
% ---------------------------------------------------- 
%
\def\helvnormal#1{{\fontfamily{phv}\fontsize{11}{14pt}\selectfont #1}}
\def\helvfoot  #1{{\fontfamily{phv}\fontsize{9}{14pt} \selectfont #1}}
\def\helvscript#1{{\fontfamily{phv}\fontsize{8}{14pt} \selectfont #1}}
%
\newcommand{\entete}[5][Nom.Prénom]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Supélec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique          \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYSTÈMES}}\\%
\helvfoot{Unité mixte de recherche n$^{\rm o}$ 8506\\%
Supélec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
Téléphone\,: 01 69 85 17 12 --- 
Télécopie\,: 01 69 85 17 65 --- 
Courriel\,: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{V/Réf.\,: #2} & \helvscript{\sca[-3]{Gif}, le} #5\\%
\helvscript{N/Réf.\,: #3} \\%
\helvscript{Objet\,: #4}%
\end{tabular}
} 

\newcommand{\inhead}[5][Name.Surname]{
%%%%%%\def\entete#1#2#3#4#5{%
\helvscript{\renewcommand{\arraystretch}{.8}
\begin{tabular}{c} Supélec
\\--------\end{tabular} \hfill
\begin{tabular}{c}Centre national de la recherche scientifique  \\
--------\end{tabular} \hfill
\begin{tabular}{c}\UPS  \\--------\end{tabular}} \\[-.4cm]%
%
\begin{center}\helvnormal{\textbf{LABORATOIRE DES SIGNAUX \& SYSTÈMES}}\\%
\helvfoot{Unité mixte de recherche n$^{\rm o}$ 8506\\%
Supélec, plateau de Moulon, 
3 rue Joliot-Curie, 91192 \sca[-3]{Gif--sur--Yvette} Cedex (France)\\%
Telephone: 01 69 85 17 12 --- 
Fax: 01 69 85 17 65 --- 
E-mail: {#1}@lss.supelec.fr}%
\\[0.5cm]\end{center}% 
\begin{tabular}{p{8.5cm}l}%
\helvscript{Y/Ref.: #2} & \helvscript{\sca[-3]{Gif}, } #5\\%
\helvscript{O/Ref.: #3} \\%
\helvscript{Subject: #4}%
\end{tabular}
} 



==> abstracts_announcement.tex <==


Résumé en français:

La découverte d'une nouvelle population de sources extragalactiques avec un spectre dans l'infrarouge moyen (MIR) dominé par les raies d'émission de l'hydrogène moléculaire (H2) est un résultat inattendu des observations spectroscopiques du satellite Spitzer.
Ces sources sont toutes dans des phases actives de l'évolution des galaxies (intéractions entre galaxies, rétroaction des noyaux actifs sur le milieu interstellaire de leur galaxie-hôte, accrétion de gaz dans les amas, etc.). Contrairement à ce qui est observé dans les galaxies standard, ces objets possèdent une grande quantité de gaz moléculaire, mais ont une faible intensité de formation stellaire. Pourquoi H2 est-il présent dans ces phases violentes d'évolution? Comment l'émission de H2 est-elle produite? Pourquoi le gaz H2 est-il si inefficace à former des étoiles? Que nous apprennent ces ``galaxies H2'' sur la formation des galaxies? Je discuterai ces questions au cours de cette présentation, puis donnerai les perspectives théoriques et observationnelles (en particulier avec les satellites Herschel et JWST) de ce travail.

Abstract in english

Spitzer space telescope spectroscopy reveal a new class of H2-luminous galaxies with enhanced H2 line emission, but where star formation is strongly suppressed. This is in sharp contrast with what is observed in standard star forming galaxies. These sources are all in active phases of galaxy evolution (galaxy interactions, AGN feedback, gas accretion in galaxy clusters, etc.). Why is H2 present in violent phases of galaxy evolution? How is the H2 emission powered? Why is the H2 gas inefficient at forming stars? What can we learn from these ``H2 galaxies'' about galaxy formation? This presentation will address these questions, and discuss the theoretical and observational perspectives (in particular Herschel and JWST).



==> alphabet.tex <==
% Document LaTeX        Auteur : Guy Le Besnerais       Date : 25/05/94
% Modification : J.-F. Gio      (15/09/95)
%                               J.I. (format Latex 2e, taille adaptative 22/03/99)
%                                    (fonte blackboard 27/08/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% c pour cursif : \Ac
% bb pour blackboard : \Abb
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace, amsmath, bbm)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}
\RequirePackage{bbm}
\RequirePackage{oldgerm}		% 04.06.2003   Pour les alphabet Gauthiques

%-------------------------------------------

% DEFINITIONS PRELIMINAIRES 

\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)           
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)           
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

%-------------------------------------------

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}


% ALPHABET CURSIF MAJUSCULE, taille adaptative
% Cursif,               % Cursif gras

\def\Ac{{\scu{A}}\XS}   \def\Acb{{\scb{A}}\XS}
\def\Bc{{\scu{B}}\XS}   \def\Bcb{{\scb{B}}\XS}
\def\Cc{{\scu{C}}\XS}   \def\Ccb{{\scb{C}}\XS}
\def\Dc{{\scu{D}}\XS}   \def\Dcb{{\scb{D}}\XS}
\def\Ec{{\scu{E}}\XS}   \def\Ecb{{\scb{E}}\XS}
\def\Fc{{\scu{F}}\XS}   \def\Fcb{{\scb{F}}\XS}
\def\Gc{{\scu{G}}\XS}   \def\Gcb{{\scb{G}}\XS}
\def\Hc{{\scu{H}}\XS}   \def\Hcb{{\scb{H}}\XS}
\def\Ic{{\scu{I}}\XS}   \def\Icb{{\scb{I}}\XS}
\def\Jc{{\scu{J}}\XS}   \def\Jcb{{\scb{J}}\XS}
\def\Kc{{\scu{K}}\XS}   \def\Kcb{{\scb{K}}\XS}
\def\Lc{{\scu{L}}\XS}   \def\Lcb{{\scb{L}}\XS}
\def\Mc{{\scu{M}}\XS}   \def\Mcb{{\scb{M}}\XS}
\def\Nc{{\scu{N}}\XS}   \def\Ncb{{\scb{N}}\XS}
\def\Oc{{\scu{O}}\XS}   \def\Ocb{{\scb{O}}\XS}
\def\Pc{{\scu{P}}\XS}   \def\Pcb{{\scb{P}}\XS}
\def\Qc{{\scu{Q}}\XS}   \def\Qcb{{\scb{Q}}\XS}
\def\Rc{{\scu{R}}\XS}   \def\Rcb{{\scb{R}}\XS}
\def\Sc{{\scu{S}}\XS}   \def\Scb{{\scb{S}}\XS}
\def\Tc{{\scu{T}}\XS}   \def\Tcb{{\scb{T}}\XS}
\def\Uc{{\scu{U}}\XS}   \def\Ucb{{\scb{U}}\XS}
\def\Vc{{\scu{V}}\XS}   \def\Vcb{{\scb{V}}\XS}
\def\Wc{{\scu{W}}\XS}   \def\Wcb{{\scb{W}}\XS}
\def\Xc{{\scu{X}}\XS}   \def\Xcb{{\scb{X}}\XS}
\def\Yc{{\scu{Y}}\XS}   \def\Ycb{{\scb{Y}}\XS}
\def\Zc{{\scu{Z}}\XS}   \def\Zcb{{\scb{Z}}\XS}


% ALPHABET DROIT EN MATHS, taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT, taille adaptative

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% Nouveau (08/99) : ALPHABET BLACKBOARD, taille adaptative

\def\Abb{{\sbl{A}}\XS}  \def\abb{{\sbl{a}}\XS}
\def\Bbb{{\sbl{B}}\XS}  \def\bbb{{\sbl{b}}\XS}
\def\Cbb{{\sbl{C}}\XS}  \def\cbb{{\sbl{c}}\XS}
\def\Dbb{{\sbl{D}}\XS}  \def\dbb{{\sbl{d}}\XS}
\def\Ebb{{\sbl{E}}\XS}  \def\ebb{{\sbl{e}}\XS}
\def\Fbb{{\sbl{F}}\XS}  \def\fbb{{\sbl{f}}\XS}
\def\Gbb{{\sbl{G}}\XS}  \def\gbb{{\sbl{g}}\XS}
\def\Hbb{{\sbl{H}}\XS}  \def\hbb{{\sbl{h}}\XS}
\def\Ibb{{\sbl{I}}\XS}  \def\ibb{{\sbl{i}}\XS}
\def\Jbb{{\sbl{J}}\XS}  \def\jbb{{\sbl{j}}\XS}
\def\Kbb{{\sbl{K}}\XS}  \def\kbb{{\sbl{k}}\XS}
\def\Lbb{{\sbl{L}}\XS}  \def\lbb{{\sbl{l}}\XS}
\def\Mbb{{\sbl{M}}\XS}  \def\mbb{{\sbl{m}}\XS}
\def\Nbb{{\sbl{N}}\XS}  \def\nbb{{\sbl{n}}\XS}
\def\Obb{{\sbl{O}}\XS}  \def\obb{{\sbl{o}}\XS}
\def\Pbb{{\sbl{P}}\XS}  \def\pbb{{\sbl{p}}\XS}
\def\Qbb{{\sbl{Q}}\XS}  \def\qbb{{\sbl{q}}\XS}
\def\Rbb{{\sbl{R}}\XS}  \def\rbb{{\sbl{r}}\XS}
\def\Sbb{{\sbl{S}}\XS}  \def\sbb{{\sbl{s}}\XS}
\def\Tbb{{\sbl{T}}\XS}  \def\tbb{{\sbl{t}}\XS}
\def\Ubb{{\sbl{U}}\XS}  \def\ubb{{\sbl{u}}\XS}
\def\Vbb{{\sbl{V}}\XS}  \def\vbb{{\sbl{v}}\XS}
\def\Wbb{{\sbl{W}}\XS}  \def\wbb{{\sbl{w}}\XS}
\def\Xbb{{\sbl{X}}\XS}  \def\xbb{{\sbl{x}}\XS}
\def\Ybb{{\sbl{Y}}\XS}  \def\ybb{{\sbl{y}}\XS}
\def\Zbb{{\sbl{Z}}\XS}  \def\zbb{{\sbl{z}}\XS}


% ALPHABET GREC GRAS italique, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}      \def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\varkappab   {{\sbmm{\varkappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}     \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}         \def\Xib       {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}         \def\Pib       {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}   \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib      {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib      {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}


% CHIFFRES
% Gras et Blackboard, taille adaptative

\def\zerob   {{\sbv{0}}\XS}        \def\zerobb   {{\sbl{O}}\XS}
\def\unb     {{\sbv{1}}\XS}        \def\unbb     {{\sbl{1}}\XS}
\def\deuxb   {{\sbv{2}}\XS}        \def\deuxbb   {{\sbl{2}}\XS}
\def\troisb  {{\sbv{3}}\XS}        \def\troisbb  {{\sbl{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}        \def\quatrebb {{\sbl{4}}\XS}
\def\cinqb   {{\sbv{5}}\XS}        \def\cinqbb   {{\sbl{5}}\XS}
\def\sixb    {{\sbv{6}}\XS}        \def\sixbb    {{\sbl{6}}\XS}
\def\septb   {{\sbv{7}}\XS}        \def\septbb   {{\sbl{7}}\XS}
\def\huitb   {{\sbv{8}}\XS}        \def\huitbb   {{\sbl{8}}\XS}
\def\neufb   {{\sbv{9}}\XS}        \def\neufbb   {{\sbl{9}}\XS}


% QUELQUES ENSEMBLES

\def\eC{\Cbb}
\def\eE{\Ebb}
\def\eN{\Nbb}
\def\eQ{\Qbb}
\def\eR{\Rbb}
\def\eZ{\Zbb}

% ALPHABET GAUTHIQUES  04.06.2003  M.M. ICHIR

\def\Ag{{\textgoth{A}}\XS}  \def\ag{{\textgoth{a}}\XS}
\def\Bg{{\textgoth{B}}\XS}  \def\bg{{\textgoth{b}}\XS}
\def\Cg{{\textgoth{C}}\XS}  \def\cg{{\textgoth{c}}\XS}
\def\Dg{{\textgoth{D}}\XS}  \def\dg{{\textgoth{d}}\XS}
\def\Eg{{\textgoth{E}}\XS}  \def\eg{{\textgoth{e}}\XS}
\def\Fg{{\textgoth{F}}\XS}  \def\fg{{\textgoth{f}}\XS}
\def\Gg{{\textgoth{G}}\XS}  %\def\gg{{\textgoth{g}}\XS}
\def\Hg{{\textgoth{H}}\XS}  \def\hg{{\textgoth{h}}\XS}
\def\Ig{{\textgoth{I}}\XS}  \def\ig{{\textgoth{i}}\XS}
\def\Jg{{\textgoth{J}}\XS}  \def\jg{{\textgoth{j}}\XS}
\def\Kg{{\textgoth{K}}\XS}  \def\kg{{\textgoth{k}}\XS}
\def\Lg{{\textgoth{L}}\XS}  \def\lg{{\textgoth{l}}\XS}
\def\Mg{{\textgoth{M}}\XS}  \def\mg{{\textgoth{m}}\XS}
\def\Ng{{\textgoth{N}}\XS}  \def\ng{{\textgoth{n}}\XS}
\def\Og{{\textgoth{O}}\XS}  \def\og{{\textgoth{o}}\XS}
\def\Pg{{\textgoth{P}}\XS}  \def\pg{{\textgoth{p}}\XS}
\def\Qg{{\textgoth{Q}}\XS}  \def\qg{{\textgoth{q}}\XS}
\def\Rg{{\textgoth{R}}\XS}  \def\rg{{\textgoth{r}}\XS}
\def\Sg{{\textgoth{S}}\XS}  \def\sg{{\textgoth{s}}\XS}
\def\Tg{{\textgoth{T}}\XS}  \def\tg{{\textgoth{t}}\XS}
\def\Ug{{\textgoth{U}}\XS}  \def\ug{{\textgoth{u}}\XS}
\def\Vg{{\textgoth{V}}\XS}  \def\vg{{\textgoth{v}}\XS}
\def\Wg{{\textgoth{W}}\XS}  \def\wg{{\textgoth{w}}\XS}
\def\Xg{{\textgoth{X}}\XS}  \def\xg{{\textgoth{x}}\XS}
\def\Yg{{\textgoth{Y}}\XS}  \def\yg{{\textgoth{y}}\XS}
\def\Zg{{\textgoth{Z}}\XS}  \def\zg{{\textgoth{z}}\XS}


==> chapter_MolecularGasInGalaxies.tex <==

%%% Chapter heading commands %%%
\chapter{The multiphase interstellar medium (ISM) in galaxies}
\label{chapter:mol_galaxies}

%\renewcommand{\publ}{\flushleft\footnotesize{Published as:
%C. Grigorescu, N. Petkov and M.A. Westenberg -- \textit{``Contour
%Detection Based on non-CRF Inhibition,''} IEEE Transactions on Image
%Processing, vol. 12, no. 7, pp. 729--739, July 2003.}}


\epigraph{I hate quotations. Don't use quotations. Tell me what you know.}{
Ralph Waldo Emerson}
%\epigraph{The question is not what you look at, but what you
%see.}{Henry David Thoreau}

%\index{Molecular hydrogen in space!Mol}

%%% Abstract %%%

\begin{Abstract}


\end{Abstract}

\minitoc

%%% Chapter sections %%%

%\index{Visual system}
\section{The gaseous phases of the ISM}
\label{sec:}
%\PARstart{O}

\section{Interstellar dust in galaxies}
\label{sec:}

\begin{floatingfigure}[r]{0.52\textwidth}
   \includegraphics[width=0.52\textwidth]{figures/fun/interstellar_dust_maid.png}
\end{floatingfigure}


\section{Gas cooling and thermal instability}
\label{sec:}


\section{Molecular gas and star formation}
\label{sec:}

Relation between molecular gas and star formation: Schmidt-Kennicut law.

==> chapter_SQ_H2_full_v20090910.tex <==
\part{Detailed studies of H$_{\bf 2}$-luminous sources in space}

%%% Chapter heading commands %%%
\chapter{Powerful H$_{\bf 2}$ emission from the Stephan's Quintet galaxy-wide shock}
\label{chapter:H2_SQ}

%\renewcommand{\publ}{\flushleft\footnotesize{Published as:
%C. Grigorescu, N. Petkov and M.A. Westenberg -- \textit{``Contour
%Detection Based on non-CRF Inhibition,''} IEEE Transactions on Image
%Processing, vol. 12, no. 7, pp. 729--739, July 2003.}}

\epigraph{Nothing shocks me. I'm a scientist.}{Indiana Jones, \textit{in Indiana Jones and the Temple of Doom}}

%%% Abstract %%%

\begin{Abstract}
The Stephan's Quintet (SQ) is a compact group of interacting galaxies and a spectacular example of H$_2$ luminous source. The \textit{Spitzer Space Telescope} indeed detected a powerful mid-infrared H$_{2}$ line emission from the X-ray bright galaxy-wide shock created by the high-velocity ($\sim 1000$~km~s$^{-1}$) collision between a galaxy and the tidail tail of an other member of the group. Observations shows that the H$_{2}$ gas is extremely turbulent and that the H$_2$ luminosity exceeds that of the X-rays. The core of my PhD work was dedicated to the interpretation of these observations. 
In this chapter we give an overview of the multi-wavelength observations of SQ, and we present our results on H$_2$ formation and excitation in the SQ shock.
\end{Abstract}

\minitoc
%%% Chapter sections %%%

\index{Stephan's Quintet}

\section{Introduction}
\label{sec:SQ_intro}

\PARstart{S}tephan's Quintet (hereafter SQ) is a fascinating example of an interacting galaxy system (Fig.~\ref{fig_SQ_HST_legend}). Perhaps not as famous as Arp 220 or M82, SQ is a well-known astrophysical target for amateur or professional astronomers. It is a nearby (94~Mpc) compact group of galaxies situated in the Pegasus constellation, at about half a degree to the South-West of NGC~7331\footnote{\url{http://antwrp.gsfc.nasa.gov/apod/ap071124.html}}. SQ has been observed in almost all wavebands, and it keeps revealing surprises when being looked at by new instruments.
SQ belongs to a peculiar class of interacting systems of galaxies: the compact groups \citep{Hickson1982} that are characterized by aggregates of more than $4$ galaxies in implied space densities as high as those in galaxy cluster cores. 

SQ is a complex web of galaxy-galaxy and galaxy-intragroup medium (henceforth IGM) interactions that have triggered different types of phenomena related to the interactions, including an IGM starburst, long tidal tails ($>100$~kpc) with tidal dwarf candidates, and a  large scale shock ($\sim 40$~kpc long). This shock is materialized by  a giant X-ray and radio-bright \textit{ridge}, attributed to the collision of an intruding galaxy with the tidal tail of another member of the group. 


In 2006, \textit{Spitzer Space Telescope} observations revealed a powerful mid-IR H$_2$ rotational line emission in the SQ shock structure. This discovery makes SQ the first known example of an \textit{``$\rm H_2$-luminous source''}, among the emerging class of MOHEG galaxies presented in chapter~\ref{chapter:mol_galaxies}. This was perhaps one of the most exciting results of extragalactic spectroscopic observations carried out with the \textit{Spitzer} mission. 

This surprising observational result was published at the start of my PhD thesis. Much of my PhD work was dedicated to its interpretation. I have devoted a significant part of my time in building a theoretical model that attempts to explain the formation and excitation of H$_2$ in the SQ galaxy collision within the broader framework of the numerous multi-wavelength observations of the system. It was not an easy task (!), and I will try to show that our current understanding is the result of a long path, along which several working hypothesis have been explored before coming to what we think to be a ``coherent'' scenario. 
This work has been published in \citet{Guillard2009} (hereafter \hyperref[paper_SQ_H2]{paper~{\sc i}}). In this manuscript, I will introduce the two questions of H$_2$ formation and excitation almost independently. The physical processes that lead to such a powerful H$_2$ emission are not understood in details and remain largely unexplored by mean of quantitative models.



After reading this chapter, I hope that the reader will be conviced that SQ is an outstanding source to study in detail phenomena such as large scale shocks and high velocity galaxy collisions. SQ is a beautiful example of astrophysical source where detailed and rich micro-physics of the ISM are needed to understand the global observational picture. These studies have implications for our understanding of the dynamics and energetics of the molecular gas in galaxy evolution.

%More generally, inferences from these studies are crucial to understand the physics of high-redshift galaxy interactions, which is a key process in galaxy formation and evolution.   


In this chapter, I will first present the observational discovery of H$_2$ emission in SQ, which was followed by deeper and more extended \textit{Spitzer} spectroscopy (sect.~\ref{sec:H2obsSQ}). These observations raise a set of astrophysical questions. 
Before adressing these questions by a theoretical interpretation work, I describe the SQ group of galaxies and give an overview of its multi-wavelength data (sect.~\ref{sec:SQ_context}). This review is focused on the evidences for a high-speed, galaxy-wide shock. This is crucial to understand the complexity of this interacting system and to set the context for the interpretation of the H$_2$ emission. These observations set the mass and energy budget of the collision, which is the first step to understand the mechanisms that produce the high H$_2$ luminosity. Then sect.~\ref{sec:H2formation_SQ}  adresses the question of the H$_2$ formation in the SQ shock. I present the long route that drove us to our current interpretation of these observations and introduce our \hyperref[paper_SQ_H2]{paper~{\sc i}}. Our modeling of the H$_2$ line excitation is described in sect.~\ref{sec:H2-excitation}. Then I discuss  the dynamical picture of the energy transfer between the ISM phases that emerges from this interpretation (sect.~\ref{sec:SQ-Why-H2-important-coolant}). 
This work on H$_2$ is complemented by the interpretation of the emission from the ionized gas in the group (optical and fine-structure mid-IR lines, sect.~\ref{sec:opt-midIR-line-excit}). 
Section~\ref{SQ-NGC7319-comments} comments about the AGN member of the group, NGC~7319, which shows an interesting H$_2$ feature revealed by our new \textit{IRS} spectral maps. A quick summary and concluding remarks end this chapter (sect.~\ref{sec:SQ-conclusions})

%Thermal mid-IR emission and star formation will be discussed in chapter~\ref{chapter:SQ_dust}.  


\section{Observations of warm H$_{\bf 2}$ gas in Stephan's Quintet}
\label{sec:H2obsSQ}
\index{Stephan's Quintet!H$_2$ emission}


The first mid-IR spectroscopic observations of the SQ shock were performed by \citet{Appleton2006}. 
We present the observational discovery based on single-pointing observations (sect.~\ref{subsec:SQdiscoveryH2}), and their extension to new spectral maps (sect.~\ref{subsec:spectral_IRSmap_H2}).


\subsection{The discovery: an H$_{\bf 2}$-bright giant shock!}
\label{subsec:SQdiscoveryH2}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: IRS OBSERVATIONS OF SQ by APPLETON 2006
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[width=\textwidth]{figures/sq/SQ_IRS_obs_Appleton06.pdf}
      \caption[\textit{Spitzer IRS} H$_2$ observations by \citet{Appleton2006}]{\textit{Spitzer IRS} H$_2$ observations by \citet{Appleton2006}. \textit{Left:} Positioning of the \textit{IRS} slits overlaid on an R-band image and \textit{VLA} radio contours at 1.4$\,$GHz by \citet{Xu2003}. The slits are centered on $\alpha_{J2000} = 22$h35m59s.57, $\delta_{J2000} = 33^{\rm o}$58'1.8''. Only the central portion of the slits
(red boxes) were common to the two separate observing (nod) positions made in
each IRS module slit (the purple shows the full coverage). $\rm SL = 57 \times 3.6$~arcsec$^{2}$,
$\rm SH = 11.3 \times 4.7$~arcsec$^{2}$, and $\rm LH = 22.3 \times 11.1$~arcsec$^{2}$. \textit{Right: } top:  IRS SH spectrum of the brightest radio/IR point in the shock front. Middle: Combined SH (gray line) and LH (black line) spectrum of the
same target region. Bottom left: SL spectrum at the same position. SL2 is the gray line, and SL1 is the black line. Bottom right: zoom on the 17$\,\mu$m H$_2$ 0-0 S(1) line (detected with a signal-to-noise ratio of 33) showing that the line is resolved (intrinsic FWHM of $870 \pm 60$~km~s$^{-1}$) as compared with two unresolved spectral lines
($\mathcal{R} = 600$) in the planetary nebula NGC 6543 at 15.6 and 18.7$\,\mu$m that bracket the H$_2$ line (gray line).}
       \label{SQ_IRS_obs_Appleton06}
\end{figure}


The \emph{Spitzer} Infra-Red Spectrograph (\textit{IRS}) observations of the SQ galaxy-wide collision led to the unexpected detection of extremely bright mid-IR $\rm H_2$ rotational line emission from warm ($\sim 50 - 10^{3}\,$K) molecular gas in the center of the X-ray emitting ridge \citep{Appleton2006}.
The observational results about the first detection of H$_2$ in the SQ shock are summarized in Fig.~\ref{SQ_IRS_obs_Appleton06}. The left panel shows the position of the \textit{IRS} slits (SH, LH and SL modules; see caption for the slit sizes) overlaid on a $R$-band image with radio \textit{VLA} contours. The high-resolution modules are placed close to the ``center'' of the radio-bright ridge. The SL slit is oriented along the radio filament that traces the shock structure.

The right panel of Fig.~\ref{SQ_IRS_obs_Appleton06} gathers the low- and high-resolution spectra extracted in the SQ shock. These spectacular spectra are dominated by the mid-IR rotational emission of H$_2$. The 0-0 S(0) to S(5) lines are detected, plus atomic lines of [Ne$\,${\sc ii}] at $12.8\,\mu$m and [Si$\,${\sc ii}] at $34.8\,\mu$m. No PAH emission is seen\footnote{this conclusion will be revised in sect.~\ref{subsec:spectral_IRSmap_H2}. New \textit{Spitzer IRS} observations indeed show PAH emission in the ridge\protect  \citep{Cluver2009}} and the thermal dust continuum is very weak. 
This is the first time an almost pure $\rm H_2$ line spectrum has been seen in an extragalactic object. 

A two-temperatures fit of the observed H$_2$ excitation diagram reproduces the data satisfactorily and gives a rough estimation of the excitation temperatures of the gas. The warm molecular gas is constrained by the S(0)/S(1) line ratio and is consistent with $T_{\rm exc} = 185 \pm 30$~K and an H$_2$ column density of $2.06 \times 10^{20}$~cm$^{-2}$. The higher order S(3)/S(5) [ortho] transitions give $T_{\rm exc} = 675 \pm 80$~K and an H$_2$ column density of $1.54 \times 10^{18}$~cm$^{-2}$. \citet{Appleton2006} assume an ortho-to-para ratio of 3 and note no obvious deviations from this value in the data.

The SL spectroscopy shows that the H$_2$ emission is extended on the scale of 52'' (24 kpc). Assuming that the extra, undetected H$_2$ lines represent 40\% of the flux detected by \textit{Spitzer},  \citet{Appleton2006} derive an total H$_2$ luminosity of $8.4 \times 10^{33}$~W from the SH slit area ($11.3 \times 4.7$~arcsec$^{2}$).

The bottom right inset of Fig.~\ref{SQ_IRS_obs_Appleton06} shows one of the remarkable results of these observations: the H$_2$ $17\,\mu$m 0-0 S(1) line is resolved, though the relatively low resolution ($\mathcal{R} = 600$) of the \textit{IRS}. The S(1) line is extremely broad, with a FWHM linewidth of $\Delta v = 870 \pm 60$~km~s$^{-1}$. This is the broadest H$_2$ line ever observed!
The high velocity dispersion  of the warm molecular gas suggest that the postshock medium in the ridge is extremely turbulent. This is a puzzling result since H$_2$ is a fragile molecule and easily dissociated in $V_{\rm s} > 50$~km~s$^{-1}$ shocks. 

We summarize the main unexpected results from the \citet{Appleton2006} observational paper:
\begin{enumerate}
\item 
the H$_2$ gas is coexisting with a hot ($ \sim 5 \times 10^6$~K), X-ray emitting plasma.
\item 
the velocity dispersion of the H$_2$ gas seems unusually large and of the order of the velocity of the galaxy collision $\sim 900$~km~s$^{-1}$, which is of the order of the velocity of the galaxy collision.
\item
 the total H$_2$ line luminosity within the SH slit aperture exceeds that of the X-rays in this area by a factor of 3. 
\item
the spectroscopic signatures (dust or ionized gas lines) of star formation are much fainter than the $\rm H_2$ emission. This is unlike what is observed in star forming galaxies where the $\rm H_2$ lines are much weaker than the mid-IR dust features \citep{Rigopoulou2002, Higdon2006, Roussel2007}.
\end{enumerate}

\subsection{Astrophysical questions}

These surprising observations raise the following questions:
\begin{itemize}
\item Why is there H$_2$ gas is the extreme environment of the SQ postshock gas?
\item How can we account for the H$_2$ excitation characteristics?
\item Why is H$_2$ a dominant coolant?
\end{itemize}

Much of my thesis work has been driven by these astrophysical questions. 
The interpretation of H$_2$ observations presented in \citet{Guillard2009} (\hyperref[paper_SQ_H2]{paper~{\sc i}}) is based on the single-pointing observations presented above. At that time, we did not have the new spectral maps that we present in the next section.

\subsection{Mid-IR spectral mapping of the SQ shock:  H$_{\bf 2}$ spatial distribution}
\label{subsec:spectral_IRSmap_H2}

The spectacular result of \citet{Appleton2006} led us to propose new \textit{Spitzer} observations to obtain a full mid-IR spectral map of the  X-ray bright shock region. I have participated to the preparation of this proposal (P.I.: P.N. Appleton) by performing the model calculations that support it. It was accepted and observed in December 2007 and January 2008. The \textit{Spitzer IRS} mapping strategy is summarized in Fig.~\ref{SQ_IRS_MappingStrategy}. The SL and LL modules were used to map the entire shock region, the SL slits being oriented along the shock structure and the LL slits perpendicular to it.  The spectral mapping aims at spatially resolving the H$_2$ and dust across the shock.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: IRS MAPPING STRATEGY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[width=\textwidth]{figures/sq/SQ_IRS_MappingStrategy.jpg}
      \caption[\textit{Spitzer IRS} mapping strategy]{The IRS mapping strategy. \textit{Left Panel:} The SL and LL slits superimposed over the DSS image of Stephan's Quintet. The SL map covers most of the intruder galaxy NGC~7318b. \textit{Right Panel: }The same SL slit-mapping superimposed on the Chandra image of the shock. The shock is the vertical X-ray structure. NGC~7318b does not show up in the X-ray image, although the brighter of the two X-ray sources just on the right-edge of the SL region is associated with NGC~7318a.}
       \label{SQ_IRS_MappingStrategy}
\end{figure}


The new spectral maps are reported in \citet{Cluver2009} (hereafter  \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}).  We summarize here the main observational results, focusing on  the distribution and characteristics of the  H$_2$ emission in the SQ intra-group. 
The main results regarded the mapping of other mid-IR fine-structure lines are discussed later in sect.~\ref{subsec:IRSmap_fine_struct_lines}.
This \hyperref[subsec:paper_Cluver]{paper~{\sc ii}} is included in sect.~\ref{sec:publications} because it contains all the observational details and key figures to which I will make reference throughout this manuscript.

Fig.~2 of \hyperref[subsec:paper_Cluver]{paper~{\sc ii}} shows contours of the H$_2$ S(0)-S(5) line emission overlaid on an $R$-band image. The S(0) and S(1) lines were mapped by the LL modules, while S(2) - S(5) transitions were mapped by the SL modules of the \textit{IRS}. These spectral maps show an  extended emission from a giant filament  ($\sim 40$~kpc long) oriented north-south along the direction of the \textit{``main shock''}. This ``H$_2$ ridge'' spatially correlates very well with the radio or the X-ray emission. 
This provides an unambigious link between the origin of the $\rm H_2$ emission, and a large-scale high-speed shock generated by the galaxy collision between NGC~7318b and the tidal tail of NGC ~7319. We define the main shock aperture as a $\mathcal{A}_{\rm MS} = 77'' \times 30''$ rectangular aperture, corresponding to $\sim 13.7 \times  35.1$~kpc$^{2}$, centered on the coordinates $\alpha =  \rm 22h35m59.6s$, $\delta = +33$\degre$58'05.7''$. 

H$_2$ emission from the star forming region, SQ-A, as well as associated with NGC~7319 is also detected. We note that the $28.2 \, \mu$m S(0) line emission appears to be concentrated towards the SQ-A northern region. The maps also show an H$_2$ structure running eastward, from the center of the main shock to NGC~7319. We call this the \textit{``H$_2$ bridge''}, because it connects the ridge to the core of NGC~7319.  
This feature is also visible in radio,  H$\,\alpha$, and is and faintly detected in X-rays. The origin of this bridge feature is not clear, and we will come back to this point later (sect.~\ref{SQ-NGC7319-comments}). 

The spectra (see Fig.~8 of  \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}) and the  H$_2$ line fluxes (see sect.~4 and table~2) have been calculated for different apertures in the ridge (Fig.~7). 
The spectra show the striking dominance of the H$_2$ lines in the mid-IR range of the \textit{IRS}. 
The thermal dust continuum is very weak in the center of the shock and in the bridge structure, whereas it is stronger for the northern region SQ-A where star formation is likely occuring.
For the main shock structure, the 0-0S(1) line luminosity alone, the sum of the S(0) to S(5), and the total H$_2$ (accounting for $\approx 30\,$\% of the flux in undetected lines) luminosities are respectively
\begin{eqnarray}
\mathcal{L}_{\rm S(1)}({\rm H_2}) &\approx&  2.3 \times 10^{34} \ \rm W \\
\mathcal{L}_{\rm S(0)-S(5)}({\rm H_2}) &\approx&  7 \times 10^{34} \ \rm W \\
\mathcal{L}_{\rm tot.}({\rm H_2}) &\approx&  9 \times 10^{34} \ \rm W
\label{eq:H2-line-lumin-total}
\end{eqnarray}
This exceptional power in the molecular hydrogen lines is one order of magnitude brighter than the next brightest mid-IR line, [Si$\,${\sc ii}]$\lambda$34.82$\mu$m, with a line luminosity of $\mathcal{L}(\rm Si  II)  = 8.5 \times 10^{33}$~W.

The mid-IR spectral mapping  will allow us to map the excitation of the H$_2$ along and across the X-ray shock. We have started to work on a two-dimensional modelling of the H$_2$ excitation.  We will create  maps the H$_2$ excitation temperature across the shock, and correlate this with dust emission SEDs, in order to  test models we are developing to explain the extreme H$_2$ power observed. This work will be pursued during my postdoc.

\subsection{Updated mass and energy budgets for the whole ridge}
\label{subsec:mass-energ-budget}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     TABLE : MASS AND ENERGY BUDGETS FOR THE WHOLE RIDGE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{1.1} 
\begin{sidewaystable}
\begin{center}
\begin{minipage}[t]{18cm}
\renewcommand{\footnoterule}{}
\def\thefootnote{\alph{footnote}}
\small
\centering
      \caption{Mass, energy and luminosity budgets of the preshock and postshock gas in the SQ ridge\protect\footnotemark[1]. }
    \begin{tabular}{c || c c c || c c c c c}
	\hline
	\hline
		& \multicolumn{3}{c ||}{{\sc Preshock Gas}} &  \multicolumn{5}{c}{{\sc Postshock Gas}} \\
  \hline
	\hline
   & Hot Plasma\footnotemark[2] & H{\sc i}\footnotemark[4] & $\rm H_2$ &  Hot Plasma\footnotemark[2] & H{\sc ii}\footnotemark[3]  & H{\sc i}\footnotemark[4] & Warm $\rm H_2$\footnotemark[5]& Cold $\rm H_2$ \\
  $n_{\rm H}$ [cm$^{-3}$] & $3.2 \times 10^{-3}$ & & & $1.17 \times 10^{-2}$ &  & & & \\
  $T$ [K] & $5.7 \times 10^{6}$ &  & & $6.9 \times 10^{6}$ &  & & $>10^2$ & $< 10^{2}$ \\
  $P / k_{\rm B}$ [ K cm$^{-3}$] &  &  & & $1.9 \times 10^{5}$ &  &  & &   \\
   $N_{\rm H}$ [cm$^{-2}$] & & $3 \times 10^{20}$ & & & $1.4 \times 10^{19}$  & $< 5.8 \times 10^{19}$ & $2 \times 10^{20}$ & \\
  \hline
	\hline
	\multirow{2}*{Masses [$\rm M_{\odot}$]} & Hot Plasma\footnotemark[2] & H{\sc i}\footnotemark[4] & $\rm H_2$ &  Hot Plasma\footnotemark[2] & H{\sc ii}\footnotemark[3]  & H{\sc i}\footnotemark[4] & Warm $\rm H_2$\footnotemark[5]& Cold $\rm H_2$ \\
     & $ 2.4 \times 10^8 $ &  $0.8 - 2.5 \times 10^{9}$ &  &  $ 5.3 \times 10^{8}$ & $4.9 \times 10^7$ & $< 2 \times 10^8$  & $ 1.2 \times 10^9$ & \\
 \hline
	\hline
	\multirow{3}*{Energy [erg]} & \multicolumn{1}{c}{Thermal} & \multicolumn{2}{c ||}{Bulk Kinetic} & \multicolumn{2}{c}{Thermal} & \multicolumn{3}{c}{Bulk Kinetic\footnotemark[6]} \\
& \multicolumn{1}{c}{(Plasma in halo)} & \multicolumn{2}{c ||}{(Shocked H$\,${\sc i} gas)} & \multicolumn{2}{c}{(X-ray emitting plasma)} & \multicolumn{3}{c}{(Turbulent $\rm H_2$)} \\
& $3.4  \times 10^{56}$ & \multicolumn{2}{c ||}{$0.4  - 1.2 \times 10^{58}$} &  \multicolumn{2}{c}{$ 9 \times 10^{56}$} & \multicolumn{3}{c}{$\gtrsim 1.8 \times 10^{57}$} \\
	\hline
	\hline
  \multirow{2}*{Flux [W m$^{-2}$]} & \multicolumn{1}{c}{X-rays} & & & \multicolumn{1}{c}{X-rays} & \multicolumn{1}{c}{H$\, \alpha$} &   \multicolumn{1}{c}{O{\sc i}} & \multicolumn{1}{c}{H$_{2}$ \footnotemark[5]}\\
& $6.6 \times 10^{-17}$ & & & $31.4 \times 10^{-17}$ & $7.8 \times 10^{-17}$ & $5.5 \times 10^{-17}$ & $74.6 \times 10^{-17}$ \\
\hline
 \multirow{2}*{$\mathcal{L}$\footnotemark[7]  [erg s$^{-1}$]} &  \multirow{2}*{$6.2 \times 10^{40}$} &  \multicolumn{2}{c||}{} &  \multirow{2}*{$2.95 \times 10^{41}$} &  \multirow{2}*{$6.5 \times 10^{40}$} &  \multirow{2}*{$4.6 \times 10^{40}$} &  \multirow{2}*{$8 \times 10^{41}$} \\
& & & & & & & &  \\
  \hline
	\hline
    \end{tabular}
    \label{table_mass_NRJ_budgets_SQ}
\footnotetext[1]{All the numbers are scaled to our main shock aperture ($A_{\rm MS} = 70'' \times 30'' = 33.8 \times 13.2$~kpc$^{2}$) where \textit{Spitzer} mapping was performed. The preshock gas is mainly the H{\sc i} gas contained in the tidal tail of NGC~7319. After the shock, the mass is distributed between the hot X-ray emitting plasma and the  $\rm H_2$ gas (see text for details). Before the shock, most of the energy available is the kinetic energy of the H{\sc i} gas that will be shocked. The shock splits the energy budget in two parts: thermal and kinetic energy. The former is stored in the hot plasma whereas the latter goes into turbulent motions that heat the $\rm H_2$ gas. Observations show that mechanical energy is the dominant energy reservoir.}
\footnotetext[2]{\textit{Chandra} observations of the extended X-ray emission in the shock and the tidal tail \citep{O'Sullivan2009}.}
\footnotetext[3]{H$\, \alpha$ and O{\sc i} optical line observations by  \citet{Xu2003}.}
\footnotetext[4]{Based on extrapolation of H{\sc i} observations in the tidal tail by \citet{Sulentic2001, Williams2002}.}
\footnotetext[5]{From \textit{Spitzer IRS} observations. The $\rm H_2$ line flux is summed over the S(0) to S(5) lines \citep{Cluver2009}.}
\footnotetext[6]{This bulk kinetic energy is a lower limit because an unknown mass of turbulent cold molecular gas can contribute to this energy.}
\footnotetext[7]{Luminosities are indicated assuming a distance to SQ of 94~Mpc.}
\normalsize
\end{minipage}
\end{center}
\end{sidewaystable}
\renewcommand{\arraystretch}{1.0} 

In \citet{Guillard2009}, we use the multiwavelength observations to estimate the masses, thermal and mechanical energy, and luminosities in the preshock and postshock medium (see table~1 of \hyperref[paper_SQ_H2]{paper~{\sc i}}). At that time, only the single-pointing H$_2$ observations by \citet{Appleton2006} were available, so the mass and energy budgets were calculated within the \textit{IRS}  SH slit aperture. Now that we have a complete spectral mapping of the ridge, we are able to estimate the physical quantities within the full shock region. The details on how we determine the quantities from the observations are given in sect.~2.2 and 2.4 of \hyperref[paper_SQ_H2]{paper~{\sc i}}. The new results for the whole ridge are gathered in table~\ref{table_mass_NRJ_budgets_SQ}. All the quantities are estimated  within the ``main shock'' $77'' \times 30''$ aperture defined above. 

The conclusions are the same than those of \citet{Guillard2009}. In the preshock medium, the thermal energy of the hot plasma ($\frac{3}{2} \frac{M_X}{m_{\rm H}} T_X$) is only a few percent of the bulk kinetic energy of the H$\,${\sc i} gas. In the postshock medium, the main energy reservoir is the mechanical energy associated with the high-velocity dispersion of the warm H$_2$ gas. All the mechanical energy of the collision is not dissipated in the hot plasma, but a substantial amount is carried by the warm H$_2$. We show that the bulk kinetic energy of the molecular gas is $> 2$ times the thermal energy of the postshock plasma.




%Others aspects, like tidal dwarf galaxy candidates for instance, will not be discussed in details, but we provide the relevant references if the reader wants to go deeper in these areas.


\section{Astrophysical context: observational constrains}
\label{sec:SQ_context}

\subsection{Historical litterature and description of the SQ system}
\index{Stephan's Quintet!early litterature}
\index{Stephan's Quintet!population}
\index{Stephan's Quintet!description}

\begin{figure}
\begin{minipage}{\textwidth}
% \renewcommand{\footnoterule}{}
    \def\thefootnote{\alph{footnote}}
      \setlength{\footnotesep}{0pt}
   \centering
   \includegraphics[width=0.6\textwidth]{figures/sq/SQ_HST_legend.pdf}
      \caption[The main sources in Stephan's Quintet]{The main elements of Stephan's Quintet (North is up, East is left). The top panel shows a CCD image (NOAO\protect \footnotemark[1], Kitt Peak) of SQ. The five members of the quintet are: NGC~7317, NGC~7318a, NGC~7318b, NGC~7319, ans NGC~7320c. The NGC~7320 galaxy is a foreground. The bottom panel is the HST image\protect \footnotemark[2] of the center of SQ \citep{Gallagher2001}, which shows that stars are forming outside of the galactic disks of the group members, in the SQ halo. }
       \label{fig_SQ_HST_legend}
\footnotetext[1]{National Optical Astronomy Observatory, \url{http://www.noao.edu/}}
\footnotetext[2]{\url{http://hubblesite.org/newscenter/archive/releases/2001/22}}
\end{minipage}
   \end{figure}
%\protect \footnote{National Optical Astronomy Observatory, \url{http://www.noao.edu/}}
%Since its discovery \citep{Stephan1877}, the Stephan's Quintet 
%(94~Mpc) multigalaxy compact group has been extensively studied, 
%although one member of the original quintet (\object{NGC7320}) is now presumed to be a foreground dwarf galaxy and will not be discussed further here. Later studies
%have restored the ``quintet'' status with the discovery of a more distant member. The inner group galaxies are shown on the left-hand side of Fig.~\ref{Fig_picture_shocks}.



SQ was discovered in 1877 by the french astronomer Edouard Jean-Marie Stephan ($1837-1923$) at the Observatory of Marseille, France \citep{Stephan1877}. He discovered a group of four ``elliptical nebulae'', today known as SQ, much earlier than anyone knew the existence of galaxies outside the Milky Way!
When one looks at a SQ image, one actually sees 6 galaxies: NGC~7317, NGC~7318a, NGC~7318b, NGC~7319, NGC~7320 and NGC~7320c (see Fig.~\ref{fig_SQ_HST_legend}).  
So how many galaxies belong to the group, 4, 5 or 6?

The first estimates of the redshifts of the SQ members were done through optical spectroscopy, and observations show a  wide range of values among the galaxies within the group \citep{Humason1956, Ambartsumian1958, Limber1960, Burbidge1961}. 
In particular, NGC~7320 has a recession velocity of $\sim 6000$~km~s$^{-1}$ less than NGC~7317, NGC~7318a and NGC~7319 that are at $\sim 6600$~km~s$^{-1}$ (see table~\ref{table_SQmembers}). In addition, NGC~7318b and NGC~7320c have respectively ``redshift'' $\sim 900$ and $\sim 700$~km~s$^{-1}$ less than the three members at $\sim 6600$~km~s$^{-1}$.
This puzzling result was the start of a long debate about the population of Stephan's Quintet.  Do all the galaxies belong to the group? How many galaxies are in gravitational interaction?


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                         TABLE: SQ MEMBERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{landscape}
\begin{sidewaystable}
%\begin{table}
\small
\begin{center}
\begin{minipage}{\textwidth}
 \renewcommand{\footnoterule}{}
\def\thefootnote{\alph{footnote}}
 \caption[Characteristics of the galaxies lying in the Stephan's Quintet field of view]{Characteristics of the galaxies lying in the Stephan's Quintet field of view \footnotemark[1]}
\centering
\begin{tabular}{c c c c c c c }
\hline
\hline
			& NGC 7317 &	NGC 7318a &	NGC 7318b & 	NGC 7319 & NGC 7320c & NGC 7320 \\
\hline
Type \footnotemark[2] & 	 E4 &	 E2 pec &	 SB(s)bc pec &  SB(s)bc pec (Sy2  \footnotemark[6]) &	(R)SAB(s)0/a &  SA(s)d  \\
 	RA, $\alpha$ &	22 35' 51.9'' 	& 22 35' 56.8'' &	22 35' 58.5'' & 22 36' 03.7'' &	22 36' 20.4''& 22 36' 03.6s \\
 DEC, $\delta$ &	+33 56' 40.5" &	+33 57' 54.3" &	+33 57' 55.4" &	+33 58' 31.1" & +33 59' 06'' &	+33 56' 52.7" \\
Distance \footnotemark[3] & $93.3 \pm 6.5$  & $93.7 \pm 6.6 $ & $82.0 \pm 5.8 $  &	$95.4 \pm 6.7 $ & $ 84.9 \pm 5.9 $ & $ 13.7 \pm1.0$  \\
B-mag  \footnotemark[4] & 	15.3 & 14.4 & 14.06 & 14.8 & 17 & 13.8 \\
Ang. Size \footnotemark[5] & 	$0.512 \times 0.512$  &	$0.512 \times 0.512$  &	 $1.862 \times 1.348 $   &  $1.737 \times 1.348 $  & $ 0.575 \pm 0.489 $  & $2.041 \times 1.148$ \\
Velocity &  $6564 \pm 47 $ & $6597 \pm 32$ & $5727 \pm 24$ & $ 6578\pm49 $ & $ 5932 \pm 11$ & $738 \pm 48$ \\
Redshift & 	$0.02214 \pm 0.00016$ &	$0.02225 \pm 0.00011 $ &	$0.019289 \pm 0.00009 $ & $ 0.02219 \pm 0.00016$ &$ 0.019987 \pm 0.000037 $ & $0.00247 \pm 0.00016$ \\
\hline
\end{tabular}
\footnotetext[1]{Data extracted from the Simbad and NED databases. See Fig.~\ref{fig_SQ_HST_legend} for an image of SQ.}
\footnotetext[2]{Morphological type. E stands for elliptical galaxy, S for spiral.}
\footnotetext[3]{Galactocentric distance in Mpc}
\footnotetext[4]{Magnitude in the B-band ($0.83\,\mu$m)}
\footnotetext[5]{Angular size: major axis [arcmin] $\times$ minor axis [arcmin].}
\footnotetext[6]{ NGC~7319 is a Seyfert 2 galaxy showing a weak Active Galactic Nucleus (AGN) activity \citep{Durret1994a}}
\label{table_SQmembers}
\end{minipage}
\end{center}
\normalsize
\end{sidewaystable}
%\end{table}
%\end{landscape}

 \citet{Burbidge1961a} reported that the difference in redshift of $\sim 6000$~km~s$^{-1}$  between the high- and low-redshift members of SQ could only means one of two things: \textit{(i)} NGC~7320 is a foreground galaxy, or \textit{(ii)} NGC~7320 is literally exploding away from the other members. They estimated the probability of \textit{(i)} being true is $\sim 1/1500$. On the other hand, 
they stated that conclusion \textit{(ii)} ``is outside conventional ideas about the [dynamics] of galaxy groups''.
\citet{Arp1973} reports the first H$\alpha$ interference filter images of SQ. These images clearly separate the low- and high-redshifts systems, associated with the foreground galaxy NGC~7320 ($\sim 800$~km~s$^{-1}$) and the SQ group ($\sim 6000$~km~s$^{-1}$).
Based on the analysis of the distribution and diameters of the H$\,${\sc ii} regions, \citet{Arp1973, Arp1976} argued that NGC~7320 is physically associated with other SQ galaxies, and this was a prime case for the existence of non-Dopler redshift.

 \citet{Tammann1970, Allen1980, Moles1997} provided counter arguments against this claim. First, H$\,${\sc i} and H$\alpha$ observations show no evidence for NGC~7320 interaction with other SQ galaxies. Second, redshift independent estimates yield
to distances consistent with the redshifts. Third, the redshift of NGC~7320  is close to that of NGC~7331 ($818 \pm 5$~km~s$^{-1}$), so NGC~7320 appear to be a member of a foreground loose galaxy group which includes the large spiral galaxy NGC 7331. 
In the following, we thus assume that NGC~7320 is a foreground galaxy and it will not be further discussed hereafter.
 \citet{Arp1973a} suggested that NGC~7320c, the galaxy lying 4~arcmin to the
east of NGC 7319 (see Fig.~\ref{fig_SQ_HST_legend}, top panel) is linked to the group by optical tidal tails. Therefore the ``quintet'' status is restored!

In the bottom panel of Fig.~\ref{fig_SQ_HST_legend} we show a recent mosaic picture  taken by  \citet{Gallagher2001} with the Wide Field and Planetary Camera 2 (WFPC2) onboard the \textit{Hubble Space Telescope} (\textit{HST}), on Dec. 30, 1998 and June 17, 1999. One clearly sees on the image that galaxy interactions have distorted the galaxies' shapes, creating elongated spiral arms and long, gaseous streamers. Interestingly, this spectacular image reveals that star clusters are forming outside the galactic disks, in the SQ halo. Some of these star cluster contain a few millions of stars.

In the following, we assume the distance to the SQ group to be 94~Mpc (with a Hubble constant of 70 km~s$^{-1}$~Mpc$^{-2}$) and a systemic velocity for the group as a whole of $6\,600$~km~s$^{-1}$. At this distance, 10~arcsec$=4.56\,$kpc.

\subsection{The complex dynamical history of Stephan's Quintet}
\index{Stephan's Quintet!dynamical history}


\begin{figure}
   \centering
    \includegraphics[width=\textwidth]{figures/sq/SQ_Palomar_Arp1973_tails.pdf}
      \caption[Tidal tails in Stephan's Quintet]{Iso-density image of an optical photographic plate (3h of observations) taken with the 200-inch telescope at Palomar \citep{Arp1973a}. We identify the members of the Stephan's Quintet group and the two tidail tails. Recent measurements of redshifts are indicated.}
       \label{fig_SQ_Palomar_Arp1973_tails}
   \end{figure}
  

The first deep optical images taken by  \citet{Arp1972, Arp1973a, Arp1976} show
 two concentrating parallel tidal tails, both starting from NGC~7319 and extending to
NGC~7320c, with the more diffuse one passing through the low redshift galaxy NGC 7320. Fig.~\ref{fig_SQ_Palomar_Arp1973_tails} presents an example of a photographic plate taken at the 200-inch Palomar telescope, where these two tidal tails are clearly visible. This is the first indication of a long list of observations that show that the group has a complex dynamical history.

As its population, the dynamical history of SQ has been a long debate that is not entirely solved yet. In the following, we first summarize the scenario of past and present dynamical interactions  that emerges from  multi-wavelengths observations. Then we detail the different arguments that support it, and we point out the remaining uncertainties.

\subsubsection{Summary of the scenario: multiple galaxy collisions}

In the past, an ``old intruder'', NGC~7320c, stripped most of the gas from group members (essentially NGC~7319 and NGC~7318a), and a new intruder, NGC~7318b is currently colliding with this gas and triggering a large scale shock. The old
intruder passed the core of SQ twice, first $\sim 5 - 7 \times 10^8$~yrs ago and creating the ``old tail'' (the southern tail in  Fig.~\ref{fig_SQ_Palomar_Arp1973_tails}), and second  about $2 \times 10^8$~yrs ago, triggering the ``young tail'' (the narrower one in Fig.~\ref{fig_SQ_Palomar_Arp1973_tails}).

\subsubsection{Observational constrains on past interactions with NGC~7320c}

The ``two-intruders'' scenario summarized above was clearly formulated by  \citet{Moles1997} and further confirmed by \citet{Sulentic2001}, who discussed in detail the link between the two tidal tails and the two passages of NGC~7320c through the kernel of the group. 

The \textit{HST} image (Fig.~\ref{fig_SQ_HST_legend}) highlights that star birth occurs mainly in three dynamically-perturbed sub-regions of the group: the long, sweeping tail and spiral arms of NGC 7319 [left]; the gaseous debris of the galaxy pair NGC~7318a and b [bottom right]; and an area north of those galaxies, the so-called SQ-A starburst region [top right]. Since galaxy interactions are known to trigger star formation (see sect.~\ref{subsec:SFgal_interactions}), the SQ star formation history is closely linked to its dynamical history. Photometric analysis of the \textit{HST} images shows that the ages of these star clusters span over a wide range, spanning from $\sim 2 \times 10^{6}$~yrs to $\sim 3 \times 10^{9}$~yrs, which shows past and recent star formation \citep{Gallagher2001}. 
The southern, diffuse tail mostly contains an old population of star clusters, whereas the northern one is comprised of younger stars.

X-ray observations also support multiple episods of galaxy interaction in the SQ group. A very extended halo of hot ($\sim 6 \times 10^6$~K) gas was first detected by \citet{Bahcall1984}. They state that the extent of the halo is too big and its temperature too low to have been produced by the collision of the new intruder. 
They also show that the X-ray luminosity of the halo ($\mathcal{L}_X(0.1-3\rm \ keV) = 5 \times 10^{42}$~erg~s$^{-1}$) is 10 times the expected luminosity from the combined five SQ galaxies. 
Later, \citet{Moles1997, Sulentic2001, O'Sullivan2009} suggest that this X-ray emitting hot intracluster gas  was produced by previous galaxy encounters (with NGC~7320c for instance). We will further discuss X-ray observations in sect.~\ref{subsec:obs_galaxy-wide_shock}.

\subsubsection{The discovery of a galaxy-wide shock in Stephan's Quintet}

The first evidence for the recent collision between the intruder NGC~7318b and the IGM comes from two discoveries in the radio band, both made with the Westerbork Synthesis Telescope, Netherlands.

The first is a giant ($\sim 40$~kpc long) radio continuum ridge found in the IGM between NGC 7319 and NGC 7318b \citep{Allen1972}. Among other possible interpretations, \citet{Allen1972} suggested this may be a large scale shock triggered by an on-going collision between NGC 7318b (the recent intruder) and the rest of the group. The collision velocity is about one million mph (1000~km~s$^{-1}$)! A one hundred thousand light-year long giant shock is produced!  Stephan's Quintet is thus a multi-galaxy collision caught in action!

The second \citep{Allen1980, Shostak1984} is the revelation that nearly all the H$\,${\sc i} gas associated with SQ is lying outside galaxy disks, in the group halo. This represents a mass of neutral gas of $\sim 10^{10}$~M$_{\odot}$. These observations suggest that this gas has been stripped from late type galaxy disks due to an earlier interaction (a few $10^8$ yr ago) either between NGC~7319 and NGC~7318a \citep{Allen1980}, or between NGC 7319 and NGC 7320c \citep{Shostak1984}. In sect.~\ref{subsec:obs_galaxy-wide_shock} we discuss more recent observations of the radio-emitting ridge.

\subsubsection{Ongoing debate about the origin of the ``young'' tidal tail}

If most of the litterature now agrees on the origins of the old tail and of the main shock, the origin of the ``young tail'' is more debated. Instead of the ``two step'' scenario proposed by \citet{Moles1997, Sulentic2001}, \citet{Xu2005}
proposed a ``three-intruders'' scenario based on new UV observations.

They argue that it is unlikely that the young tail is also triggered by NGC 7320c. This is
because the recently measured redshift of NGC~7320c \citep[6583~km~s$^{-1}$][]{Sulentic2001} is almost identical
to that of NGC 7319, indicating a slow passage \citep{Sulentic2001} rather than a fast passage \citep[$\sim 700$~km~s$^{-1}$][]{Moles1997}. In order for NGC~7320c to move to its current position, the NGC 7319/7320c
encounter must have occurred $\gtrsim 5 \times 10^8$~yr ago. This is close to the age of the old tail, but older than that of the young tail. They suggested that the young tail is triggered by a close
encounter between the elliptical galaxy NGC~7318a and NGC~7319. The projected distance
between NGC~7318a/7319 is only $\sim 1/3$ of that between NGC~7320c/7319. Therefore the time
argument is in favor of the new scenario. 

Numerical N-body simulations are certainly needed to explore and test the dynamical scenarii inferred from observations. Recent work within the specific context of SQ has been made by \citet{Renaud2007}, and has to be pursued. We will not further discussed this debate and shall concentrate on the main shock. 

\subsection{Further evidence for a galaxy-wide shock}
\label{subsec:obs_galaxy-wide_shock}
\index{Stephan's Quintet!galaxy-wide shock}

In the following we further discuss multi-wavelength observations of Stephan's Quintet. These data sets allow to establish the energy and mass budget of the SQ galaxy collision, which is gathered in the Table~1 of \citet{Guillard2009} (\hyperref[paper_SQ_H2]{paper I}).

\subsubsection{Radio observations}
\label{subsubsec:SQ-radio-observations}
\index{Stephan's Quintet!radio observations}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         FIGURE: VLA RADIO ONSERVATIONS OF SQ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
   \includegraphics[width=0.49\textwidth]{figures/sq/SQ_radio_continuum_Williams02.jpg}
  \includegraphics[width=0.49\textwidth]{figures/sq/SQ_radio_continuum_Xu03_4GHz.jpg}
      \caption[VLA radio continuum observations of Stephan's Quintet]{Radio continuum observations of  SQ. \textit{(Left):} Contour map of the 21 cm continuum emission at 1.4~GHz overlaid on an R-band image obtained by J. Sulentic at the 3.5 m Calar Alto telescope. The contours are $-0.2$, 0.2, 0.4, 0.8, 1.6, 3.2, 6.4, 13, and 26 mJy beam$^{-1}$, for an rms noise level of 0.1~mJy beam$^{-1}$ (0.3~K). The synthesized beam, $15.4'' \times 14.8''$, is shown on the upper left corner. Coordinate offsets are with respect to the optical nucleus of NGC 7319 at $\alpha_{\rm J 2000}$ 22 36' 03.7'', $\delta_{\rm J 2000}$ +33 58' 31.1". From \citet{Williams2002}. \textit{(Right):}   Contours of the radio continuum at 4.86 GHz (VLA B configuration) overlaid on an R-band CCD image \citep[from][]{Xu2003}. The lowest contour is 50 $\mu$Jy~beam$^{-1}$, and the spacing is equal to 2 in ratio. The FWHM of the synthesized beam is 6''.}
       \label{fig_SQ_Xrays_radio_contours}
   \end{figure}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         FIGURE: GMRT RADIO ONSERVATIONS OF SQ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
   \includegraphics[width=\textwidth]{figures/sq/SQ_radio_GMRT_OSullivan2009.jpg}
      \caption[GMRT radio observations of Stephan's Quintet]{GMRT low-frequency observations of SQ by \citet{O'Sullivan2009a}.\textit{ Left:} 327 MHz GMRT contours overlaid on POSS blue image
of the core of Stephan's Quintet. Contours start from $3 \sigma = 0.9$~mJy~beam$^{-1}$,
HPBW (Half Power Beam Width) is $12'' \times 10''$. \textit{Center: } 610 MHz GMRT contours overlaid on a Swift UVOT UVW2-band image ($\sim \! 200$~nm). \textit{Right:} $1400-610$ MHz spectral index map (HPBW of $6''\times 5''$) with 610 MHz contours overlaid.}
       \label{fig_SQ_radio_GMRT_OSullivan2009}
   \end{figure}
  

The galaxy-wide radio ridge discovered by \citet{Allen1980}  has been confirmed
by  VLA\footnote{Very Large Array \url{http://www.vla.nrao.edu/}} observations by \citet{VanDerHulst1981, Williams2002, Xu2003}. Fig.~\ref{fig_SQ_Xrays_radio_contours} presents radio observations of SQ at 1.416 and 4.86~GHz. 
\citet{O'Sullivan2009a} extend these observations to lower frequencies (327 and 610~MHz) with the GMRT telescope. Fig.~\ref{fig_SQ_radio_GMRT_OSullivan2009} shows \textit{GMRT} radio contours overlaid on optical and UV images of the group core, and on a $1400-610$~MHz spectral index map. 
We summarize the main results:
\begin{itemize}
\item there is a bright north-south linear ridge of radio emission running in between NGC~7319 and NGC~7318b.  The diffuse radio emission is more extended at lower frequencies, including areas
west of the ridge. The 1.4~GHz image shows that faint emission connects this extended ridge to NGC~7319.
A faint extension to the northwest, coinciding with H$\alpha$ emission \citep{Plana1999, Sulentic2001}, is also detected.
The  total flux density associated with the extended radio ridge is $48 \pm 7$~mJy \citep{Williams2002}. 
\item  The spectral index map shows that the southern part of the
ridge has an index of $0.7-0.8$, while the northern part has a steeper spectrum \citep{O'Sullivan2009a}.
Some of the brightest spots of radio emission corresponds with knots of UV emission in the
south-eastern spiral arm of NGC 7318b. In this region the spectral index is consistent with star formation, so the underlying extended radio emission arising from shocks may be  enhanced by star formation in some areas.
\item the core of the Seyfert 2 NGC~7319 shows a radio source with a flux $28.5 \pm 0.5$~mJy. Both images also show that there is a radio source associated with the nucleus of NGC~7318a \citep[$0.95 \pm 0.05$~mJy][]{Xu2003}.
\item note that the bright source lying to the north of SQ-A is a backgroung distant binary source seen in projection behind SQ \citep{VanDerHulst1981, Williams2002}. 
\end{itemize}

The total luminosity emitted by the radio ridge at 1.4~GHz is $\mathcal{L}_{\rm1.4GHz} \sim 4 \times 10^{31}$~W from a volume extending about $90'' \times 15''$. 
This luminosity is 10 times the radio-luminosity of all star-forming regions in SQ (NGC~7318a, SQ-A, and a possible non-AGN component from 7319). \citet{VanDerHulst1981} proposed that the radio emission in the ridge is produced by an intra-cluster starburst. This would imply a star-formation rate of $\sim 30$~M$_{\odot}$~yr$^{-1}$, which is uncompatible with optical spectroscopy, H$\alpha$ imaging, or mid-IR observations (see chapter~\ref{chapter:SQ_dust}).

The radio ridge must be associated with synchrotron emission of relativistic electron accelerated in the giant shock created by the NGC~7318b galaxy that is entering into NGC~7319's tidal tail.
The ridge is the interface between the interloper NGC~7318b and the group. Indeed, the shocked, ionized gas is predicted to produce significant amounts of synchrotron emission \citep{VanDerHulst1981, Allen1972}. The synchrotron life time for the radiating electrons is estimated to be rather short, a few times $10^7$~yr, which is comparable to the crossing time for the collision.

Assuming the equipartition of energy between gas internal energy, cosmic rays and magnetic energy, \citet{Xu2003} estimate the magnetic field strength to be $B_{\rm eq} \simeq 10\,\mu$G.
The corresponding energy density of relativistic particles plus the magnetic fields is $\mathcal{U}_{\rm min} \sim 10^{11}$~erg~cm$^{-3}$. This is significantly lower than the thermal energy density implied by X-ray observations (see below). 

\subsubsection{Kinematics of the H$\,${\sc i} gas}
\index{Stephan's Quintet!H$\,${\sc i} observations}
\label{subsubsec:SQ_HI_kinematics}

 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         FIGURE: HI CONTOURS OF SQ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[width=\textwidth]{figures/sq/SQ_HI_contours_Sulentic.pdf}
      \caption[H$\,${\sc i} gas in Stephan's Quintet ]{H$\,${\sc i} 21 cm radio contours superposed on H$\alpha$ interference filter images. \textit{Left:} H{\sc i} contours for velocities in the SQ range $6475-6755$ km~s$^{-1}$. \textit{Right:} H{\sc i} contours for velocities in the new intruder range ($5597-6068$ km s$^{-1}$). H{\sc i} contours levels correspond to [0.526, 1.58, 2.63, 5.26, 7.89]$\times 10^{20}$~cm$^{-2}$ with last contour shown only in the left panel. Adapted from \citet{Sulentic2001}.}
       \label{fig_SQ_HI_contours_Sulentic}
   \end{figure}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         FIGURE:  SQ HI VELOCITY MAPS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[width=\textwidth]{figures/sq/SQ_velocity_maps.png}
      \caption[H$\,${\sc i} velocity maps in Stephan's Quintet]{The of H$\,${\sc i} column density contours and first-order moment of the radial velocity (lines and numbers in km~s$^{-1}$) for low (cyan and blue), intermediate (green
and orange) and high (red and black) velocity ranges. The galaxies velocities are from \citet{Sulentic2001}. This image is taken from \citet{Renaud2007}.}
       \label{fig_SQ_velocity_maps}
   \end{figure}


Fig.~\ref{fig_SQ_HI_contours_Sulentic} shows 21~cm observations of the H$\,${\sc i} line at two velocities, that of the intruding galaxy, $\sim 5700$~km~s$^{-1}$, and that of NGC~7319, $\sim 6700$~km~s$^{-1}$. 
The H$\,${\sc i} contours are overlaid on H$\alpha$ interference filter images centered at the intruder and intra-group velocities. 
These images will be discussed later, in sect.~\ref{subsec:opticallineemission_shocks}.
On Fig.~\ref{fig_SQ_velocity_maps}, the H$\,${\sc i} contours are overlaid  on an optical R-image. In colors we show the radial velocities of the gas. 
H{\sc i} observations exhibit a large stream created by tidal interactions between NGC~7320c, and NGC~7319 \citep{Moles1997, Sulentic2001}.  This stream corresponds to the ``old tidal tail'' (see Fig.~\ref{fig_SQ_Palomar_Arp1973_tails}) and the velocity of the gas in the tail is $6600 - 6700$~km~s$^{-1}$. No H$\,${\sc i} gas is detected in the younger tail. 
The SQ-A starburst region both contains H$\,${\sc i} gas at the intragroup (tidal tail) velocity ($\sim 6600$~km~s$^{-1}$) and at a velocity slightly higher that the intruder velocity ($\sim 6000$~km~s$^{-1}$), which suggests that this gas was accelerated by the shock.
Some H$\,${\sc i} gas associated with the intruder velocity ($\sim 5700$~km~s$^{-1}$) is detected to the south of NGC~7318a/b. 

The observed difference in radial velocities between the H$\,${\sc i} tidal tail and the intruder is about $1\,000$~km~s$^{-1}$. 
On Fig.~\ref{fig_SQ_HI_contours_Sulentic}, the 21~cm contours are overlaid on an H$\,\alpha$ Fabry-Pérot image. At the velocity of the intra-group medium, the H$\,\alpha$ image (left panel) clearly shows the linear feature associated with the shock.  Over the shock region, no H$\,${\sc i} gas is detected, but optical line emission from H$\,${\sc ii} gas is observed at
the H$\,${\sc i} tidal tail velocity. This suggests that \textit{the H$\,${\sc i} gas  present in the ridge before the recent galaxy collision was ionized  by the shock induced by the collision between the two gas flows}. It is likely that the H$\,${\sc i} gas at $\sim 6600$~km~s$^{-1}$ in SQ-A was physically connected to the   H$\,${\sc i}  tail.
We infer the preshock H$\,${\sc i} gas masses based on the $\,${\sc i} column densities observed on both sides of the ridge (see \hyperref[paper_SQ_H2]{paper I}). 

\subsubsection{X-ray observations}
\label{subsubsec:Xray_obs_SQ}
\index{Stephan's Quintet!X-ray observations}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%           FIGURE: X-RAY  IMAGES OF SQ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
   \includegraphics[width=0.51\textwidth]{figures/sq/SQ_CFHT_Xray_label.jpg}
   % \includegraphics[width=0.48\textwidth]{figures/sq/SQ_Xrays.png}
     \includegraphics[width=0.48\textwidth]{figures/sq/SQ_Xrays_contours.png}
      \caption[Chandra X-ray observations of Stephan's Quintet]{Chandra X-ray observations of SQ \textit{(Left)}: $0.3-2.0$~keV image (curved, light blue ridge running down the center of the image) overlaid on a deep CFHT image. \textit{(Right):} A zoomed X-ray contour map ($0.5-3$ keV) of the main concentration of X-ray photons \citep[from][]{Trinchieri2003}. Contours are superimposed on a CFHT B-band image of the field. The X-ray data are smoothed with an adaptive filter (FFT method) and 2.5$\, \sigma$ as the lowest significance of the signal within the kernel. 
% \textit{(Right): zoomed and smoothed \textit{Chandra} $0.3-2.0$~keV image (blue)} overlaid on  an optical Palomar DSS image.
}
       \label{fig_SQ_CFHT_Xray}
   \end{figure}

The first X-ray observations of SQ were performed with the \textit{Einstein Observatory} and were reported by \citet{Bahcall1984}. They found an extended halo but the spatial resolution was not high enough to resolve the structure of the ridge. 
The presence of shock-heated gas in the SQ halo was confirmed by X-ray \textit{ROSAT}, \textit{Chandra} and \textit{XMM} observations. 
X-ray maps \citep{Pietsch1997, Sulentic2001} revealed an extended and diffuse hot halo, plus features  associated with the radio ridge and with galaxy members of the group. 
The extent of the underlying X-ray emitting halo is too big to have been produced by the new interaction of NGC~7318b with the tidal tail, strongly suggesting that it must have been heated during previous dynamical encounters \citep{Moles1997, Sulentic2001, O'Sullivan2009}.
One third of the total X-ray luminosity, $\mathcal{L}_{X} = 5 \times 10^{41}$~erg~s$^{-1}$, is associated with the intergalactic ridge. The comparison of the relative structures in radio and X-ray bands (Fig.~\ref{fig_SQ_Xrays_radio_contours} and \ref{fig_SQ_CFHT_Xray}) show that the X-ray emission is brightest in the northern part of the ridge, while the radio emission is brightest in the south.


High spatial resolution maps \citep{Trinchieri2003, Trinchieri2005, O'Sullivan2009} and optical narrow-band H$\alpha$/[N$\,$II] maps \citep{Vilchez1998, Ohyama1998, Xu1999, Plana1999, Sulentic2001} show a similar structure, in both the hot gas and the ionized gas. The left panel of Fig.~\ref{fig_SQ_CFHT_Xray} shows a spectacular \textit{Chandra} image (blue) overlaid on an optical CFHT image.The right panel shows a zoomed gray-scale B-band image overlaid with \textit{Chandra} $0.5 - 3$~keV iso-contours. 

The width of the radio or X-ray emission in the shock is $\sim 5$~kpc, which is commensurate with the width of the H$\, \alpha$ ridge. Dividing the width of the ridge by the collision velocity (assumed to be $1\,000$~km~s$^{-1}$), we get a collision age of the order of $t_{\rm coll} \sim 5 \times 10^{6} \,$yr.

Spectral energy distribution fitting of \emph{Chandra} and \emph{XMM} observations of SQ show that the temperature of the hot plasma in the ridge is $T_{\rm X} = 6.9 \times 10^{6} \,$K \citep{Trinchieri2003, Trinchieri2005, O'Sullivan2009}. 
The postshock temperature for a perpendicular shock is given by \citep[see e.g.][]{1993ARA&A..31..373D}:
\begin{equation}
\label{eq_postshock_temp_norm}
T_{\rm ps} = \frac{2(\gamma - 1)}{(\gamma + 1)^{2}} \, \frac{\mu}{k_{\rm B}} \, V_{\rm s}^{2} \simeq 6.94 \times 10^6 \, \left( \frac{V_{\rm s}}{715 \ \rm km \, s^{-1}}\right) ^{2} \ \ \rm K \; ,
\end{equation}
where $V_{\rm s}$ is the velocity of the shock wave, $\mu$ the mean particle mass (equals to $10^{-24}$~g for a fully ionized gas), $k_B$ the Boltzmann constant and $\gamma = 5/3$. Therefore, the postshock temperature of the hot plasma allows us to estimate a shock velocity of $\sim 700$~km~s$^{-1}$. 
We expect  the shock velocity to be equal to the gas velocity in the center of mass frame. 
If the volume-averaged gas densities are the same on the intruder side and on the side of the tidal tail  (see sect.~\ref{subsubsec:SQ_HI_kinematics} for details), the shock velocity would be approximately half of the observed relative velocity, so $1000 / 2 = 500$~km~s$^{-1}$. This is significantly lower than the shock velocity we deduce from X-ray observations, suggesting that the mass of the gas in the intruding galaxy is higher than in the tidal tail.

The fact that the shock velocity agrees with the line-of-sight relative velocity of the intruder suggests that its transverse velocity component is small. \citet{Sulentic2001} also argue that the distribution of the H$\,${\sc i} and H$\,${\sc ii} emissions support the idea of an ongoing collision of NGC~7318b with the tidail tail almost parallel to the line of sight. This conclusion has been revised by \citet{Trinchieri2003, O'Sullivan2009} who argued for an oblique shock geometry. They find that the temperature in the ridge ($6.9 \times 10^{6} \,$K) is close to that of the underlying hot halo ($5.7 \times 10^{6} \,$K). As they are assuming a shock velocity of $900-1000$~km~s$^{-1}$, they conclude that the temperature in the ridge is too low. The hypothesis of an oblique shock may help to decrease the main shock velocity and therefore the postshock temperature.  This will be further discussed in sect.~\ref{subsec:route2H2formationscenario}.

The only sign for any interaction between NGC 7317 with other members of SQ is a common
halo linking it to the binary NGC 7318, found in the deep X-ray and optical R-band images
\citep{Trinchieri2005}.


\section{How does H$_{\bf 2}$ form in the Stephan's Quintet giant shock?}
\label{sec:H2formation_SQ}

In this section we focus on the first out of our three astrophysical questions: the formation of H$_2$ in the SQ ridge. We introduce the scenario presented in \citet{Guillard2009}  (\hyperref[paper_SQ_H2]{paper~{\sc i}}).  I will first show that we have explored several working hypothesis before coming to this scenario. Obviously, our scenario may not be the right solution, but, to our knowledge, this is the first quantitative model that attempt to explain the H$_2$ formation and emission within the broader context of multi-wavelength observations of SQ. Up to now, it has not been invalidated by observations.

\subsection{A long route to a coherent scenario\dots}
\label{subsec:route2H2formationscenario}

The main difficulty in understanding the presence of H$_2$ in the SQ shock is to explain how the gas can cool and become molecular in a hot plasma, and how it can survive in such a violent environment. Inspired by previous studies, \citet{Appleton2006} evoke two possibilities: \textit{(i)} an \textit{oblique} shock geometry, and \textit{(ii)}, the presence of \textit{dust} in the hot plasma. Both ingredients will help diminishing the gas temperature and make its cooling easier to form H$_2$ within the age of the collision. These hypothesis may also explain why the gas temperature in the ridge is not much hotter than that of the underlying halo \citep[see sect.~\ref{subsubsec:Xray_obs_SQ} and][]{Trinchieri2003, Xu2003, O'Sullivan2009}.
However, these ingredients alone are not sufficient enough to explain the coexistence of warm molecular gas with a hot plasma. I will show that the multiphasic nature of the shocked gas is a key to interpret  multi-wavelength observations of SQ. 

\subsubsection{An oblique shock geometry?}
\index{Stephan's Quintet!oblique shock}

The collision between the new intruder, NGC~7318b, and the intra-group tidal tail is not necessarily head-on.
The shock associated with this collision may be oblique, i.e. the upstream fluid crosses the shock front with an incident angle $\phi \neq 90$\degre (see sect.~\ref{subsec:oblique_shocks} for a physical description of oblique shocks). 
This hypothesis is considered by \citet{Trinchieri2003, O'Sullivan2009} to explain with there is so little difference between the gas temperature in the radio ridge ($6.9 \times 10^6$~K) and outside, in the halo ($5.7 \times 10^6$~K). \citet{Trinchieri2003, O'Sullivan2009} assume a shock velocity equal to the relative line-of-sight velocity between the new intruder and NGC~7319's tidal tail ($900-1000$~km~s$^{-1}$). In the case of a perpendicular shock, a $1000$~km~s$^{-1}$ shock would lead to a post shock temperature of $\sim 1.4\times 10^7$~K (see Eq.~\ref{eq_postshock_temp_norm}), which is twice the temperature derived from X-ray observations in the ridge. If the incoming flow forms an angle $\phi$ with the shock surface, then the shock velocity is reduced by a factor $\sin \phi$. In this case, the postshock temperature can be written as
\begin{equation}
\label{eq_postshock_temp_oblique}
T_{\rm ps} = \frac{2(\gamma - 1)}{(\gamma + 1)^{2}} \, \frac{\mu}{k_{\rm B}} \, V_{\rm s}^{2} \sin ^2 \phi  \simeq 6.9 \times 10^6 \, \left( \frac{V_{\rm s}}{1000 \ \rm km \, s^{-1}}\right) ^{2} \sin ^2 \left( \frac{\phi }{30^{\circ}} \right) \ \ \rm K \; ,
\end{equation}
where $V_{\rm s}$ is the velocity of the shock wave, $\mu$ the mean particle mass (equals to $10^{-24}$~g for a fully ionized gas), $k_B$ the Boltzmann constant and $\gamma = 5/3$. 
Therefore, an incidence of $\phi \sim 30$\degre would be required to match the observed temperature of the hot gas in the ridge. 

The possibility that the large-scale shock is oblique may be an argument to reduce the X-ray power with respect to the more luminous H$_2$ emission in the ridge. However, it does not explain why part of the gas has cooled down  efficiently to form H$_2$, and part of the gas is still hot and emits X-rays. 

\subsubsection{A significant cooling of the hot gas by the dust?}

Based on \textit{ISO} IR observations, \citet{Xu2003} suggest that dust grains are the main coolant of the hot gas, which produce FIR emission. After subtraction of the IR emission from the individual sources in the group, they  detect a residual IR emission from the shock. The IR emission is extended, its morphology is similar to the radio emission in the ridge, and is one order of magnitude more luminous than the X-ray emission. They interpret this IR emission by collisional heating of dust grains by the hot electrons and ions of the plasma. Assuming a constant dust-to-gas mass ratio of $6 \times 10^{-3}$, they estimate a cooling time scale of $t_{\rm cool} \sim 2 \times 10^6$~yr, which is two orders of magnitude shorter than if the plasma is dust-free (see sect.~\ref{sec:gascooling_therm_instability}). They use the collisional heating model of \citet{Popescu2000} and find that the expected FIR luminosity is in agreement with observations.


The problem is that the cooling timescale is so short that we should observe cool gas around the shock, which is not seen on the X-ray temperature maps \citep{O'Sullivan2009}. This scenario has difficulties to explain why we observed both a diffuse hot ($6-7 \times 10^6$~K) component in the ridge and in its outskirts, and warm ($100-1000$~K) molecular gas.
In fact, at the beginning of our study, we started to work in the direction of  \citet{Xu2003} to explain the cooling of the gas by the dust grains in the ridge. This is why I decided to carry on a detailed  calculation of the time-dependant cooling of the hot gas, taking into account dust destruction. This modeling has been presented in sect.~\ref{subsec:time-dependent-cooling-gas} and in \hyperref[paper_SQ_H2]{paper~{\sc i}}. The results lead us to revise the conclusions of \citet{Xu2003}, and we discuss the application of this modeling to the case of SQ in  sect.~\ref{subsubsec:gas-cooling-dust-survival-H2-formation}.

We find that the cooling timescale of the hot gas in the ridge is more than one order of magnitude longer than the shock age. We conclude that it is very unlikely that the H$_2$ gas results from the direct cooling of the hot gas. 
This result has driven us to the idea that, if the H$_2$ formation was induced by the galaxy collision, it must have cooled down from much lower temperatures. Then the gas in the ridge must have been shocked by a wide distribution of shock velocities, a thus of postshock temperatures. This is how we came to consider that the preshock medium was inhomogeneous. 
In the following, we present our scenario for H$_2$ formation. New IR observations and modeling of the dust emission in the SQ shock within the framework of this scenario will be discussed in chapter~\ref{chapter:SQ_dust}. 

\subsection{H$_2$ formation out of multiphase postshock gas}
\label{subsec:SQ-H2formation-multiphase-gas}

The difficulties evoked above suggest that it is very difficult to explain H$_2$ formation from homogeneous shocked gas at high-speed. In our view, the presence of H$_2$ in the SQ ridge is closely related to the multiphase structure of the preshock gas and may result from two possibilities:
\begin{enumerate}
\item molecular clouds are present in the preshock gas and embedded within the pre-existing halo of hot gas. Because of the density contrast between the tenous gas and the clouds, slower shocks are driven into 
the clouds (see sect.~\ref{sec:shocksinmultiphasemedia}), and H$_2$ molecules may or may not be dissociated, depending on the shock velocity. If the shock transmitted into the cloud is dissociative,
H$_2$ molecules may reform in the postshock medium \citep[see sect.~\ref{sec:MHD_shocks} and][]{Hollenbach1979}.
If gravitationally bound molecular clouds are present in the preshock medium, we expect the shock to trigger their collapse, which would lead to star formation \citep{Jog1992}. 
This process is perhaps what is happenning in the northern region of the shock, SQ-A, where optical and IR imaging show that a starburst is occuring \citep{Xu1999}.
% The starburst may be induced by the collision of the new intruder with the IGM. However, the triggering mechanism and the presence of preshoc GMCs are unclear. 

The weakness of tracers of star formation in the region of the main shock \citep{Xu2003} suggests that preshock GMCs are not a major source of the observed postshock H$_2$ gas in the ridge. 
Although we do not exclude pre-existing molecular gas in the ridge, we explore the following second possibility.

\item

H$_2$ gas forms out of preshock H$\,${\sc i} gas. \citet{Appleton2006} also evoke this scenario by proposing that a large-scale shock overruns a clumpy preshock medium. H$_2$ molecules would form in the denser regions that experience slower shocks compared with the high-speed shock in the tenuous gas. 
In the following we summarize and complete the results presented in our  \hyperref[paper_SQ_H2]{paper~{\sc i}}.
\end{enumerate}
 
\subsubsection{Supersonic collision between two inhomogeneous gas streams} 

Multiwavelength observations of SQ suggest that two multiphase gas flows are colliding (see sect.~\ref{subsec:obs_galaxy-wide_shock}). One stream is associated with the intruding galaxy (NGC~7318b), and the other is associated with the tidal tail of NGC~7319. Both gas streams are likely to contain hot (a few million K), H$\,${\sc i} and perhaps molecular clouds. Therefore we consider the collision of two flows of multiphase dusty gas. 
The relative velocity between the flow is $900-1000$~km~s$^{-1}$, constrained by H$\,${\sc i} observations and optical line spectroscopy. 
Our model quantifies the gas cooling, dust destruction, and H$_{2}$ formation in the postshock medium within this framework.



If the colliding gas flows are inhomogeneous, the rise of pressure in the hot, tenuous gas drives slower shocks into the denser clouds (see sect.~\ref{sec:shocksinmultiphasemedia}).
Each cloud density corresponds to a shock velocity. 
The galaxy collision generates a range of shock velocities and postshock gas temperatures. The state of the postshock gas is related to the preshock gas density. Schematically, low density (preshock at $n_{\rm H} \lesssim 3 \times 10^{-3}\,$cm$^{-3}$) gas is shocked at high speed ($\gtrsim~700\,$km~s$^{-1}$) and accounts for the X-ray emission. Denser H$\,${\sc i} gas ($n_{\rm H}  \gtrsim \times 10^{-2}$) is heated to lower ($ \lesssim10^6$~K) temperatures. 
The fig.~1 of \hyperref[paper_SQ_H2]{paper~{\sc i}} sketches this scenario. The rise of pressure in the hot gas triggers the compression of the H$\,${\sc i} clouds that are the sites for H$_2$ formation.

In the following we compute the isobaric cooling, the evolution of the dust-to-gas mass ratio, and the formation of molecules in this multi-temperature postshock gas (see sect.~\ref{subsec:time-dependent-cooling-gas} for a description of the microphysics included in  the calculation). We show that the hot plasma did not have time to cool down significantly  since the collision was initiated, whereas the denser gas has time to cool and form $\rm H_2$.

\subsubsection{Gas cooling, dust survival and H$_2$ formation in the SQ ridge}
\label{subsubsec:gas-cooling-dust-survival-H2-formation}

We summarize here the context and main results of our calculation of the time-dependence of the gas temperature and dust-to-gas mass ratio. 
We start  the computation with a galactic dust-to-gas mass ratioand equilibrium ionization. We assume that the metallicity of the gas is solar and that the cooling gas is in pressure equilibrium with the  hot, volume-filling gas (the average thermal pressure of the hot plasma is $P / k_{\rm B} = 2 \times 10^5$~K~cm$^{-3}$).  As the gas cools, it condenses. In \hyperref[paper_SQ_H2]{paper~{\sc i}} we explore the possibility that the gas pressure vary around this average value (see in particular Fig.~3).

The H$_2$ formation, gas cooling, and dust destruction timescales are plotted as a function of the postshock temperature in the key-figure 2 of \hyperref[paper_SQ_H2]{paper~{\sc i}}.
The gas cooling timescale is defined as the time at which the temperatures coolds down to $10^4$~K. The H$_2$ formation timescale is the time when the H$_2$ fractional abundance reaches  90\% of its final (end of cooling) value, including the gas cooling time from the postshock temperature to $10^4$~K. The dust destruction timescale is the time when 90\% of the dust mass is destroyed and returned to the gas. We remind that a given initial postshock temperature is associated to a given preshock density. 
The relative values of the timescales with respect to the collision age define three gas phases:

\begin{description}
\item[The hot plasma:] the preshock gas at $n_{\rm H} \lesssim 6 \times 10^{-3}\ \rm cm^{-3}$  is shocked at $V_{\rm s} > 500$~km~s$^{-1}$ and therefore heated to temperatures $T_{\rm ps} > 5 \times 10^6$~K. Our estimate of the cooling timescale of the hot plasma takes into account the time-dependence of the dust-to-gas mass ratio. 
Fig.~2 of \hyperref[paper_SQ_H2]{paper~{\sc i}} shows that,  because the dust grains are efficiently sputtered in the hot gas, the cooling  timescale is much longer ($t_{\rm cool} = 2 \times 10^7$~yr for $T_{\rm ps} = 7 \times 10^6$~K) than if one estimates it for a constant dust-to-gas mass ratio \citep[$t_{\rm cool} = 2 \times 10^6$~yr as estimated by][]{Xu2003}. The cooling timescale of the hot gas is longer than the age of the collision, so the tenuous, shocked gas has not yet cooled down significantly.
This is the X-ray emitting plasma indicated by the red thick line.
Note that this hot gas may still contain some dust because the largest  grains (representing most of the mass) may not have been completely sputtered within the collision age. However, these grains are the less numerous, so their contribution to the gas cooling is weak (see sect.~\ref{subsec:dust-destruction-processes} and \ref{subsec:time-dependent-cooling-gas} for a quantitative discussion of these processes).

\item[The molecular gas:] The preshock gas at $n_{\rm H} \gtrsim 3 \times 10^{-2}\ \rm cm^{-3}$ is shocked at 
$V_{\rm s} < 250$~km~s$^{-1}$ and therefore heated to temperatures $T_{\rm ps} \lesssim 8 \times  10^{5}$~K. In this case, the gas cooling timescale to $10^4$~K and the $\rm H_2$ formation timescale are shorter than the collision age, whereas the dust destruction timescale is longer. Therefore, this gas keeps a significant fraction of its initial dust content and becomes $\rm H_2$ gas (blue thick line) within the age of the collision.

\item[Atomic and ionized  gas:] for intermediate densities ($6 \times 10^{-3} \lesssim n_{\rm H} \lesssim 3 \times 10^{-2}$) and therefore intermediate postshock temperatures ($8 \times 10^{5} < T_{\rm ps} < 5 \times 10^{6}$~K), the gas has time to cool down but it loses its dust content and does not have time to form $\rm H_2$ within the collision age. This phase is indicated with the grey thick line and may represents H$\,${\sc i} and H$\,${\sc ii} gas phases.
\end{description}

This description of the multiphase postshock ignores the fragmentation of the clouds by thermal and hydrodynamical instabilities (Rayleigh-Taylor and Kelvin-Helmholtz) that develop when a cloud is shocked. As discussed in sect.~\ref{subsec:hydro-instabilities}, this fragmentation can lead to the mixing (evaporation), and therefore the destruction, of the clouds with the background hot plasma. 
The powerful H$_2$ emission in the SQ shock suggest that warm molecular gas is formed before the clouds mixing timescale. In sect.~3.3 of \hyperref[paper_SQ_H2]{paper~{\sc i}} we compare the H$_2$ formation timescale to the fragmentation and mixing timescales. The conclusions are the following:

\begin{description}
\item[Cloud fragmentation:]
we show that for a wide range and preshock cloud densities and sizes (see Fig.~4,  \hyperref[paper_SQ_H2]{paper~{\sc i}}), the crushing time is longer than the cooling, so the gas fragments by thermal instability as the shock penetrates into the cloud. 
H$_2$ forms before the shock has crossed the cloud, and therefore before hydrodynamical instabilities start to develop. 

\item[Cloud evaporation:] analytical and numerical studies suggest that the typical evaporation timescale of warm ($\sim 10^4$~K) H$\,${\sc i} clouds in hot ($> 10^6$~K) gas is a few million years (see sect.~\ref{sec:mass-energy-transfers-ISM} for a description of turbulent mixing and references).  This is long enough for H$_2$ to form within the lifetime of the fragments.
The cloud lifetime may be even longer because they are stabilized by the efficient H$_2$ cooling. Up to now, none of the simulations include both the detailed micro-physics (realistic cooling functions and H$_2$ formation on dust grains), and the full dynamic range of spatial scales and densities that are involved in the evolution of clouds embedded into a flow of hot gas (see sect.~\ref{sec:mass-energy-transfers-ISM} for the description of the state-of-art simulations).
\end{description}


\section{How can we account for the H$_2$ excitation?}
\label{sec:H2-excitation}

In this section we adress the question of the H$_2$ excitation in the ridge. The interpretation work carried out in \hyperref[paper_SQ_H2]{paper~{\sc i}} is based on the single-pointing observations of \citet{Appleton2006}. The \textit{IRS} spectral mapping of the ridge presented in sect.~\ref{subsec:spectral_IRSmap_H2} allows us to extend our analysis on the full area of the SQ shock. 
We will also complement the H$_2$ analysis by studying the excitation of the mid-IR fine structure lines in sect.~\ref{sec:opt-midIR-line-excit}.

\subsection{Possible H$_2$ excitation mechanisms in the SQ shock}
\label{subsec:SQ-possible_H2-excitation-mec}

H$_2$ can be excited by several mechanisms: X-ray heating, cosmic-ray heating and shock excitation. We have discussed the micro-physics of these processes in sect.~\ref{subsec:H2excitation-mechanisms} and we discuss here which are the dominant processes for H$_2$ excitation in the environment of the SQ ridge.

\subsubsection{X-ray heating}

The physics of the H$_2$ excitation by X-rays is discussed in sect.~\ref{subsec:H2-collisional-excitation} and  \ref{subsec:H2-cosmic-X-ray-heating}. We show that the energy conversion from X-ray flux to the bolometric $\rm H_2$ emission is at most 10$\,$\% for a molecular cloud that is optically thick to X-ray photons. This excitation efficiency may be even smaller because the absorbed fraction of X-ray photons may be smaller than 1. We indeed expect that the surface filling factor of  the postshock $\rm H_2$ gas  is smaller than 1.

The \textit{Spitzer} observations show that the H$_2$ line luminosity domines the X-ray emission from the SQ shock region. This result is true for the whole SQ ridge, but also for sub-regions extracted in the center of the ridge or in the ``H$_2$ bridge structure'' towards NGC~7319 (see sect.~\ref{subsec:spectral_IRSmap_H2} and \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}).
For the main shock, the total X-ray  flux is $\mathcal{F}_X (0.001-10\, \rm kev) \approx 
2.8 \times 10^{-16}$~W~m$^{-2}$, which corresponds to a luminosity of $\mathcal{L}_X (0.001-10\, \rm kev) \approx 2.95 \times 10^{34}$~W.  Therefore, we find an H$_2$ to X-ray luminosity ratio of
\begin{equation}
\frac{\mathcal{L}_{\rm tot.}(\rm H_2)}{\mathcal{L}_X (0.001-10\, \rm keV) } \approx 3
\end{equation}
Given the X-ray to H$_2$ flux conversion estimated previously, this ratio shows that the H$_2$ gas cannot be predominantly excited by the X-ray photons of the hot plasma. 

\subsubsection{Cosmic ray heating}

Warm $\rm H_2$ gas may also be heated by relativistic particles in the radio ridge. 
The physical processes related to H$_2$ excitation by cosmic-ray ionization ahve been discussed in sect.~\ref{subsec:H2-collisional-excitation} and \ref{subsec:H2-cosmic-X-ray-heating}. 
An enhanced cosmic ray density has been proposed to account for the high temperatures of molecular clouds in the Milky Way nuclear disk  \citep{Yusef-Zadeh2007} and for the mid-IR H$_2$ emission in the filaments of the Perseus A (3C~84) cool core cluster \citep{Ferland2008}. 
Is the cosmic-ray heating can explain the powerful H$_2$ emission in the SQ ridge?

Let us estimate the cosmic-ray ionization rate $\zeta$ that is needed to balance the cooling of the gas by H$_2$ line emission. 
In the SQ ridge, the total H$_2$ line luminosity is $9 \times 10^{34}$~W (see eq.~\ref{eq:H2-line-lumin-total}) and the estimated total mass of H$_2$ is $1.2 \times 10^9$~M$_{\odot}$ (see sect~\ref{subsec:mass-energ-budget}, table~\ref{table_mass_NRJ_budgets_SQ}). Therefore, the average total line emission per H$_2$ molecule is 
\begin{equation}
\mathcal{L}_{\rm H_2}(\rm SQ) \approx 1.3 \times 10^{-31} \quad \rm W \ H_2^{-1}
\end{equation}
We assume that each H$_2$ ionization releases $\mathcal{E}_{\rm ion.}(\rm H_2) \approx 7$~eV of energy to heat the molecular gas (see sect.~\ref{subsec:H2-cosmic-X-ray-heating} for the determination of this value). Therefore, the H$_2$ line cooling is balanced by cosmic ray heating for an ionization rate per hydrogen equal to
\begin{equation}
\zeta = 1.2 \times 10^{-13} \left( \frac{\mathcal{L}_{\rm H_2}(\rm SQ) }{ 1.3 \times 10^{-31} \, \rm W} \right) \left(\frac{7 \, \rm eV}{\mathcal{E}_{\rm ion.}(\rm H_2)} \right)  \quad \rm s^{1} \ H^{-1}
\end{equation}
Therefore, the cosmic-ray ionization rate needed to balance the H$_2$ line cooling in the SQ ridge is $\approx 5 \times 10^3$ times higher than the standard  Galactic rate \citep{Shaw2005}. For a cosmic ray energy density $\approx 5 \times 10^3$ times higher the the Milky Way mean value, the cosmic ray pressure would be a factor 400 higher than the mean cosmic ray pressure in the Milky Way disk \citep[$P_{\rm cos}(\rm MW) \approx 10^4$~K~cm$^{-3}\,$,][]{Boulares1990} and $\approx 20$ times larger than the thermal gas pressure. 
Such a high difference in the pressures is unlikely on large scales. It would imply large departures from the g	as equilibrium and from the  equipartition of energy on a very large volume,  which does not seem to be confirmed by radio observations \citep[see][and paper~{\sc i}]{Xu2003, O'Sullivan2009a}.

However, enhanced cosmic-ray ionization rates may be produced at small scales, for instance in turbulent mixing layers. This turbulent mixing occurs when the flow of the background hot plasma interacts with the molecular clouds. At the interface, cosmic-ray particles can be accelerated efficiently \citep[see][for a review of these processes]{Scalo2004}. For such a high value, cosmic rays are the main destruction mechanism of H$_2$ molecules, and the molecular gas fraction depend on the ionization rate to gas density ratio $ \zeta / n_{\rm H}$. The models by \citet{Ferland2008} show that for $\zeta \approx 10^{-13}$~s$^{-1}$, the gas is molecular for $n_{\rm H} > 10^4$~cm$^{-3}$ (see their figure~2). Given that the warm H$_2$ temperature inferred from the S(1) to S(0) line ratio is $\approx 160$~K (see fig.~9 of  \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}) in the main shock region, the pressure of the warm molecular gas would be $> 2 \times 10^6$~K~cm$^{-3}$, which is physically possible  in the SQ environment.

%However, radio continuum observations of SQ show that the combined cosmic ray plus magnetic energy is not the dominant energy reservoir.

\subsubsection{H$_{\bf 2}$ emission associated with its formation}

The formation of H$_2$ during the cooling of the dense postshock gas (discussed in sect.~\ref{subsec:SQ-H2formation-multiphase-gas}) must be accompanied by H$_2$ emission. The excitation mechanism associated with H$_2$ formation in sect.~\ref{subsec:H2-excitation-during-formation}.
Can this emission explain the powerful H$_2$ excitation in the SQ ridge? To quantify this, we calculate the H$_2$ emission associated with its formation during the isobaric cooling of the gas from $10^4$~K to $\approx 10$~K. This calculation has been discussed in sect.~5 of \hyperref[paper_SQ_H2]{paper~{\sc i}} and we summarize here our results.

Within the framework of a multiphase postshock medium, we assume that the gas that is forming H$_2$ comes from hotter, ionized gas that has recombined. 
We find that the observed H$_2$ rotational line ratios are well reproduced by the model. Fig.~5 of \hyperref[paper_SQ_H2]{paper~{\sc i}} shows that the shape of the H$_2$ excitation diagram associated with H$_2$ formation during the gas cooling matches the observations very well (blue dashed curve).
However, we find that the mass flow of cooling gas (the mass of gas that recombines per unit time, $\dot{M}_{\rm rec} = d M_{\rm rec} / d t$) needed to reproduce the absolute level of H$_2$ emission in the SQ shock is 25 times larger than the mass flow derived from H$\alpha$ observations. We use the following expression to derive $\dot{M_{\rm rec.}}$ from the H$\alpha$ luminosity:
\begin{eqnarray}
\dot{M}_{\rm rec} & = & m_{\rm H} \times \dot{N} _{\rm rec} \\
								& = & m_{\rm H} \times \frac{\mathcal{L}_{\rm H\alpha}}{0.45 \times E}_{\rm H\alpha} \\
								& = & 1263 \times \frac{\mathcal{L}_{\rm H\alpha}}{6.5 \times 10^{33} \ \rm W} \quad \rm M_{\odot}~yr^{-1} \ \ ,
\end{eqnarray}
where $ \dot{N} _{\rm rec}$ is the number of hydrogen atoms that recombine per second, $E_{\rm H \alpha}$ is the energy of an H$\, \alpha$ photon and $\mathcal{L}_{\rm H\alpha}$ is the $H\alpha$ luminosity \citep[see][for details]{Heckman1989}. To match the observed H$_2$ line fluxes with this model would require a mass flow of recombining gas of $\approx 30300$~M$_{\odot}$~yr$^{-1}$, which is not compatible with the mass rate derived from  H$\alpha$ observations ($\approx 1260$~M$_{\odot}$~yr$^{-1}$). This model also fails to reproduce the [O{\sc i}]~6300\AA~line emission by a factor of 7.
Therefore, the cooling of the warm H$\,${\sc i} gas produced by H$\,${\sc ii} recombination
cannot reproduce the observed H$_2$ emission nor the  [O{\sc i}]~6300\AA~line emission. A larger amount of energy needs to be dissipated within the molecular gas to account for the
H$_2$ emission. 

\subsubsection{Shocks}

In \hyperref[paper_SQ_H2]{paper~{\sc i}} we show that, within the \textit{IRS} SH slit aperture centered in the ridge, the dominant energy reservoir of the postshock gas is the bulk kinetic energy of the molecular gas. In sect.~\ref{subsec:mass-energ-budget} we have extended the mass and energy budget of the SQ galaxy collision and shown that the mechanical H$_2$ energy is at least a factor of 2 higher than the thermal energy of the hot plasma for the whole shock. If we assume the equipartition of energy between cosmic rays and magnetic energy, the mean magnetic field strength in the SQ shocked region is $\simeq 10\, \mu$G \citep{Xu2003}.  The
magnetic energy and thereby the cosmic ray energy $\displaystyle \frac{B^2}{8\, \pi} \, V_{\rm MS}$, contained in the volume of the main shock region, $V_{\rm MS} = \mathcal{A}_{\rm MS} \times l_z$, is 
\begin{equation}
\mathcal{E}_{\rm mag.} (\rm SQ) \approx 2 \times 10^{56} \left( \frac{B}{10\,\mu \rm G} \right) ^{2} \frac{\mathcal{A}_{\rm MS}}{446\,\rm kpc^2} \, \frac{l_z}{4 \, \rm kpc} \ ,
\end{equation}
where $l_z$ is the dimension along the line-of-sight and $\mathcal{A}_{\rm MS}$ the area of the main shock region defined in \hyperref[subsec:paper_Cluver]{paper~{\sc ii}} and sect.~\ref{subsec:spectral_IRSmap_H2}. Assuming $l_z \approx 4$~kpc \citep{O'Sullivan2009}, we conclude that the equipartition energy  of cosmic-rays is one order of magnitude smaller than the bulk
kinetic energy of the $\rm H_2$ gas.  So the bulk kinetic energy of the warm H$_2$ gas greatly domines the overall energy budget of the entire SQ ridge structure.

This conclusion drives us to the following interpretation of the extreme H$_2$ power in the SQ ridge: we propose that the H$_2$ emission is powered by the dissipation of turbulent kinetic energy into molecular gas. In the turbulent postshock medium, we expect that the relative motion between the backgroung plasma and the H$82$ gas, but perhaps also the relative motion between the molecular clouds themselves, supply supersonic turbulence in the H$_2$ gas. Since the postshock medium is
magnetized (as indicated by radio synchrotron observations, see sect.~\ref{subsubsec:SQ-radio-observations}), we phenomenologically model this dissipation of mechanic energy by shocks. 
In sect.~\ref{subsec:shocks-molecular-cooling} we have discussed extensively the molecular cooling in  shocks. Non-dissociative MHD shocks are a very efficient way to channel the mechanical energy of the shock to the rotational excitation of H$_2$. Then we favor this process. In the absence of a magnetic field, shocks are rapidly dissociative and much of the cooling of the shocked gas  occurs through atomic, rather than H$_2$, line emission. 



\subsection{Low-velocity MHD shocks and H$_{\bf 2}$ excitation}
\label{subsec:low-velShocksH2excitation}

We quantify the required gas densities and shock velocities to account for the $\rm H_2$ rotational line fluxes. In \hyperref[paper_SQ_H2]{paper~{\sc i}}, we present in details the result for the single-pointing  observations by \citet{Appleton2006}. Here we use our spectral mapping data to extend our analysis on the whole region of the SQ ridge. We compare these new results with our previous analysis in the center of the SQ shock.

The $\rm H_2$ emission induced by low velocity shocks is calculated using an updated version of the shock model of \citet{Flower2003}, presented in sect.~\ref{subsec:shockcode_Flower}.
We use the same grid of models presented in \hyperref[paper_SQ_H2]{paper~{\sc i}}, i.e.  shock
velocities from $3 \ \rm to \ 40$~km~s$^{-1}$ with steps of $1$~km~s$^{-1}$, two values of the initial $\rm H_2$ ortho to para  ratio ($3$ and $10^{-2}$), and three different preshock densities ($n_{\rm H} = 10^2$, $10^3$, and $10^4$~cm$^{-3}$).  
In this models, we assume a standard value for the cosmic ray ionization rate of $\zeta = 5 \times 10^{-17}$~s$^{-1}$. In its initial state, the gas is molecular and cold ($\sim 10$~K), with molecular abundances resulting from the output of our model for the isobaric cooling (see sect.~\ref{subsubsec:gas-cooling-dust-survival-H2-formation} and \hyperref[paper_SQ_H2]{paper~{\sc i}} for details). We adopt the scaling of the preshock magnetic strength with the gas density, $B(\mu G) = b\, \sqrt{n_{\rm H}~[\rm cm^{-3}]}$ \citep{Crutcher1999, Hennebelle2008}. In our models, $b=1$. Since the molecular gas colder than 50~K does not contribute to the H$_2$ emission, we stop the integration when the gas has cooled to 50~K, and we calculate the line fluxes at this point. 

In \hyperref[paper_SQ_H2]{paper~{\sc i}}  we present the result in terms of H$_2$ excitation diagram (see sect.~\ref{subsec:H2excdiagrams} for the details about how it is calculated). In this manuscript we present the observed and model spectral energy distribution (SED) of the H$_2$ line fluxes for \textit{(i)} the same data as in \hyperref[paper_SQ_H2]{paper~{\sc i}}, and \textit{(ii)} the new data of \hyperref[subsec:paper_Cluver]{paper~{\sc ii}} for the main shock region.



We detail how we fit the H$_2$ line fluxes with shock models. In the models presented here, the preshock gas density is $n_{\rm H} = 10^4$~cm$^{-3}$. The shock velocity is the only shock parameter that we allow to vary.  
From the output of the shock model we derive the H$_2$ line brightnesses $\mathcal{B}^{\rm 50\,K} (\rm H_2)$ at 50~K, in units of [W~m$^{-2}$~sr$^{-1}$]. We perform a least-squares fit of the observed $\rm H_2$ line fluxes to a linear combination of two MHD shocks at different velocities $V_{s1}$ and $V_{s2}$ has been performed. These fits provide a scaling factor for each of the shocks which represents a mass flow $\dot{M} = dM/dt$, the amount of gas traversing the shocks per unit time. 
The $\rm H_2$ gas luminosity is proportional to this mass flow.  
For a given H$_2$  line of upper rotational  level $J$, the model line flux is derived as follows:
\begin{equation}
\mathcal{F}^{\rm mod.}_{J} (\rm H_2) = \frac{1}{4 \pi d^2} \,\frac{\dot{M}}{m_{\rm H}} \, \frac{4 \pi \mathcal{B}^{\rm 50\,K}_{J} (\rm H_2)}{n_{\rm H} V_{\rm s}} \quad \rm [W~m^{-2}],
\end{equation} 
where $d$ is the distance to the source (94~Mpc for SQ), $m_{\rm H }$ is the mass of an hydrogen atom, $\dot{M}$ the hydrogen mass flow [kg~s$^{-1}$],  and $n_{\rm H} V_{\rm s}$ represents the flow of hydrogen atoms per unit surface [H~m$^{-2}$~s$^{-1}$].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: Fitting H2 line fluxes with shock models
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[angle=90, width=0.495\textwidth]{figures/sq/H2line_flux_SQ_SH}
    \includegraphics[angle=90, width=0.495\textwidth]{figures/sq/H2line_flux_SQ_MS}
      \caption[Fit of the Stephan's Quintet H$_2$ SED with 2 shocks]{Fit of the Stephan's Quintet H$_2$ spectral energy distribution with 2 shocks at fixed density $n_{\rm H} = 10^4$~cm$^{-3}$.
 \textit{Left:} data from \citet{Appleton2006}, extracted within the \textit{IRS} SH slit aperture in the center of the ridge.  \textit{Right:} data from \citet{Cluver2009} (\hyperref[subsec:paper_Cluver]{paper~{\sc ii}}) for the main shock region.
 The 2 shock components account for comparable fractions of the total H$_2$ luminosity but the less energetic component accounts for most of the warm H$_2$ mass (see table~\ref{tab_shock_mass_SQ_SH} and \ref{tab_shock_mass_SQ_MS}).}
       \label{fig_H2line_flux_SQ}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: CHI2 map for SQ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[angle=90, width=0.495\textwidth]{figures/sq/H2chi2map_twoCshocks_flux_SQ_SH}
    \includegraphics[angle=90, width=0.495\textwidth]{figures/sq/H2chi2map_twoCshocks_flux_SQ_MS}
      \caption[$\chi ^2$ map for C-shocks fit of the SQ H$_2$ SED]{Reduced $\chi ^2$ map for the fit of the Stephan's Quintet H$_2$ spectral energy distribution with 2 shocks at fixed density $n_{\rm H} = 10^4$~cm$^{-3}$. \textit{Left:} data from \citet{Appleton2006}, extracted within the \textit{IRS} SH slit aperture in the center of the ridge. The $\chi ^2$ contours are 1.5, 3, 10, 30. \textit{Right:} data from \citet{Cluver2009} (\hyperref[subsec:paper_Cluver]{paper~{\sc ii}}) for the main shock region. The $\chi ^2$ contours are 40, 100, 200, 300.}
       \label{fig_H2chi2map_twoCshocks_flux_SQ}
\end{figure}


% REsults
The data cannot be fitted with a single shock. For the six H$_2$ lines detected S(0)$-$S(5), we obtain a good fit for two different shock velocities, $V_{s1}$ and $V_{s2}$.
The Fig.~\ref{fig_H2line_flux_SQ} shows the observed and modeled H$_2$ line fluxes for the \citet{Appleton2006} data (left panel, corresponding to the fig.~5 of \hyperref[paper_SQ_H2]{paper~{\sc i}}) and for the main shock region (data from \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}). 
For a preshock density of $10^4$~cm$^{-3}$, the best fit is obtained for a combination of $5$ and $\approx 20$~km~s$^{-1}$ shocks (22~km~s$^{-1}$ for the main shock region)  with an initial value of the ortho to para ratio of $3$. Note  that no satisfactory fit  could be obtained with the low value of the initial H$_2$ ortho-to-para ratio.
The red line shows the weighted sum of the two shock components (best fit). 
The contributions of the $5$ (blue dashed line) and $\approx 20$~km~s$^{-1}$  (green dashed line) shocks to the total column densities are also plotted.
The $5$~km~s$^{-1}$ component dominates the contribution to the column densities of the upper levels of S(0) and S(1) lines.
The $20$~km~s$^{-1}$ component has a major contribution for the upper levels of S(3) to S(5). For S(2), the 2 contributions are comparable.

The fig.~\ref{fig_H2chi2map_twoCshocks_flux_SQ} shows the reduced chi-square contour maps of the two-velocities shock fit for the two apertures used. These maps allow the visualize which are the best combinations of shock velocities to fit the data. As compared to the small aperture in the center of the shock, there are bigger discrepancies between the best-fit model and the data for the extended ridge aperture. We note that the agreement between the model and the data is very good for the odd $J$ values of upper H$_2$ levels, whereas much larger differences are seen for the even-levels.
The error bars on the H$_2$ line fluxes are also much smaller for the main shock aperture because data is much deeper than the previous observations by \citet{Appleton2006}, so the $\chi ^2$ value are thus much higher. The extended ridge aperture is more contaminated by star-forming regions than the small aperture (see chapter~\ref{chapter:SQ_dust} for a discussion of star formation in the ridge), which may explain why the fit is poorer.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLE: SHOCK MODELS PARAM & MASS FLOWS (APPLETON ET AL. DATA)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{1.1} 
\begin{table}
\begin{center}
\begin{minipage}[t]{\textwidth}
\renewcommand{\footnoterule}{}
\def\thefootnote{\alph{footnote}}
\centering
\small
%\footnotemark[1]
\caption[MHD shock model parameters and mass flows for the \citet{Appleton2006} data.]{MHD shock model parameters, mass flows and cooling times for the \citet{Appleton2006} data  \protect\footnotemark[1].}
    \begin{tabular}{ c c c c c c c }
	\hline
	\hline
  \multirow{2}*{$V_s$ \footnotemark[2] } &  \multirow{2}*{Mass Flow} &   \multicolumn{2}{c}{{\sc Cooling Times}} & &   \multicolumn{2}{c}{{\sc Gas Masses}} \\
\cline{3-4}
\cline{6-7}
    &  & $t_{\rm cool}(150\rm K)$ \footnotemark[3] & $t_{\rm cool}(50\rm K)$ \footnotemark[3] & &  (150$\,$K) &  (50$\,$K)  \\
\hline
$[\rm km~s^{-1}]$ & [M$_{\odot}$~yr$^{-1}$]  & [yr] &  [yr] & & [M$_{\odot}$] & [M$_{\odot}$] \\
\hline
5   & 5870 & 14460 & 18160 & & $8.5 \times 10^7$ & $1.07 \times 10^8$ \\
20 &  260  &   2375 &   3230 & & $6.2 \times 10^5$ & $8.5 \times 10^5$ \\
\hline
\end{tabular}
\label{tab_shock_mass_SQ_SH}
\footnotetext[1]{This table lists the mass flows, cooling time to 150~K and 50~K, and molecular gas masses, associated with each shock velocity components.  The models are the same as those used in the left panel of fig.~\ref{fig_H2line_flux_SQ}.}
\footnotetext[2]{MHD Shock velocity.}
\footnotetext[3]{Cooling time computed down to 150~K and 50~K.}
\normalsize
\end{minipage}
\end{center}
\end{table}
\renewcommand{\arraystretch}{1.0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLE: SHOCK MODELS PARAM & MASS FLOWS (CLUVER ET AL. DATA)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{1.1} 
\begin{table}
\begin{center}
\begin{minipage}[t]{\textwidth}
\renewcommand{\footnoterule}{}
\def\thefootnote{\alph{footnote}}
\centering
\small
%\footnotemark[1]
\caption[MHD shock model parameters and mass flows for the \citet{Cluver2009} data.]{MHD shock model parameters, mass flows and cooling times for the \citet{Cluver2009} main shock region data  \protect\footnotemark[1].}
    \begin{tabular}{ c c c c c c c }
	\hline
	\hline
  \multirow{2}*{$V_s$ \footnotemark[2] } &  \multirow{2}*{Mass Flow} &   \multicolumn{2}{c}{{\sc Cooling Times}} & &   \multicolumn{2}{c}{{\sc Gas Masses}} \\
\cline{3-4}
\cline{6-7}
    &  & $t_{\rm cool}(150\rm K)$ \footnotemark[3] & $t_{\rm cool}(50\rm K)$ \footnotemark[3] & &  (150$\,$K) &  (50$\,$K)  \\
\hline
$[\rm km~s^{-1}]$ & [M$_{\odot}$~yr$^{-1}$]  & [yr] &  [yr] & & [M$_{\odot}$] & [M$_{\odot}$] \\
\hline
5   & $6.8\! \times \! 10^4$ & 14460 & 18160 & & $9.8 \times 10^8$ & $1.23 \times 10^9$ \\
22 &  3545                           &  2100  &   2910 & & $7.5 \times 10^6$ & $1.03 \times 10^7$ \\
\hline
\end{tabular}
\label{tab_shock_mass_SQ_MS}
\footnotetext[1]{This table lists the mass flows, cooling time to 150~K and 50~K, and molecular gas masses, associated with each shock velocity components.  The models are the same as those used in the right panel of fig.~\ref{fig_H2line_flux_SQ}.}
\footnotetext[2]{MHD Shock velocity.}
\footnotetext[3]{Cooling time computed down to 150~K and 50~K.}
\normalsize
\end{minipage}
\end{center}
\end{table}
\renewcommand{\arraystretch}{1.0}

Some of the key-parameters derived from the fit are gathered in tables~\ref{tab_shock_mass_SQ_SH} and \ref{tab_shock_mass_SQ_SH} for the two sets of data. We indicate the best-fit shock velocities,  the mass flows $\dot{M}$ that are required to explain the absolute H$_2$ line fluxes, and the gas cooling times $t_{\rm cool.}$ at 150~K and 50~K. The gas masses are derived from $M = \dot{M} \times t_{\rm cool.}$. 
For the main shock region, we find a mass of gas at temperatures larger than
$T=150$~K of $9.8\times 10^8$~M$_{\odot}$, which is a factor of 2 larger than the mass derived from a three-temperatures fit of the excitation diagram (see sect.~4 of  \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}, fig.~9). This difference essentially comes from the fact that multi-temperatures fits assume that the H$_2$ ortho-to-para ratio is thermalized, which is  not the case in shock models. 
In addition, one of the advantages of shock models in estimating the gas masses is that it includes the mass of gas at lower temperatures which has sufficient time too cool before being reheated. The total mass of gas at temperatures above 50~K is $1.2 \times 10^9$~M$_{\odot}$. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLE: MODEL and OBSERVED LINE FLUXES (APPLETON ET AL. DATA)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{1.1} 
\begin{table}
\begin{center}
\begin{minipage}[t]{\textwidth}
\renewcommand{\footnoterule}{}
\def\thefootnote{\alph{footnote}}
\centering
\footnotesize
%\footnotemark[1]
\caption[MHD shock model parameters and predicted H$_2$ line fluxes for the center SQ region]{MHD shock model parameters and predicted H$_2$ line fluxes for the \citet{Appleton2006} data in the center of the SQ ridge \protect\footnotemark[1] for SQ. }
    \begin{tabular}{ c c c c c c c c c}
	\hline
	\hline
 $V_s$ \footnotemark[2]  &  \multicolumn{6}{c}{{\sc H$_2$ Line Fluxes} [$10^{-18}$ W~m$^{-2}$]} &  \multirow{2}*{$\mathcal{F}_{\rm H_2}$ \footnotemark[4]} & \multirow{2}*{$\mathcal{F}_{\rm bol}$ \footnotemark[5]} \\
\cline{2-7}
$\rm [km~s^{-1}]$   & S(0) & S(1) & S(2) & S(3) & S(4) & S(5)  & & \\
\hline 
5   & 1.44 &  17.61 & 2.85 & 0.51 & 0.0028 & 0.0012 & 22.42  & 38.05  \\
20 &  0.06 &  2.33 & 2.90 & 15.30 & 4.47 &  5.90  & 30.96  &  33.15 \\
 \hline 
2 shocks & 1.50 & 19.94  & 5.75  & 15.81 & 4.47   & 5.90   & 53.38 &  71.20 \\
\hline
\textit{Spitzer} obs. & $ 1.9 \pm 0.5 $ & $19.8 \pm 0.6$ & $6.4 \pm 0.6$ & $15.6 \pm 1.1$ & $3.4 \pm 1.1$  & $7.8 \pm 2.4$ & $54.9 \pm 3.1$ &  \\
\hline
\end{tabular}
\label{tab_shock_H2_fluxes_SQ_SH}
\footnotetext[1]{This table lists the shock model velocities, the predicted H$_2$ rotational line fluxes, and bolometric luminosities associated with each shock velocity components. The models are the same as those used in the lesft panel of Fig.~\ref{fig_H2line_flux_SQ}.}
\footnotetext[2]{MHD best fit shock velocities.}
\footnotetext[4]{Sum of the $\rm H_2$ S(0) to S(5) rotational lines in $10^{-18}$ W~m$^{-2}$}
\footnotetext[5]{Sum over all the lines (bolometric luminosity of the shock)}
\normalsize
\end{minipage}
\end{center}
\end{table}
\renewcommand{\arraystretch}{1.0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLE: MODEL and OBSERVED LINE FLUXES (CLUVER ET AL. DATA)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{1.1} 
\begin{table}
\begin{center}
\begin{minipage}[t]{\textwidth}
\renewcommand{\footnoterule}{}
\def\thefootnote{\alph{footnote}}
\centering
\scriptsize
%\footnotemark[1]
\caption[MHD shock model parameters and predicted H$_2$ line fluxes for  the main shock region]{MHD shock model parameters and predicted H$_2$ line fluxes for the \citet{Cluver2009} main shock region \protect\footnotemark[1] for SQ. }
    \begin{tabular}{ c c c c c c c c c}
	\hline
	\hline
 $V_s$ \footnotemark[2]  &  \multicolumn{6}{c}{{\sc H$_2$ Line Fluxes} [$10^{-17}$ W~m$^{-2}$]} &  \multirow{2}*{$\mathcal{F}_{\rm H_2}$ \footnotemark[4]} & \multirow{2}*{$\mathcal{F}_{\rm bol}$ \footnotemark[5]} \\
\cline{2-7}
$\rm [km~s^{-1}]$   & S(0) & S(1) & S(2) & S(3) & S(4) & S(5)  & & \\
\hline 
5   & 1.67 & 20.41 &  3.30 &  0.59 & 0.003  &   0.001 & 26.0  & 44.1  \\
22 &  0.07 & 2.98 & 3.90 &  22.67 &  7.92 & 13.33 & 50.9 &  55.5 \\
 \hline 
2 shocks & 1.74 &  23.4 &   7.20 &    23.26 & 7.92 & 13.34 & 76.9 & 99.6 \\
\hline
%3.09±0.19 23.05±0.26 9.10±0.38 22.76±0.84 2.5±1.0 14.1±0.7
\textit{Spitzer} obs. & $ 3.09 \pm 0.19$ & $23.05 \pm 0.26$ & $9.10 \pm 0.38$ & $22.76 \pm 0.84$ & $2.5 \pm 1.0$  & $14.1 \pm 0.7$ & $74.6 \pm 1.6$ &  \\
\hline
\end{tabular}
\label{tab_shock_H2_fluxes_SQ_MS}
\footnotetext[1]{This table lists the shock model velocities, the predicted H$_2$ rotational line fluxes, and bolometric luminosities, associated with each shock velocity components, for the main shock region (aperture $\mathcal{A}_{\rm MS} \approx 2310$~arcsec$^2$). The models are the same as those used in the right panel of Fig.~\ref{fig_H2line_flux_SQ}.}
\footnotetext[2]{MHD Shock velocity.}
\footnotetext[4]{Sum of the $\rm H_2$ S(0) to S(5) rotational lines in $10^{-17}$ W~m$^{-2}$}
\footnotetext[5]{Sum over all the lines (bolometric luminosity of the shock)}
\normalsize
\end{minipage}
\end{center}
\end{table}
\renewcommand{\arraystretch}{1.0}

The gas luminosities are listed in Table~\ref{tab_shock_H2_fluxes_SQ_SH} and \ref{tab_shock_H2_fluxes_SQ_MS} for the \citet{Appleton2006} small aperture and for the extended shock region. 
We list the H$_2$ S(0) to S(5) line fluxes from each best-fit shock model velocity and the sum of the two shocks. The observed values are indicated at the bottom line.  
The two last rows show the total H$_2$ S(0)$-$S(5) flux and the bolometric flux of the shocks obtained by integrating the emission in all lines. The bolometric luminosities are smaller than the kinetic luminosities 
\begin{equation}
\mathcal{L}_{\rm kin.} = \frac{1}{2} \, \dot{M} \, V_{\rm s} ^2 
\end{equation}
because some of the mechanical energy of the shock is transferred to the magnetic energy. The H$_2$ line  luminosities are close to the bolometric values obtained by integrating the emission in all lines because the H$_2$ rotational lines are the main cooling lines of magnetic shocks (see sect.~\ref{subsec:shocks-molecular-cooling} for a discussion of the energetics of magnetic shocks).
Summing over the two shocks,  we estimate a total luminosity of $8.2 \times 10 ^ {34}$~W for the S(0)$-$S(5) H$_2$ lines, which is excellent agreement with the observed value ( $8.0 \pm 0.2 \times 10 ^ {34}$~W).

Our grid of models shows that this solution is not unique. 
If one decreases the density to  $10^3$~cm$^{-3}$, we find that one can fit the observations with a combination of MHD shocks (at $9$ and $35$~km~s$^{-1}$). %, $\chi ^2 = 1.37$).
If one decreases the density to  $10^2$~cm$^{-3}$, the rotational $\rm H_2$ excitation cannot be fitted satisfactorily. At such low densities, MHD shocks fail to reproduce the S(3) and S(5) lines because the critical densities for rotational H$_2$ excitation increase steeply with the $J$ rotational quantum number (see sect.~\ref{subsec:H2-thermometer-critical-densities}).
The warm H$_2$ pressures $\rho \, V^{2}$ in the two shocks are $4.5 \times 10^{7}$~K~cm$^{-3}$ and $5.6 \times 10^{8}$~K~cm$^{-3}$) for the $5$~km~s$^{-1}$ and $20$~km~s$^{-1}$ shocks, respectively. These pressure are much higher than the pressure of the background hot plasma ($\approx 2 \times 10^5$~K~cm$^{-3}$).
Both warm and dense (i.e. high pressure)  gas is needed to account for emission from the higher $J$ levels.


Though the fit is not unique, it gives an estimate of the relevant range of shock velocities required to account for the H$_2$ excitation. The velocities ($\approx 5 - 20$~km~s$^{-1}$) are remarkably low compared to the SQ collision velocity ($\approx 1000$~km~s$^{-1}$) and to the velocity dispersion of the warm molecular gas ($\approx 900$~km~s$^{-1}$).
If our interpretation of the H$_2$ emission in terms of shock-driven dissipation of energy within the warm molecular gas is right, such a contrast in velocities is a beautiful illustration of turbulent cascade, from high-velocities at large scales, to low-velocity at small scales.
The fact that energy dissipation occurs over this low velocity range is an essential key to account for the importance of H$_2$ cooling. High velocity shocks ($> 40-50$~km~s$^{-1}$) in dense ($n_{\rm H} > 10^4$~cm$^{-3}$) molecular gas would dissociate H$_2$ molecules.
However, we are far from understanding in details how the transfer of energy from the background plasma (shocked at high speed, $\approx 700$~km~s$^{-1}$, see sect.~\ref{subsubsec:Xray_obs_SQ}) to the molecular gas. This is discussed qualitatively in sect.~5 and 6 of  \hyperref[paper_SQ_H2]{paper~{\sc i}}, and we will come back to this question in sect.~\ref{sec:SQ-Why-H2-important-coolant}.



\subsection{Future observational tests: near-IR H$_{\bf 2}$ line emission}

A missing piece of the puzzle of the SQ shock is the near-IR spectrum. This would allow to have access to  both ro-vibrational H$_2$ cooling lines and atomic lines, and therefore to gain a more complete picture of the total line cooling in the SQ shock. The near-IR ro-vibrational lines sample much hotter H$_2$ gas than the Spitzer data (see chapter~\ref{chapter:H2Molecule}). 
In particular, near-IR spectroscopy will allow us to extend the H$_2$ excitation diagram into the hotter
regime, where we can start to distinguish between dissociative or non-dissociative type of shocks.  This would have important implications for how the energy cascades down from the large
scale turbulence to the small cloud fragments. 


A proposal has been written to perform near-IR spectroscopy with the  \textit{TripleSpec} instrument installed on the  Palomar 200-inch telescope (P.I.: P.N. Appleton).
The spectral ($ \mathcal{R}=2600$ or $\Delta v =  115$~km~s$^{-1}$) and spatial (1'') resolution of TripleSpec is far superior to that of the \textit{Spitzer IRS}, and is crucial to determine if the large velocity
spread seen in the Mid-IR H$_2$ lines ($\sigma \approx 800-900$~km~s$^{-1}$) represents a single broad line  or two separate narrow lines indicating both pre-and post shocked material. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: Palomar Proposal C vs. J shocks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[angle=90, width=0.9\textwidth]{figures/sq/H2excitDiag_SQ_Rovib_lines.pdf}
      \caption[Model prediction of H$_2$ ro-vibrational emission in SQ]{The excitation diagram of H$_2$ emission in Stephan's Quintet from observations \citep[black symbols from][]{Appleton2006} compared with a model of the post-shock gas from \citep{Guillard2009}. The model predicts fluxes for the ro-vibrational lines in the range $0.2 - 14 \times 10^{-18}$~W~m$^{-2}$ over a solid angle of $5 \times 10$ arcsec$^{2}$, depending on the kind of shock. Observations in the near-IR can significantly limit the kinds of shocks capable of explaining the excitation diagram. These will influence our picture of how eneregy is funnelled down to 20~km~s$^{-1}$ shocks from the large-shock ($V_{\rm s} \sim 600$~km~s$^{-1}$) which creates the X-ray emission.}
       \label{H2excitDiag_SQ_Rovib_lines}
\end{figure}



 Fig~\ref{H2excitDiag_SQ_Rovib_lines} shows example
of dissociative and non-dissociative shock predictions from the shock model grid presented in  \hyperref[paper_SQ_H2]{paper~{\sc i}}. The blue dotted curve is our best fit model for C-shocks presented in sect.~\ref{subsec:low-velShocksH2excitation}, Fig.~\ref{fig_H2line_flux_SQ} (left panel). 
The red curve is a model where the higher velocity component (20~km~s$^{-1}$) is dissociative (J-type). In this case, the ro-vibrational line fluxes are much higher than the non-dissociative case because the gas reaches higher temperatures. Near-IR spectroscopy should provide constrains on the contribution from non-ionizing shocks to the H$_2$ emission. This would help in determining if these shocks can contribute to other line emission, like [O$\,${\sc i}] 6300\AA~for instance.

I participated to our first observation run at Palomar observatory to perform near-IR spectroscopy with the newly-commissioned \textit{TripleSpec} instrument in November 2008 with Phil Appleton and Patrick Ogle. Unfortunately the weather was very bad and we have only detected, through the clouds, some H$_2$ emission from the NGC~7319 Seyfert galaxy. The proposal was re-submitted and accepted for a new observation run in August 2009. 

\section{Why is H$_{\bf 2}$ such an important coolant?}
\label{sec:SQ-Why-H2-important-coolant}

Our interpretation of mid-IR line emission, but also optical and X-ray emission, within the context of a multiphase postshock gas, suggests that observations can be understood in terms of dynamical interactions between the ISM phases (sect.~\ref{subsec:mass_energy_transfers}). Exchanges of mass and energy between the gas phases seem a key to elucidate why the H$_2$ power is so high in the ridge. An efficient transfer of the bulk kinetic energy of the gas to turbulent motions of much lower velocities within molecular clouds seems required to make H$_2$ a dominant coolant of the postshock gas (sect.~\ref{subsec:SQ-energy-transfer-H2-power}). Here we briefly summarize and update the discussion of \hyperref[paper_SQ_H2]{paper~{\sc i}} (sect.~5 and 6). 


\subsection{Mass and energy cycle between ISM phases}
\label{subsec:mass_energy_transfers}

In the Stephan's Quintet shock region, observations and modeling suggest that the dissipation of the mechanical energy of the collision between a galaxy and a tidail tail is the main source to power the X-ray emission, the optical, and mid-IR line emission from the gas in the ridge. The relative luminosities from the different gas components depend on the dynamical coupling between the gas phases. In this section we propose a scenario for the postshock gas evolution that sketches the dynamical interaction between ISM phases. This interpretation introduces a physical framework that may apply to other astrophysical situations (AGN-driven jets in radio-galaxies, supernova remnants, starburst-driven winds, etc.).

\begin{figure}
 \centering
       \includegraphics[width=0.7\textwidth]{figures/sq/mass_flows}
   \caption[Sketch of the mass and energy cycle between ISM phases]{Schematic view at the gas evolutionary cycle proposed in our interpretation of Stephan's Quintet optical and H$_2$ observations.
Arrows represent the mass flows between the H~II, warm H~I, warm and cold H$_2$ gas components. They are numbered for clarity. The dynamical interaction between gas phases drives the cycle.
The mass flow values and associated timescales are derived from the $\rm H_{\alpha}$, O{\sc i}, and $\rm H_2$ luminosities and model calculations. Heating of the cold H$_2$ gas (red arrows) is necessary to account for the increasing mass flow from the ionized gas to cold H$_2$  phases. }
  \label{fig:mass_flows}
   \end{figure}

 Fig.~\ref{fig:mass_flows} sketches our view at the mass and energy exchanges between the different gas phases that control the evolution of the postshock gas.  This cartoon is the same as Fig.~6 of \hyperref[paper_SQ_H2]{paper~{\sc i}} except that the values of the mass flows are updated for the full SQ ridge.
 Black and red arrows represent the mass flows between the H$\,${\sc ii}, H$\,${\sc i}, warm and cold H$_2$ gas components of the post-shock gas. The large arrow to the left symbolizes the relative motion between the warm and cold gas and the surrounding plasma.
Each of the black arrows is labeled with its main associated process: gas recombination and ionization (arrow number 1), H$_2$ formation (2) and H$_2$ cooling (3). The values of the mass flows and the associated timescales are derived from observations and our model calculations.

The total mass flow associated with the low-velocity component of MHD shocks required to reproduce the H$_2$ line fluxes is much larger ($\approx 68000$~M$_{\odot}$~yr$^{-1}$) than the mass flow of recombining gas derived from H$\alpha$ observations ($\approx 1260$~M$_{\odot}$~yr$^{-1}$).
The mass rates needed to account for the $\rm H_{\alpha}$, O{\sc i}, and $\rm H_2$ luminosities increases. Therefore, one cannot explain the $\rm H_2$ luminosity with only a continuous cycle through the gas components, from H$\,${\sc ii} to cold $\rm H_2$. 
Heating of the cold H$_2$ gas towards warmer gas states (red arrows) needs to occur.

The main energy reservoir that can power these red arrows is the mechanical energy of the galaxy collision. We propose that mass and energy are transfered from cold molecular gas via shocks. 
The post-shock molecular cloud fragments are likely to experience a distribution of shock velocities, depending on their size and density. Arrow number 4 represents the low velocity magnetic shocks excitation of H$_2$ gas that can account for the H$_2$ emission (described in sect.~\ref{subsec:low-velShocksH2excitation}).
More energetic shocks may dissociate the molecular gas (arrows number 5).
They are necessary to account for the low H$ _{\alpha}$ to [O~{\sc i}]~6300~\AA~luminosity ratio.
Even more energetic shocks may ionize the molecular gas (arrow number 6).
This would bring cold $\rm H_2$ directly into the H~{\sc ii} reservoir.

%%% REWRITE

The H$\,${\sc ii} gas can also be produced by the turbulent mixing of the warm and cold gas with the hot background plasma (see sect.~\ref{subsec:turbulent-mixing} for a description of turbulent mixing layers). This is represented by the thin blue and orange arrows from the cold and warm molecular gas reservoirs to the hot plasma. This mixing produces gas at intermediate temperature (a few $10^5$~K) that is thermally instable. At these temperatures, the thermal sputtering of the dust is uneffective, so dust is preserved. This gas cools back to produce H$\,${\sc ii} gas that re-enters the cycle (thin green arrow). 

An important question is to know whether there is a significant mass of cold ($< 50$~K) molecular gas  associated with the warm H$_2$. This cold gas does not contribute to the H$_2$ emission.
The mass accumulated in this cold H$_2$ reservoir depends on the ratio between the timescale of mechanical energy dissipation  (on which gas is excited by shocks through one of the red arrows 4, 5 and 6) and the cooling timescale along the black arrow 3. 

Following the calculation made in sect.~6 of \hyperref[paper_SQ_H2]{paper~{\sc i}}, we estimate the timescale of dissipation of the turbulent energy, $t_{\rm turb}$, and compare it to the cooling time of the warm H$_2$ gas. We assume that the  dissipation of turbulent energy  powers the H$_2$ emission, so the energy dissipation rate $P_{\rm turb}$ must be at least equal to the power radiated by H$_2$, $\mathcal{L}_{\rm H_2}$.
Thus we write the turbulent dissipation timescale as the ratio of the total turbulent energy of the warm H$_2$ gas, $E_{\rm turb}$,  to the total H$_2$ power:
\begin{eqnarray}
t_{\rm turb} & = & \frac{E_{\rm turb}}{P_{\rm turb}} \\
                     & = & \dfrac{\frac{3}{2} M_{\rm H_2} \sigma _{\rm turb}^{2}}{\mathcal{L}_{\rm H_2}} \\
					 & = & 1.14 \times 10^4 \, \left( \frac{M_{\rm H_2}}{1.2 \times 10^9 \, \rm M_{\odot}}\right) \left( \frac{ \sigma _{\rm turb}}{10 \, \rm km \, s^{-1}}\right) ^{2} \left( \frac{10^{35} \, \rm W}{\mathcal{L}_{\rm H_2}} \right) \quad \rm [yr]
\label{eq:turbulent-diss-time}
\end{eqnarray}
In Eq.~\ref{eq:turbulent-diss-time}, $M_{\rm H_2}$ is the total warm H$_2$ mass and $\sigma _{\rm turb}$ is the turbulent velocity dispersion within the warm H$_2$ gas.
Using the  H$_2$ luminosity and the warm H$_2$ mass in Table~\ref{table_mass_NRJ_budgets_SQ}, we
estimate a turbulent dissipation timescale of $\approx 10^4$~yr for a typical dispersion velocity of $\approx 10$~km~s$^{-1}$. This estimate of the  turbulent dissipation timescale is a lower limit since the dissipated power $P_{\rm turb}$ may be larger if it powers the dissociative and ionizing shocks represented by the arrows 5 and 6 in Fig.~\ref{fig:mass_flows}.
Therefore, cold H$_2$ gas would be heated by turbulent dissipation on timescales comparable to the cooling time of the warm H$_2$ gas that accounts for the S(0) and S(1) line emission ($1.8 \times 10^4$~yr, see table~\ref{tab_shock_mass_SQ_MS}). 
If this is correct, the cold molecular gas mass should not be much higher than the warm H$_2$ mass inferred from the \textit{Spitzer} observations. 

We compare the turbulent dissipation timescale to the dissipation timescale of the total bulk kinetic energy of the warm H$_2$ gas, $t_{\rm TDK}$, which can be written as the ratio between the H$_2$  gas bulk kinetic energy and H$_2$ luminosity:
\begin{equation}
t_{\rm TDK} = 5.7 \times 10^8 \left( \frac{E_{\rm kin}(\rm H_2)}{1.8 \times 10^{51} \, \rm J} \right) \left(\frac{10^{35} \, \rm W}{\mathcal{L}_{\rm H_2}} \right)  \quad \rm [yr]
\end{equation}
The turbulence dissipation timescale  $t_{\rm turb}$ is more than three orders of magnitude smaller than  $t_{\rm TDK}$. Therefore, the dissipation of the mechanical energy of the galaxy collision must involve a large ($\gtrsim 1\,000$) number of cycles where H$_2$ gas fragments are accelerated and dissipate their kinetic energy in shocks. 

\subsection{Physics of the energy transfer: qualitative discussion}
\label{subsec:SQ-energy-transfer-H2-power}

We have shown that the bulk kinetic energy of the gas accelerated by the shock induced by the galaxy collision has to be transfered efficiently within molecular gas to explain the powerful H$_2$ emission. 
However, how this energy transfer occurs is far from being known. We discuss here two possible processes: \textit{(i)} the momentum transfer induced by the motion of clouds in the hot plasma, and \textit{(ii)} the production of cosmic rays in the turbulent mixing layers. The first process is discussed in more details in sect.~6.1 of \hyperref[paper_SQ_H2]{paper~{\sc i}}.

\subsubsection{Supersonic turbulence sustained by the motion of clouds}

We remind that in our interpretation of the H$_2$ emission in the SQ halo, the formation of H$_2$ gas arises from the compression of shocked H$\,${\sc i} gas. The two pre-collision H$\,${\sc i} complexes, one associated with the intruding galaxy NGC~7318b and the other with NGC~7319's tidal tail, move at a relative velocity of $\approx 900$~km~s$^{-1}$ with respect to each other. 
While they are compressed and becoming H$_2$ clouds, the clouds  move at high velocity with respect to the background plasma because they keep their preshock momentum. 
In the collision, the clouds do not share the same dynamics as the lower density intercloud gas, and the kinetic energy recorded in the  $\approx 900~\rm km\,s^{-1}$ H$_2$ line width  is dominated by the bulk motion of the H$_2$ clouds in the plasma rest frame.

The background flow applies drag forces on the clouds  \citep{Murray2004}. 
Because of the viscosity of the fluid, the dynamical friction (shear forces) between the cloud and the hot flow also lead to a transport of momentum from the fast flow into the cloud.
Analytical and numerical studies of shock-cloud interactions, or studies of the interaction between  an outflow and molecular clouds seem to show that the injection of momentum within cloud can feed supersonic turbulence within clouds \citep[e.g.][]{Kornreich2000, Matzner2007, Carroll2009}. The turbulent energy injected into the clouds is dissipated by low-velocity shocks into the dense molecular material. 
Besides, the relative motion between cloud fragments  can lead to cloud-cloud collisions, which  results in the dissipation of  kinetic energy  preferentially in the molecular gas because it is the coldest component with the lowest sound speed.

In addition to dynamics, the thermodynamics of the multiphase gas is a key to understand the energy transfers between the phases.
First, the cooling of the gas transfers the turbulent energy of the hotter  H$\,${\sc ii} and H$\,${\sc i} phases to the H$_2$ gas. Secondly, the thermal instability is also a efficient mechanism to convert the thermal energy to turbulent kinetic energy. Numerical simulations \citep{Sutherland2003, Audit2005} show that the thermal instability inhibits energy-loss through radiation from the warmer gas and feeds turbulence in the cooler gas. The turbulent velocities generated by the thermal instability are found to be of the order of the sound speed in the warmer gas and are thus supersonic for the colder gas.

\subsubsection{H$_{\bf 2}$ heating by cosmic rays produced in turbulent mixing layers}

An alternative mecanism to transfer the bulk kinetic energy of the gas to H$_2$ heating is the production of cosmic-ray particles in the turbulent mixing layers that would scatter within the molecular clouds and excite H$_2$ molecules (see sect.~\ref{subsec:H2excitation-mechanisms} for a description of H$_2$ excitation by cosmic rays). 
In sect.~\ref{subsec:SQ-possible_H2-excitation-mec} we show that the average cosmic-ray ionization rate in the SQ ridge is likely to be too low to balance the H$_2$ cooling. The advantage of cosmic-ray acceleration in mixing layers is that cosmic-ray particles are produced \textit{locally} and can diffuse into the H$_2$ gas. Cosmic rays are accelerated by the Fermi mechanism and can in turn generate turbulence and MHD waves into the molecular gas if they are accelerated to velocities faster than the local Alfvén speed. These processes are reviewed by \citet{Scalo2004} (see their sect.~4) and we direct the reader to this review for references. 

The two processes discussed above (shocks induced by momentum transfer or cosmic ray excitation produced by turbulent mixing) are two alternative means to cascade the bulk kinetic energy of the gas on large scales to small-scale dissipation withinthe H$_2$ gas. From an astrophysical point of view, the most important point is that the H$_2$ emission traces the dissipation of the bulk kinetic energy of the system. 



\section{Optical and mid-IR fine structure line diagnostics}
\label{sec:opt-midIR-line-excit}

In the previous sections we have shown that the dominance of the H$_2$ line cooling in the SQ shock region would require an efficient cascade of energy from the large-scale, bulk kinetic energy of the gas to small-scale turbulent motions within the H$_2$ gas. 
However, the H$_2$ rotational lines observed by \textit{Spitzer} do not provide a complete budget of the kinetic energy dissipation in the SQ ridge. These low-excitation lines trace gas between $\approx 50 - 1000$~K, and therefore they only sample a narrow range of shock velocities. 
Within the framework of our interpretation of the H$_2$ emission (the high-speed collision of two flows of multiphase gas), we expect a broad distribution of shock velocities. 

Fast shocks may lead to the line emission from ionized gas, which, up to now, has not been considered. This section adresses the following questions: is the emission from the ionized gas an important component of the energetics in the SQ ridge? 
Is H$_2$ really a dominant coolant? 
We first describe optical imaging and spectroscopy, as well as mid-IR fine-struture line maps from our new \textit{Spitzer IRS} observations. We use line ratios diagnostics to infer the shock properties from the ionized gas.

\subsection{H${\bf \alpha}$ imaging and optical line spectroscopy}
\label{subsec:opticallineemission_shocks}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%           FIGURE: Halpha MAPS OF SQ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
   \includegraphics[width=0.55\textwidth]{figures/sq/SQ_Ha_map.jpg}
     \includegraphics[width=0.44\textwidth]{figures/sq/SQ_Ha_velocity_map.jpg}
      \caption[H$\alpha$ contours and velocity maps of SQ]{H$\alpha$ contours and velocity maps of SQ. \textit{Left:} High-velocity ($> 5500$~km~s$^{-1}$, white contours) and low-velocity ($\sim 800$~km~s$^{-1}$, gray scale) H$\alpha$ maps of Stephan's Quintet. \textit{Right:} Velocity map obtained from the low-$v$ and high-$v$ H$\alpha$ images. Figures taken from \citet{Gutierrez2002}.}
       \label{fig_SQ_Ha}
   \end{figure}

\citet{Moles1997, Vilchez1998, Xu1999, Plana1999, Sulentic2001, Gutierrez2002} present narrowband filter and Fabry-Pérot images that show a chaotic morphology of emission-line regions and complex H$\,${\sc ii} gas kinematics. 
The left panel of Fig.~\ref{fig_SQ_Ha} shows H$\alpha$ maps of SQ from \citet{Gutierrez2002}. The white contours result from combination of four narrowband filter images centered at different wavelengths (from 6667\AA~to 6737\AA), covering the full velocity range of the SQ galaxies ($4760-7960$~km~s$^{-1}$). The grey-scale background image is a combination of two images centered at 6569\AA~($280$~km~s$^{-1}$) and 6611\AA~($2200$~km~s$^{-1}$), and thus mainly exhibits the NGC~7320 foreground galaxy. The white contours clearly show an extended and clumpy North-South H$\alpha$ filament that spatially correlates with the radio emission in the ridge, as well as an East-West feature (we called it the ``bridge'') that connects the nucleus of the Seyfert 2 NGC~7319 with the North-South ridge. In addition, emission-line regions associated with the new intruder and with the northern SQ-A region are detected.

The two background images on Fig.~\ref{fig_SQ_HI_contours_Sulentic} show H$\alpha$ Fabry-Pérot images from \citet{Sulentic2001}, centered at $\sim 6600$~km~s$^{-1}$ (left panel) and $\sim 5600$~km~s$^{-1}$ (right panel). 
These images show different morphologies. The $6600$~km~s$^{-1}$ image shows the North-South clumpy, linear shock structure, the core of NGC~7319 and its ``bridge'', and the SQ-A starburst. On the $5600$~km~s$^{-1}$ image, the intra-group emission has an ``arc shape'', with brighter emission in the southern region. This southern arc is comprised of a string of H$\alpha$ knots that connects to the east end of the faint bar in the new intruder NGC~7318b. This southern arc may be material disrupted from NGC~7318b that has been compressed by the shock. This arc almost connects to a fainter string starting from the core of NGC~7318a, then forming a peculiar ``smily face'' (the cores of NGC~7318 a and b would be the eyes of this giant smiley!), also clearly visible on the UV (see the central panel of  Fig.~\ref{fig_SQ_radio_GMRT_OSullivan2009}) and mid-IR (see chapter~\ref{chapter:SQ_dust}) images.
Note that in some regions, the two velocities components have similar morphologies \citep[see also Fig.~2 of][]{Xu1999}. This emission may arise from gas at intermediate velocities ($\sim 6000 $~km~s$^{-1}$) that may be shock-accelerated material from the new intruder.

Up to now, very few high signal-to noise optical spectra in the SQ ridge have been published.  \citet{Xu2003} performed optical spectroscopy with the Palomar 200''  telescope at several positions along the SQ ridge. In the center of the shock the flux ratios are:
\begin{eqnarray}
\mathcal{F}([\rm O\, I]~\lambda 6300) / \mathcal{F}(\rm H\,\alpha + [N\, II]) & = & 0.53 \\
\mathcal{I}(\rm [S\, II]~\lambda 6717, \lambda 6731) / \mathcal{I}(\rm H\,\alpha + [N\, II]) &= &1.09 \\
 \mathcal{I}([\rm O\, III]~\lambda 5007) / \mathcal{I}(\rm H\,\beta) &>& 1 \ .
\end{eqnarray}
These ratios are different from those observed in H$\,${\sc ii} regions, and suggest shock excitation. Based on the shock models by \citet{Dopita1995}, \citet{Xu2003} conclude that these lines are predominantly excited by fast ($V_{\rm s} > 100$~km~s$^{-1}$) shocks. 
In fact, the [O$\,${\sc i}] / H$\alpha$ line ratio is so high that it is difficult to explain this ratio only with fast shock models (see sect.~\ref{subsec:SQ-lines-fast-shocks}). 

Optical emission lines are mainly detected at three velocities (6800, 6100, and 6400~km~s$^{-1}$). The
H$\,\alpha$, [N$\,${\sc ii}],  [S$\,${\sc ii}] and  [O$\,${\sc ii}] lines are detected predominently at 6100~km~s$^{-1}$, and the [O$\,${\sc iii}]~$\lambda 5007$ line is detected at 6800~km~s$^{-1}$.
The [O$\,${\sc i}]~$\lambda 6300\,$\AA~ line is centered at 6400~km~s$^{-1}$, and is remarkably broad, with a FWHM $\Delta v \simeq 1130$~km~s$^{-1}$. The width of the line is commensurate with the relative velocity between the intruder and the tidal tail.

\citet{Dopita1996} give  the following  relation for the total energy flux of a radiative shock: 
\begin{equation}
\mathcal{F}_{\rm tot} = 2.28 \times 10^{-6} \left( \frac{V_{\rm s}}{100~\rm km\,s^{-1}} \right) ^3 \left( \frac{n_{\rm H}}{\rm cm^{-3}}\right) ~\rm W~m^{-2} \ ,
\end{equation}
where $n_{\rm H}$ is the preshock hydrogen number density and $V_{\rm s}$ the shock velocity.
We use the aperture $\mathcal{A}_{\rm MS}$ corresponding to the SQ ``main shock region'' ($30 \times 77$~arcsec$^{2}$, corresponding to $\sim 13.7 \times  35.1$~kpc$^{2}$). 
Therefore, the total mechanical luminosity of the SQ high-speed shock propagating into the tenuous intra-group medium is given by: 
\begin{equation}
\mathcal{L}_{\rm tot} = 5.48 \times 10^{36} \left( \frac{V_{\rm s}}{700~\rm km\,s^{-1}} \right) ^3 \left( \frac{n_{\rm H}}{\rm 3.2 \times 10^{-2}~cm^{-3}}\right) \left( \frac{\mathcal{A}_{\rm MS}}{2310~\rm kpc^2} \right)  ~\rm W
\end{equation}
From X-ray observations, \citet{Trinchieri2003, Trinchieri2005, O'Sullivan2009} estimate the average hydrogen density of the hot plasma in the ridge to be $n_{\rm H} \simeq 1.17 \times 10^{-2}$~cm$^{-3}$. For a fast shock, the postshock density is about 4 times the preshock density (sect.~\ref{sec:MHD_shocks}), so we estimate a preshock density of the tenuous gas of $n_{\rm H} \simeq 3.2 \times 10^{-3}$~cm$^{-3}$. The total mechanical energy flux for the SQ main shock is thus $\mathcal{F}_{\rm tot} \simeq 2.6s \times  10^{-6}$~W~m$^{-2}$.  

If we assume that this luminosity is radiated over a galaxy crossing time (the shock age) of $5 \times 10^6$~yr, the intruder/IGM collision deposits $\sim 8.7 \times 10^{57}$~erg of energy in the SQ shock region. This energy is  equivalent to the kinematic energy of $\sim 10^7$ supernovae. 




\subsection{Distribution of the fine-structure line emission}
\label{subsec:IRSmap_fine_struct_lines}

\citet{Appleton2006} reported the detection of the [Ne$\,${\sc ii}] $\lambda 12.8\,\mu$m and [Si$\,${\sc ii}] $\lambda 34.8\,\mu$m lines. Thanks to the deeper spectral maps, we have access to the  
spatial distribution of emission from the [Fe$\,${\sc ii}] $\lambda 25.99\,\mu$m and [O$\,${\sc iv}] $\lambda 25.89\,\mu$m blend, [S$\,${\sc iii}] $\lambda 33.48\,\mu$m, [Si$\,${\sc ii}] $\lambda 34.82\,\mu$m,
[Ne$\,${\sc ii}] $\lambda 12.8\,\mu$m and [Ne$\,${\sc iii}] $\lambda 15.56\,\mu$m lines. 

Fig.~4 and 5 of  \hyperref[subsec:paper_Cluver]{paper~{\sc ii}} show the intensity contours of these fine-structure lines overlaid on H$_2$  S(1) and X-ray maps. The strong  [Si$\,${\sc ii}]$\lambda 34.82\,\mu$m emission spatially correlates with the H$_2$ and X-ray emission, whereas the [Fe$\,${\sc ii}]$\lambda 25.99\,\mu$m line emission is only detected towards the AGN NGC~7319 and the center of the ridge, where there is a bright spot of X-ray emission. We direct the reader to sect.~3.2 of \hyperref[subsec:paper_Cluver]{paper~{\sc ii}} for a detailed description of these fine-structure line emission maps. We now discuss the interpretation of these observations with models that allow to constrain the gas physical conditions and the dominant excitation mechanisms (shocks, X-rays, photoionization). 


\subsection{Optical and mid-IR fine structure lines as shock diagnostics}
\label{subsec:SQ-lines-fast-shocks}

The deep mid-IR spectral mapping data presented above allow to complement the analysis of the rotational H$_2$ lines with the fine-structure line emission from the SQ ridge (see sect.~\ref{subsec:spectral_IRSmap_H2} for a description of the observational results). 
These metal lines provide complementary diagnostics to probe the physical conditions of the emitting gas and more energetic excitation mechanisms. Since the main shock region (the X-ray ridge) also contains star forming regions, we have selected a sub-region of our extended \textit{IRS} spectral mapping, so-called \textit{``center''} because it is located in the central region of the ridge, that has less contamination by star-forming regions (see sect.~4, Fig.~7 of  \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}). We compare the line ratio diagnostics within these two apertures. 

We use the \citet{Allen2008}  shock model library described in sect.~\ref{sec:fast-shock-models} to compare models with the fine structure line ratios measured with \textit{Spitzer IRS} data. The model results depend on the preshock magnetic parameter $b=B/\sqrt{n_{\rm H}}$, where $B$ is the magnetic field strength and $n_{\rm H}$ the preshock gas density. In the models presented here, we assume $b=1$, which is slightly lower than the equipartition value of 3.23. We compare the model results with and without the radiative precursor. The radiative precursor of a fast shock moving into low-density
gas adds an emission component which has the spectral characteristics of photoionized gas with a high ionization parameter.
To neglect the precursor may be relevant if the shock is propagating in a clumpy medium because only a fraction of the ionizing photons will interact with the molecular gas (see sect.~\ref{sec:shocksinmultiphasemedia}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: FAST SHOCK MODELS: LINE RATIOS for S
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/SIII33_SIII18_Vsh_SQ}
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/SIII33_SIII18_Vsh_SQ_s}
      \caption[Model and observed fine-structure line ratios for SQ]{The fine-structure line ratios measured in the SQ shock (full ridge and sub-region in the center) are  compared with shock calculations (broken curves)  from \citet{Allen2008}. The model values are shown for shock velocities between 100 and 1000~km~s$^{-1}$ (with steps of 25~km~s$^{-1}$ ), four preshock gas densities ($n_{\rm H} = 1$, 10, 100 and 1000~cm$^{-3}$) for a magnetic parameter $B/\sqrt{n_{\rm H}} = 1$.   Observed values are the horizontal solid lines in colors.}
       \label{fig_SIII33_SIII18_Vsh_SQ}
\end{figure}

The [S$\,${\sc iii}] lines ratios are shown on Fig.~\ref{fig_SiII_SIII33_Vsh_SQ} as a function of the shock velocity. The broken curves are the shock models for different preshock gas densities ($1-1000$~cm$^{-3}$). The solid coloured lines are the observed values.
The electron  critical densities of the [S$\,${\sc iii}]$\lambda 33.48\,\mu$m and [S$\,${\sc iii}]$\lambda 18.71\,\mu$ lines are $n_{e} = 1.2 \times 10^{3}$~cm$^{-3}$ and $n_{e} = 10^{4}$~cm$^{-3}$, respectively. The observed ratio for the full ridge (2.46) is close to the low density limit \citep[$n_{e} < 100$~cm$^{-3}$, see Fig.~8 of][]{Mart'in-Hern'andez2002}. The comparison with shock models show that the gas preshock density is smaller than $\sim 1$~cm$^{-3}$. The lower limit for the shock sub-region is compatible with preshock gas densities smaller than $100$~cm$^{-3}$ and shock velocities $100 < V_{\rm s} < 300$~km~s$^{-1}$.
The [S$\,${\sc iii}] lines ratio diagnostic clearly shows that the mid-IR line emission from the ionized gas originates from moderate shocks (of the order of 100~km~s$^{-1}$) in low-density ($\approx 1$~km~s$^{-1}$). Faster shocks in denser gas would not be compatible with the available ram pressure in the surrounding hot plasma ($\approx 2 \times 10^5$~K~cm$^{-3}$).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: FAST SHOCK MODELS: LINE RATIOS for Si
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/SiII_SIII33_Vsh_SQ}
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/SiII_SIII33_Vsh_SQ_s}
      \caption[Model and observed fine-structure line ratios for SQ]{The fine-structure line ratios measured in the SQ shock (full ridge and sub-region in the center) are  compared with shock calculations (broken curves)  from \citet{Allen2008}. The model values are shown for shock velocities between 100 and 1000~km~s$^{-1}$ (with steps of 25~km~s$^{-1}$ ), four preshock gas densities ($n_{\rm H} = 1$, 10, 100 and 1000~cm$^{-3}$) for a magnetic parameter $B/\sqrt{n_{\rm H}} = 1$.   Observed values are the horizontal solid lines in colors.}
       \label{fig_SiII_SIII33_Vsh_SQ}
\end{figure}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: FAST SHOCK MODELS: LINE RATIOS for Ne
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/NeIII_NeII_Vsh_SQ}
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/LineRatios_SiII_NeIII_NeII_NeIII_SQ}
      \caption[Model and observed fine-structure line ratios for SQ]{Observed mid-IR line ratios compared with shock models (same as Fig.~\ref{fig_SiII_SIII33_Vsh_SQ}.  The model values are shown for shock velocities between 100 and 1000~km~s$^{-1}$ (with steps of 25~km~s$^{-1}$ ), four preshock gas densities ($n_{\rm H} = 1$, 10, 100 and 1000~cm$^{-3}$) for a magnetic parameter $B/\sqrt{n_{\rm H}} = 1$.   Observed values are the horizontal solid lines in colors. The Ne line ratios shown on the \textit{left} panel contrain the shock velocities to be of order of $100-200$~km~s$^{-1}$. This result is confirmed by the Ne and S line diagnostic plot on the \textit{right panel}. Note that the radiative precursor is included in both panels.  }
       \label{fig_NeIII_NeII_Vsh_SQ}
\end{figure}

XDRs\footnote{X-ray Dissociation Regions} models show that the  [Si$\,${\sc ii}] line is one of the major mid-IR cooling line from gas exposed to X-rays \citep[see Fig.~8 of][]{Maloney1996}. 
XDRs models have been used to interpret the line emission from AGN.
Powerfull [Si$\,${\sc ii}] line emission can also be produced by shock excitation, whereas the  [S$\,${\sc iii}] mid-IR lines are mostly tracers of H$\,${\sc ii} regions. Therefore, the [Si$\,${\sc ii}] /  [S$\,${\sc iii}] line ratio measures the ratio between the X-rays or shocks and photoionization excitation powers.

Fig.~\ref{fig_SiII_SIII33_Vsh_SQ} shows the observed (solid, coloured lines) and model (broken curves) [Si$\,${\sc ii}]$\lambda 34.82\,\mu$m /  [S$\,${\sc iii}]$\lambda 33.48\,\mu$m and  [S$\,${\sc iii}]$\lambda 33.48\,\mu$m /  [S$\,${\sc iii}]$\lambda 18.71\,\mu$m line flux ratios as a function of the shock velocity, and for different preshock gas densities ($1-1000$~cm$^{-3}$). The [S$\,${\sc iii}]$\lambda 33.48\,\mu$m line is not detected in the sub-region in the center of the shock, so we indicate an lower limit for the line ratios (red line). For comparison, the average line ratios observed in local AGN and extragalactic star-forming regions (from the \textit{SINGS}\footnote{\textit{Spitzer} Infrared Nearby Galaxies Survey, \url{http://sings.stsci.edu/}} survey) are shown.

The [Si$\,${\sc ii}] /  [S$\,${\sc iii}] SQ line ratios stand out above typical values observed in star-forming regions or AGN, and cannot be accounted for by PDRs or XDRs models. They are rather consistent with the line ratios observed in supernova remnants (see sect.~5 of \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}), suggesting shock-excitation. 
The  lower limit of the  [Si$\,${\sc ii}]$\lambda 34.82\,\mu$m /  [S$\,${\sc iii}]$\lambda 33.48\,\mu$m line ratio observed in the SQ shock sub-region seems to be consistent with $\sim 100$~km~s$^{-1}$ shocks into $n_{\rm H} \simeq 10$~cm$^{-3}$ gas. Unlike the sub-region, the SQ-A starburst line ratios are consistent with the values observed in standard extragalactic star-forming regions. This shows that photoionization must be the dominant process in this region, with a minor contribution from shocks. 

The Fig.~\ref{fig_NeIII_NeII_Vsh_SQ} shows the [Ne$\,${\sc iii}]$\lambda 15.56$ / [Ne$\,${\sc ii}]$\lambda 12.8$ line flux ratio as a function of the shock velocity (left panel) or as a function of the  [Si$\,${\sc ii}] / ([Ne$\,${\sc ii}] + [Ne$\,${\sc iii}]) line ratio. 
For our range of preshock densities ($1-1000$~cm$^{-3}$), the shock models show that the observed line  ratios are consistent with shock velocities of $\sim 100 - 200$~km~s$^{-1}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%				FIGURE: FAST SHOCK MODELS: LINE RATIOS for OI/Halpha and Ne II / Ne III
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
   \centering
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/LineRatios_OIHa_NeII_NeIII_SQ}
    \includegraphics[angle=90, width=0.49\textwidth]{figures/sq/LineRatios_OIHa_NeII_NeIII_SQ_s}
      \caption[Model and observed optical and fine-structure line ratios for SQ]{Ne fine-structure line ratio vs. optical line ratio measured in the SQ shock (sub-region in the center) as  compared with shock calculations (broken curves)  from \citet{Allen2008}. The model values are shown for shock velocities between 100 and 1000~km~s$^{-1}$ (with steps of 25~km~s$^{-1}$ ), four preshock gas densities ($n_{\rm H} = 1$, 10, 100 and 1000~cm$^{-3}$) for a magnetic parameter $B/\sqrt{n_{\rm H}} = 1$. In the \textit{left} panel, the radiative precursor is included, whereas in the \textit{right} panel, only the shock contribution is plotted.}
       \label{fig_LineRatios_OIHa_NeII_NeIII_SQ}
\end{figure}


\citet{Xu2003} suggest that the optical lines ratios observed in the center of the ridge (see sect.~\ref{subsec:opticallineemission_shocks}) are evidence for a dominant shock excitation.
The mid-IR fine structure lines detected by \textit{Spitzer} confirm this conclusion. 
However, the large value of the [O$\,${\sc i}] / H$\alpha$ line ratio observed in the ridge, 
$\mathcal{F}([\rm O\, I]~\lambda 6300) / \mathcal{F}(\rm H\,\alpha + [N\, II])  =  0.53$, is difficult to explain with fast shocks models. Fig.~\ref{fig_LineRatios_OIHa_NeII_NeIII_SQ} shows the [Ne$\,${\sc ii}] to  [Ne$\,${\sc iii}] ratio as a  function of the [O$\,${\sc i}] / H$\alpha$ optical line ratio. 
In the left panel, where the precursor is included, the observed value do not match with the models.
The mid-IR [Ne$\,${\sc ii}] to  [Ne$\,${\sc iii}] line ratio in SQ suggest a low ionization parameter, whereas the radiative precursor produces a highly-ionized medium ahead of the shock. This apparent contradiction can be solved if the SQ intragroup medium is clumpy. In this case, a large fraction of the ionizing photons can escape from the medium without interacting with the dense phase.
 If we neglect the radiative precursor (right panel), we find a much better agreement with the models. The   line ratios are reproduced for a preshock density of $n_{\rm H} = 10-10^2$~cm$^{-3}$ and a shock velocity of $V_{\rm s} = 200 - 250$~km~s$^{-1}$. These conditions imply high values of the postshock pressure as compared with the ambient value. 
Note that a significant contribution from non-ionizing $J$-shocks contribute to the optical lines, in particular to the [O$\,${sc i}] 6300\AA~line (see sect.~\ref{subsec:shocks-molecular-cooling}). 
This will be further discussed in sect.~\ref{subsec:mass_energy_transfers}.


In sect.~6 of \hyperref[subsec:paper_Cluver]{paper~{\sc ii}} we discuss the [Fe$\,${\sc ii}] $\lambda 25.99\,\mu$m and  [Si$\,${\sc ii}]$\lambda 34.82\,\mu$m line emission. The fact that the observed [Fe$\,${\sc ii}] / [Ne$\,${\sc ii}]  and  [Si$\,${\sc ii}] /  [Ne$\,${\sc ii}] line ratios are both smaller than the
shock model values can be interpreted as evidence for Si and Fe depletion onto dust grains (see Fig.~11 of \hyperref[subsec:paper_Cluver]{paper~{\sc ii}}). This supports our idea that dust survives in the dense gas phases that are the sites for H$_2$ formation. This will be further discussed in chapter~\ref{chapter:SQ_dust} where we model the dust emission from the molecular gas in SQ.

\subsection{Conclusion: a distribution of shock velocities}

The X-ray, optical and mid-IR line emissions from the SQ shock suggest that the gas experiences a wide distribution of shock velocities. We relate this distribution of shock velocities with a distribution of preshock gas densities, due to the multiphasic nature of the preshock medium (\hyperref[paper_SQ_H2]{paper~{\sc i}}).  The denser gas phases are associated with the smaller shock velocities. 

Very fast shocks  ($V_{\rm s} \sim 700$~km~s$^{-1}$) driven into preshock gas of a few $10^{-3}$~cm$^{-3}$ are responsible for the bright X-ray emission in the ridge. Optical lines and mid-IR fine-structure lines are likely to be produced by intermediate ($100 < V_{\rm s} < 300$~km~s$^{-1}$) ionizing $J$-shocks. A significant contribution from non-ionizing $J$-shocks can also contribute to these lines, in particular to the [O$\,${\sc i}] 6300\AA ~(which may help in explaining the very high value of  [O$\,${\sc i}]/ H$\,\alpha$), [Fe$\,${\sc ii}] $\lambda 25.99\,\mu$m and  [Si$\,${\sc ii}]$\lambda 34.82\,\mu$m lines. And last but not least, low-velocity ($5-20$~km~s$^{-1}$), non-dissociative $C$-shocks driven into dense gas ($>10^3$~cm$^{-3}$) are associated to the rotational H$_2$ emission seen by \textit{Spitzer}.





\section{Remarks about the NGC~7319 Seyfert galaxy}
\label{SQ-NGC7319-comments}
\index{NGC 7319!outflow}
\index{NGC 7319!bridge}

\subsection{Observational context: and AGN in the SQ group}

In this short paragraph I gather some observational results about the NGC~7319 galaxy. Although not related to the SQ main shock itself, these results are helpful to interpret our recent, extended IR and CO observations of SQ.

\citet{VanDerHulst1981} first detected the NGC~7319 AGN with radio continuum VLA observations of
SQ at 20cm. They detected a bright compact source with a jet-like extension, and suggested this might be related to those found in Seyfert galaxies. \citet{Huchra1982} obtained the optical spectrum which shows clearly Sy2-type emission-line features. Based on the stellar velocity dispersion, \citet{Woo2002} estimated a black hole mass of $2.4 \times 10^7$~M$_{\odot}$.
\citet{Aoki1999} made VLA A-array radio continuum observations, complimented with an
archival HST optical image. They found a chain of 3 radio sources, interpreted as the nucleus
and its two jets on opposite sides. Optical features are found in the HST image closely related
to the radio jets, interpreted as gas compressed and excited by bow shocks driven into the
ambient medium by the jets. This is different from the so-called extended emission line regions
(EELR) which are supposedly excited by the AGN radiation \citep{Aoki1996}. 

Even higher
resolution (0.16'') radio continuum observations at 1658 MHz, using MERLIN, were reported
by \citet{Xanthopoulos2004}. They compared the data with an HST/ACS U-band (F330W)
image, and found extended UV emission around the nucleus and the northern jet. They argued
that this indicates star formation triggered by the jet/ISM interaction. By assuming the diffuse
radio emission outside the compact sources is due to the star formation, they estimated that
the SFR in the circum-nuclear region is 8.4~M$_{\odot}$~yr$^{-1}$. However, all of the optical spectra of emission line regions in the circum-nuclear region show Seyfert or LINER line ratios and none is H$\,${\sc ii} region-like \citep{Aoki1996}, indicating that most of the radio and UV radiation is related to the AGN and/or the shocks. Comparing the UV and MIR observations, \citet{Xu2005} found the AGN
and the surrounding region is highly obscured, with an FUV extinction of $A_{\rm FUV} = 5.4$~mag, consistent with the Sy2 classification.

\subsection{The H$_{\bf 2}$ bridge: AGN-driven outflow or tidal interactions?}

\index{NGC 7319!outflow}
\index{NGC 7319!bridge}

Our new \textit{Spitzer} spectral maps presented in sect.~\ref{subsec:spectral_IRSmap_H2} show that the H$_2$ emission extends from the ridge to the core of the AGN NGC~7319. 
This ``H$_2$  bridge'' feature is also seen on the 1.4~GHz radio image \citep[see Fig.~\ref{fig_SQ_Xrays_radio_contours} and][]{Williams2002}, on H$\,\alpha$ maps \citep[see Fig.~\ref{fig_SQ_Ha} and][]{Xu1999, Plana1999, Sulentic2001, Gutierrez2002}, and faintly detected in X-rays \citep[see Fig.~\ref{fig_SQ_CFHT_Xray} and][]{Trinchieri2003, Trinchieri2005}. The distribution of the H$_2$ emission seems to correlate with that of the radio emission. 

The origin of the ``H$_2$  bridge''  is unclear. Is it related to the AGN activity of NGC~7319, or is it related to past or recent galaxy interactions? Optical spectroscopy \citep{Aoki1996} and VLA radio observations \citep{Aoki1999} seem to support the first hypothesis. Indeed, \citet{Aoki1996} interpret the large velocity gradients between the AGN core and the South-West bridge as an high-speed ($\sim 500$~km~s$^{-1}$) jet-induced outflow of gas. The very high electron density in the outflow ($\sim 600$~cm$^{-3}$, twice that of the nucleus) and the multiple radio structure in the jet suggest that the outflow is interacting with interstellar matter. The H$_2$ emission in this bridge may then be powered by jet-driven shocks within dense clouds or/and AGN radiation. \citet{Cluver2009} propose an alternative explanation: the bridge is a remnant of previous tidal interactions. This scenario is suggested by the similarity between the mid-IR spectrum and X-ray properties of the \textit{ridge} and \textit{bridge} regions. This picture fits in the context of multiple shock heating events proposed by \citet{Moles1997, Sulentic2001, O'Sullivan2009}.
The two scenarii (AGN-driven outflow and galaxy-wide shock) are difficult to disentangle because they lead to similar observational signatures. Our new CO observations in the ridge and in the bridge set a new light on this question, and we will discuss this further in sect.~\ref{sec:CO_EMIR}.

\section{Summary and conclusions}
\label{sec:SQ-conclusions}

One of the most interesting features of the Stephan's Quintet compact group is the presence of a galaxy-wide shock in the halo of the group, created by an intruding galaxy colliding with a tidal tail at a relative velocity of $\sim 1\,000$~km~s$^{-1}$.  Evidence for a group-wide shock comes from observations of X-rays from the hot postshock gas in the ridge strong radio synchrotron emission from the radio emitting plasma and shocked-gas excitation diagnostics from optical emission lines. \textit{Spitzer} observations show that this gas also contains molecular hydrogen with an extreme velocity dispersion. The $\rm H_2$ luminosity  is larger than the X-ray emission from the same region, thus the $\rm H_2$ line emission dominates over X-ray cooling in the shock. As such, it plays a major role in the energy dissipation and evolution of the postshock gas. 

The interpretation of these observations is the core of my PhD work. I present a scenario where H$_2$ gas forms out of the postshock gas that results from the supersonic collision between two multiphase gas streams. 
This collision leads to a multiphase medium with a distribution of shock velocities, related to the variations of the density in the preshock medium. The H$_2$ formation in the SQ ridge environment is quantified by calculating the time-dependent isobaric cooling of the gas, including dust destruction mechanisms. I show that H$_2$ forms out of the dense regions where dust survives the shocks. 
The bulk kinetic energy of the molecular gas is the main energy reservoir of the postshock gas, and it has to be dissipated within the H$_2$ gas to explain the poserful H$_2$ excitation. I propose that supersonic turbulence is sustained within the molecular gas by a transfer of momentum induced by cloud-cloud collisions and the relative shear motions between the molecular gas and the hot plasma. A phenomenological model of low-velocity MHD shocks driven into the dense H$_2$ gas is capable of explaining the observed excitation characteristics.

Within this framework, dust is a key ingredient. It is required for H$_2$ formation. Our model has implications on the expected dust emission in the SQ halo and on dust survival in a multiphase environment. These points are adressed in the next chapter, as well as a discussion of star formation in the SQ group.

\section{Publications}
\label{sec:publications}

In the following, we reproduce the two papers \citet{Guillard2009}, \textit{H$_2$ formation and excitation in the Stephan's Quintet galaxy-wide collision}, 2009, A\&A, 502, 515, and \citet{Cluver2009}, \textit{Powerful H2 line-cooling in Stephan's Quintet : I- Mapping the dominant cooling pathways in group-wide shocks}, submitted to ApJ. These papers contain key-figures that have discussed in this chapter, and a lot of details that we have intentionally not repeated in this manuscrit.

\subsection{Paper I}
\label{paper_SQ_H2}
\includepdf[noautoscale=true, scale=0.9,link=true,frame=true,pages=-]{papers/Guillard2009.pdf}

\subsection{Paper II}
\label{subsec:paper_Cluver}
 \includepdf[noautoscale=true, scale=0.9, frame, pages=-, fitpaper=true, link=true]{papers/Cluver2009.pdf}




==> conclusion_french.tex <==

%%% Chapter heading commands %%%

\chapter*{Conclusions}
\label{chapter:conclusion_french}

%\renewcommand{\publ}{\flushleft\footnotesize{Published as:
%C. Grigorescu, N. Petkov and M.A. Westenberg -- \textit{``Contour
%Detection Based on non-CRF Inhibition,''} IEEE Transactions on Image
%Processing, vol. 12, no. 7, pp. 729--739, July 2003.}}


%\epigraph{I hate quotations. Don't use quotations. Tell me what you know.}{
%Ralph Waldo Emerson}
\epigraph{C'est long de faire court, c'est bien connu!}{André Brahic, pendant un cours.}
%\epigraph{Le bruit d'aujourd'hui est l'information de demain}{Didier Pelat, pendant un cours.}
%\index{Molecular hydrogen in space!Mol}

%%% Abstract %%%

%\begin{Abstract}



%{Abstract}
Conclusion en français

%%% Chapter sections %%%

%\index{Visual system}

%\PARstart{O}ne of the most frequently encountered tasks in machine




==> introduction.tex <==

%%% Chapter heading commands %%%

\chapter*{Introduction}
\label{chapter:introduction_en}

%\renewcommand{\publ}{\flushleft\footnotesize{Published as:
%C. Grigorescu, N. Petkov and M.A. Westenberg -- \textit{``Contour
%Detection Based on non-CRF Inhibition,''} IEEE Transactions on Image
%Processing, vol. 12, no. 7, pp. 729--739, July 2003.}}


%\epigraph{I hate quotations. Don't use quotations. Tell me what you know.}{
%Ralph Waldo Emerson}
\epigraph{The question is not what you look at, but what you
see.}{Henry David Thoreau}

%\index{Molecular hydrogen in space!Mol}

%%% Abstract %%%

%\begin{Abstract}

%\end{Abstract}


%%% Chapter sections %%%

%\index{Visual system}
\section*{The Universe is like a great wine\dots}
\label{sec:intro_wine_context}
%\PARstart{O}ne of the most frequently encountered tasks in machine


starbursts = cosmic fireworks

\section*{Honey, what have you been searching for?}
\label{sec:intro_issues}

\section*{and so what have you been doing exactly?}

\begin{floatingfigure}[r]{0.55\textwidth}
   \includegraphics[width=0.52\textwidth]{figures/fun/physicists_BillOfRights.jpg}
\end{floatingfigure}



\section*{So, OK, you've been searching for something\dots but at least, did you ``find'' something?}
\label{sec:intro_find?}


==> preface.tex <==
\chapter*{Preface}

==> thesis_remerciements.tex <==
\chapter*{Remerciements}
\pagestyle{empty}

\epigraph{L'art c'est moi, la science c'est nous}{Claude Bernard}

Une route sinueuse. Des sacrifices, du travail et beaucoup d'aventures et de satisfaction.
Le cheminement. Le  début H2Ex, la modélisation. 
La découverte observationnelle de Phil. Le sujet défini.



First and foremost, I would like to especially thank François Boulanger, 
with whom I worked during these three years. It is difficult to ask 
more from a supervisor~! I greatly appreciated his kindness, his dynamism, his availability, 
the clarity of his explanations, and his patience, despite my many questions~! We have always worked
as a team, in a relaxed atmosphere and I really enjoyed all the discussions we had about the
physics of the interstellar medium.

I would like to acknowledge François Boulanger, Alain Abergel and Anthony for having allowed me to
participate in the School of Les Houches on interstellar dust. It was a very enriching week. I'd like to thank Xander Tielens and Hugues Leroux for nice discussion we had about presolar grains. 
 
%I thank all the members of the astrochemistry and interstellar matter \& cosmology groups and
%particularly Louis D'Hendecourt, Janet Borg and Zahia Djouadi for their advice, clarifications, 
%and huge skills in the physics of implantation and analysis of presolar grains. 
%I am very honoured to have had such a team of scientists at my side~!

I also appreciated the hospitality of the IAS staff. I would like to thank Ghislaine Renoux 
for the hard-to-find articles she managed to get for me. Moreover, I enjoyed all the many seminars
organized by the group. Relaxing coffee and lunch breaks also contributed to this friendly work
atmosphere. A special acknowledgement to all the PhD students of IAS, especially Nathalie,
Faustine, Nicolas, Mathieu and Doug for your friendship and for the good time spent in Les Houches,
playing ping pong, cards and babyfoot~! Thanks Doug for the car trip~!

A thought to my former supervisors, Karl-Ludwig Klein and Gilles Theureau, for always 
having kept in touch with me and without whom my passion for astrophysical research wouldn't
exist~! 
%See you in Prague, Gilles, for the IAU meeting in August~!

I will always be grateful to my family and friends, and last but not least, a big kiss to Carole, for her love, support and 
understanding.


{\flushright Pierre Guillard\\ Orsay\\ \today\\ }

